A Unified Multisensor Machine-Learning Framework for Live Fuel Moisture Content Retrieval

Live fuel moisture content controls vegetation flammability and is a high-importance variable in fire management. Nevertheless, it remains difficult to estimate and map over large areas due to the concentration of field observations in specific regions. We develop a unified machine-learning framework that estimates live fuel moisture content from satellite vegetation indices, meteorological variables, topography and seasonal predictors. GlobeLFMC 2.0 measurements are matched to Terra and Aqua MODIS, VIIRS, Landsat 8/9, Sentinel-2 and Sentinel-3 surface-reflectance products, combining the long MODIS record with finer-resolution recent observations. To account for differences among sensors, optical predictors are restricted to a common red, near-infrared and shortwave-infrared feature space; site--product combinations and field time series are screened for remote-sensing suitability; and spectral response function diagnostics are combined with target-independent empirical reflectance calibration toward a Sentinel-2 reference domain. Preliminary single-product experiments show that weather, topography and cyclic day-of-year provide most of the predictive gain beyond vegetation indices, whereas optional product-specific predictors do not justify their additional dependencies. Separate Grass, Shrub and Tree models are trained with Random Forest and XGBoost regressors. Under the primary validation design, which withholds observation dates from sites represented in training, the best models achieve pooled R2 values of 0.715, 0.693 and 0.700 for Grass, Shrub and Tree, respectively. The framework can incorporate additional optical sensors when compatible reflectance bands, documented spectral responses and sufficient overlap observations are available for calibration and validation.

==> Definitions/journalnames.tex <==
%%%%% Updated 14 October 2026 %%%%%
%%-----  All MDPI journal information -----%%
%\DeclareOption{}{%
%	\gdef\@journal{}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@societyowner{}
%	\gdef\@journaltype{}}
%%% Website Name
%%% Website Name
%%% Full Name
%%% Short Name-ISO4
%%% DOI abbr
%%% ISSN
%%% Society Owner
%%% Journal type
\DeclareOption{aam}{%
	\gdef\@journal{aam}
	\gdef\@journalfull{Advanced Air Mobility}
	\gdef\@journalshort{Adv. Air Mobil.}
	\gdef\@doiabbr{aam}
	\gdef\@ISSN{3043-0399}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aamr}{%
	\gdef\@journal{aamr}
	\gdef\@journalfull{Annals of African Medical Research}
	\gdef\@journalshort{Ann. Afr. Med. Res.}
	\gdef\@doiabbr{aamr}
	\gdef\@ISSN{2297-7007}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aapm}{%
	\gdef\@journal{aapm}
	\gdef\@journalfull{Advances in Anesthesia and Pain Medicine}
	\gdef\@journalshort{Adv. Anesth. Pain Med.}
	\gdef\@doiabbr{aapm}
	\gdef\@ISSN{3103-2214}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{acbr}{%
	\gdef\@journal{acbr}
	\gdef\@journalfull{Annals of Clinical and Biomedical Research}
	\gdef\@journalshort{Ann. Clin. Biomed. Res.}
	\gdef\@doiabbr{acbr}
	\gdef\@ISSN{2724-508X}
	\gdef\@societyowner{Nigerian Medical Association Enugu State}
	\gdef\@journaltype{ACS}}
\DeclareOption{accountaudit}{%
	\gdef\@journal{accountaudit}
	\gdef\@journalfull{Accounting and Auditing}
	\gdef\@journalshort{Account. Audit.}
	\gdef\@doiabbr{accountaudit}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{acn}{%
	\gdef\@journal{acn}
	\gdef\@journalfull{Advances in Carbon Neutrality}
	\gdef\@journalshort{Adv. Carbon Neutrality}
	\gdef\@doiabbr{acn}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{acoustics}{%
	\gdef\@journal{acoustics}
	\gdef\@journalfull{Acoustics}
	\gdef\@journalshort{Acoustics}
	\gdef\@doiabbr{acoustics}
	\gdef\@ISSN{2624-599X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{actuators}{%
	\gdef\@journal{actuators}
	\gdef\@journalfull{Actuators}
	\gdef\@journalshort{Actuators}
	\gdef\@doiabbr{act}
	\gdef\@ISSN{2076-0825}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{addictions}{%
	\gdef\@journal{addictions}
	\gdef\@journalfull{Addictions}
	\gdef\@journalshort{Addictions}
	\gdef\@doiabbr{addictions}
	\gdef\@ISSN{0006-0006}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{addictprev}{%
	\gdef\@journal{addictprev}
	\gdef\@journalfull{Addiction \& Prevention}
	\gdef\@journalshort{Addctn. Prev.}
	\gdef\@doiabbr{addictprev}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{adhesives}{%
	\gdef\@journal{adhesives}
	\gdef\@journalfull{Adhesives}
	\gdef\@journalshort{Adhesives}
	\gdef\@doiabbr{adhesives}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{admsci}{%
	\gdef\@journal{admsci}
	\gdef\@journalfull{Administrative Sciences}
	\gdef\@journalshort{Adm. Sci.}
	\gdef\@doiabbr{admsci}
	\gdef\@ISSN{2076-3387}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{adolescents}{%
	\gdef\@journal{adolescents}
	\gdef\@journalfull{Adolescents}
	\gdef\@journalshort{Adolescents}
	\gdef\@doiabbr{adolescents}
	\gdef\@ISSN{2673-7051}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aee}{%
	\gdef\@journal{aee}
	\gdef\@journalfull{Advances in Environmental Engineering}
	\gdef\@journalshort{Adv. Environ. Eng.}
	\gdef\@doiabbr{aee}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aep}{%
	\gdef\@journal{aep}
	\gdef\@journalfull{Agricultural Economics and Policy}
	\gdef\@journalshort{Agric. Econ. Policy}
	\gdef\@doiabbr{aep}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aerobiology}{%
	\gdef\@journal{aerobiology}
	\gdef\@journalfull{Aerobiology}
	\gdef\@journalshort{Aerobiology}
	\gdef\@doiabbr{aerobiology}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aeronautics}{%
	\gdef\@journal{aeronautics}
	\gdef\@journalfull{Aeronautics}
	\gdef\@journalshort{Aeronautics}
	\gdef\@doiabbr{aeronautics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aerospace}{%
	\gdef\@journal{aerospace}
	\gdef\@journalfull{Aerospace}
	\gdef\@journalshort{Aerospace}
	\gdef\@doiabbr{aerospace}
	\gdef\@ISSN{2226-4310}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{agriculture}{%
	\gdef\@journal{agriculture}
	\gdef\@journalfull{Agriculture}
	\gdef\@journalshort{Agriculture}
	\gdef\@doiabbr{agriculture}
	\gdef\@ISSN{2077-0472}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{agriengineering}{%
	\gdef\@journal{agriengineering}
	\gdef\@journalfull{AgriEngineering}
	\gdef\@journalshort{AgriEngineering}
	\gdef\@doiabbr{agriengineering}
	\gdef\@ISSN{2624-7402}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{agrochemicals}{%
	\gdef\@journal{agrochemicals}
	\gdef\@journalfull{Agrochemicals}
	\gdef\@journalshort{Agrochemicals}
	\gdef\@doiabbr{agrochemicals}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{agronomy}{%
	\gdef\@journal{agronomy}
	\gdef\@journalfull{Agronomy}
	\gdef\@journalshort{Agronomy}
	\gdef\@doiabbr{agronomy}
	\gdef\@ISSN{2073-4395}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ai}{%
	\gdef\@journal{ai}
	\gdef\@journalfull{AI}
	\gdef\@journalshort{AI}
	\gdef\@doiabbr{ai}
	\gdef\@ISSN{2673-2688}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aiaerosp}{%
	\gdef\@journal{aiaerosp}
	\gdef\@journalfull{AI for Aerospace}
	\gdef\@journalshort{AI Aerosp.}
	\gdef\@doiabbr{aiaerosp}
	\gdef\@ISSN{3043-193X}
	\gdef\@societyowner{Southeast University}
	\gdef\@journaltype{ACS}}
\DeclareOption{aiagents}{%
	\gdef\@journal{aiagents}
	\gdef\@journalfull{AI Agents and Autonomous Systems}
	\gdef\@journalshort{AI Agents Auton. Syst.}
	\gdef\@doiabbr{aiagents}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aibiol}{%
	\gdef\@journal{aibiol}
	\gdef\@journalfull{AI Biology}
	\gdef\@journalshort{AI Biol.}
	\gdef\@doiabbr{aibiol}
	\gdef\@ISSN{3043-2189}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aichem}{%
	\gdef\@journal{aichem}
	\gdef\@journalfull{AI Chemistry}
	\gdef\@journalshort{AI Chem.}
	\gdef\@doiabbr{aichem}
	\gdef\@ISSN{3042-6723}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aieduc}{%
	\gdef\@journal{aieduc}
	\gdef\@journalfull{AI in Education}
	\gdef\@journalshort{AI Educ.}
	\gdef\@doiabbr{aieduc}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{aieng}{%
	\gdef\@journal{aieng}
	\gdef\@journalfull{AI for Engineering}
	\gdef\@journalshort{AI Eng.}
	\gdef\@doiabbr{aieng}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aimater}{%
	\gdef\@journal{aimater}
	\gdef\@journalfull{AI Materials}
	\gdef\@journalshort{AI Mater.}
	\gdef\@doiabbr{aimater}
	\gdef\@ISSN{3042-6715}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aimed}{%
	\gdef\@journal{aimed}
	\gdef\@journalfull{AI in Medicine}
	\gdef\@journalshort{AI Med.}
	\gdef\@doiabbr{aimed}
	\gdef\@ISSN{3042-6707}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aipa}{%
	\gdef\@journal{aipa}
	\gdef\@journalfull{AI and Precision Agriculture}
	\gdef\@journalshort{AI Precis. Agric.}
	\gdef\@doiabbr{aipa}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{air}{%
	\gdef\@journal{air}
	\gdef\@journalfull{Air}
	\gdef\@journalshort{Air}
	\gdef\@doiabbr{air}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aisens}{%
	\gdef\@journal{aisens}
	\gdef\@journalfull{AI Sensors}
	\gdef\@journalshort{AI Sens.}
	\gdef\@doiabbr{aisens}
	\gdef\@ISSN{3042-5999}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aisoc}{%
	\gdef\@journal{aisoc}
	\gdef\@journalfull{AI for Society}
	\gdef\@journalshort{AI Soc.}
	\gdef\@doiabbr{aisoc}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aiua}{%
	\gdef\@journal{aiua}
	\gdef\@journalfull{Archivio Italiano di Urologia e Andrologia}
	\gdef\@journalshort{Arch. Ital. Urol. Androl.}
	\gdef\@doiabbr{aiua}
	\gdef\@ISSN{2282-4197}
	\gdef\@societyowner{Societ\`{a} Italiana di Andrologia, Societ\`{a} Italiana di Ecografia Urologica Nefrologica e Andrologica, Societ\`{a} Italiana di Uro-Oncologia and Urologi Ospedalit\`{a} Gestione Privata}
	\gdef\@journaltype{ACS}}
\DeclareOption{algorithms}{%
	\gdef\@journal{algorithms}
	\gdef\@journalfull{Algorithms}
	\gdef\@journalshort{Algorithms}
	\gdef\@doiabbr{a}
	\gdef\@ISSN{1999-4893}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{allergies}{%
	\gdef\@journal{allergies}
	\gdef\@journalfull{Allergies}
	\gdef\@journalshort{Allergies}
	\gdef\@doiabbr{allergies}
	\gdef\@ISSN{2313-5786}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{alloys}{%
	\gdef\@journal{alloys}
	\gdef\@journalfull{Alloys}
	\gdef\@journalshort{Alloys}
	\gdef\@doiabbr{alloys}
	\gdef\@ISSN{2674-063X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{amh}{%
	\gdef\@journal{amh}
	\gdef\@journalfull{Acta Microbiologica Hellenica}
	\gdef\@journalshort{Acta Microbiol. Hell.}
	\gdef\@doiabbr{amh}
	\gdef\@ISSN{0438-9573}
	\gdef\@societyowner{Hellenic Society for Microbiology}
	\gdef\@journaltype{ACS}}
\DeclareOption{analog}{%
	\gdef\@journal{analog}
	\gdef\@journalfull{Analog}
	\gdef\@journalshort{Analog}
	\gdef\@doiabbr{analog}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{analytica}{%
	\gdef\@journal{analytica}
	\gdef\@journalfull{Analytica}
	\gdef\@journalshort{Analytica}
	\gdef\@doiabbr{analytica}
	\gdef\@ISSN{2673-4532}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{analytics}{%
	\gdef\@journal{analytics}
	\gdef\@journalfull{Analytics}
	\gdef\@journalshort{Analytics}
	\gdef\@doiabbr{analytics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{anatomia}{%
	\gdef\@journal{anatomia}
	\gdef\@journalfull{Anatomia}
	\gdef\@journalshort{Anatomia}
	\gdef\@doiabbr{anatomia}
	\gdef\@ISSN{2813-0545}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{anesthres}{%
	\gdef\@journal{anesthres}
	\gdef\@journalfull{Anesthesia Research}
	\gdef\@journalshort{Anesth. Res.}
	\gdef\@doiabbr{anesthres}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{animals}{%
	\gdef\@journal{animals}
	\gdef\@journalfull{Animals}
	\gdef\@journalshort{Animals}
	\gdef\@doiabbr{ani}
	\gdef\@ISSN{2076-2615}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{antibiotics}{%
	\gdef\@journal{antibiotics}
	\gdef\@journalfull{Antibiotics}
	\gdef\@journalshort{Antibiotics}
	\gdef\@doiabbr{antibiotics}
	\gdef\@ISSN{2079-6382}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{antibodies}{%
	\gdef\@journal{antibodies}
	\gdef\@journalfull{Antibodies}
	\gdef\@journalshort{Antibodies}
	\gdef\@doiabbr{antib}
	\gdef\@ISSN{2073-4468}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{antioxidants}{%
	\gdef\@journal{antioxidants}
	\gdef\@journalfull{Antioxidants}
	\gdef\@journalshort{Antioxidants}
	\gdef\@doiabbr{antiox}
	\gdef\@ISSN{2076-3921}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{apajournal}{%
	\gdef\@journal{apajournal}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{applbiosci}{%
	\gdef\@journal{applbiosci}
	\gdef\@journalfull{Applied Biosciences}
	\gdef\@journalshort{Appl. Biosci.}
	\gdef\@doiabbr{applbiosci}
	\gdef\@ISSN{2813-0464}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{appliedchem}{%
	\gdef\@journal{appliedchem}
	\gdef\@journalfull{AppliedChem}
	\gdef\@journalshort{AppliedChem}
	\gdef\@doiabbr{appliedchem}
	\gdef\@ISSN{2673-9623}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{appliedmath}{%
	\gdef\@journal{appliedmath}
	\gdef\@journalfull{AppliedMath}
	\gdef\@journalshort{AppliedMath}
	\gdef\@doiabbr{appliedmath}
	\gdef\@ISSN{2673-9909}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{appliedphys}{%
	\gdef\@journal{appliedphys}
	\gdef\@journalfull{AppliedPhys}
	\gdef\@journalshort{AppliedPhys}
	\gdef\@doiabbr{appliedphys}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{applmech}{%
	\gdef\@journal{applmech}
	\gdef\@journalfull{Applied Mechanics}
	\gdef\@journalshort{Appl. Mech.}
	\gdef\@doiabbr{applmech}
	\gdef\@ISSN{2673-3161}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{applmicrobiol}{%
	\gdef\@journal{applmicrobiol}
	\gdef\@journalfull{Applied Microbiology}
	\gdef\@journalshort{Appl. Microbiol.}
	\gdef\@doiabbr{applmicrobiol}
	\gdef\@ISSN{2673-8007}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{applnano}{%
	\gdef\@journal{applnano}
	\gdef\@journalfull{Applied Nano}
	\gdef\@journalshort{Appl. Nano}
	\gdef\@doiabbr{applnano}
	\gdef\@ISSN{2673-3501}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{applsci}{%
	\gdef\@journal{applsci}
	\gdef\@journalfull{Applied Sciences}
	\gdef\@journalshort{Appl. Sci.}
	\gdef\@doiabbr{app}
	\gdef\@ISSN{2076-3417}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aps}{%
	\gdef\@journal{aps}
	\gdef\@journalfull{Advanced Petroleum Science}
	\gdef\@journalshort{Adv. Pet. Sci.}
	\gdef\@doiabbr{aps}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{aquacj}{%
	\gdef\@journal{aquacj}
	\gdef\@journalfull{Aquaculture Journal}
	\gdef\@journalshort{Aquac. J.}
	\gdef\@doiabbr{aquacj}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{archaeolstud}{%
	\gdef\@journal{archaeolstud}
	\gdef\@journalfull{Archaeological Studies}
	\gdef\@journalshort{Archaeol. Stud.}
	\gdef\@doiabbr{archaeolstud}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{architecture}{%
	\gdef\@journal{architecture}
	\gdef\@journalfull{Architecture}
	\gdef\@journalshort{Architecture}
	\gdef\@doiabbr{architecture}
	\gdef\@ISSN{2673-8945}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{arm}{%
	\gdef\@journal{arm}
	\gdef\@journalfull{Advances in Respiratory Medicine}
	\gdef\@journalshort{Adv. Respir. Med.}
	\gdef\@doiabbr{arm}
	\gdef\@ISSN{2543-6031}
	\gdef\@societyowner{Polish Respiratory Society}
	\gdef\@journaltype{ACS}}
\DeclareOption{arthropoda}{%
	\gdef\@journal{arthropoda}
	\gdef\@journalfull{Arthropoda}
	\gdef\@journalshort{Arthropoda}
	\gdef\@doiabbr{arthropoda}
	\gdef\@ISSN{2813-3323}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{arts}{%
	\gdef\@journal{arts}
	\gdef\@journalfull{Arts}
	\gdef\@journalshort{Arts}
	\gdef\@doiabbr{arts}
	\gdef\@ISSN{2076-0752}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{asc}{%
	\gdef\@journal{asc}
	\gdef\@journalfull{Automatic Systems and Control}
	\gdef\@journalshort{Autom. Syst. Control}
	\gdef\@doiabbr{asc}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{asd}{%
	\gdef\@journal{asd}
	\gdef\@journalfull{Affective Science and Disorders}
	\gdef\@journalshort{Affect. Sci. Disord.}
	\gdef\@doiabbr{asd}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{asi}{%
	\gdef\@journal{asi}
	\gdef\@journalfull{Applied System Innovation}
	\gdef\@journalshort{Appl. Syst. Innov.}
	\gdef\@doiabbr{asi}
	\gdef\@ISSN{2571-5577}
	\gdef\@societyowner{International Institute of Knowledge Innovation and Invention}
	\gdef\@journaltype{ACS}}
\DeclareOption{astronautics}{%
	\gdef\@journal{astronautics}
	\gdef\@journalfull{Astronautics}
	\gdef\@journalshort{Astronautics}
	\gdef\@doiabbr{astronautics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{astronomy}{%
	\gdef\@journal{astronomy}
	\gdef\@journalfull{Astronomy}
	\gdef\@journalshort{Astronomy}
	\gdef\@doiabbr{astronomy}
	\gdef\@ISSN{2674-0346}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{atmosphere}{%
	\gdef\@journal{atmosphere}
	\gdef\@journalfull{Atmosphere}
	\gdef\@journalshort{Atmosphere}
	\gdef\@doiabbr{atmos}
	\gdef\@ISSN{2073-4433}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{atoms}{%
	\gdef\@journal{atoms}
	\gdef\@journalfull{Atoms}
	\gdef\@journalshort{Atoms}
	\gdef\@doiabbr{atoms}
	\gdef\@ISSN{2218-2004}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{audiolres}{%
	\gdef\@journal{audiolres}
	\gdef\@journalfull{Audiology Research}
	\gdef\@journalshort{Audiol. Res.}
	\gdef\@doiabbr{audiolres}
	\gdef\@ISSN{2039-4349}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{automation}{%
	\gdef\@journal{automation}
	\gdef\@journalfull{Automation}
	\gdef\@journalshort{Automation}
	\gdef\@doiabbr{automation}
	\gdef\@ISSN{2673-4052}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{axioms}{%
	\gdef\@journal{axioms}
	\gdef\@journalfull{Axioms}
	\gdef\@journalshort{Axioms}
	\gdef\@doiabbr{axioms}
	\gdef\@ISSN{2075-1680}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bacteria}{%
	\gdef\@journal{bacteria}
	\gdef\@journalfull{Bacteria}
	\gdef\@journalshort{Bacteria}
	\gdef\@doiabbr{bacteria}
	\gdef\@ISSN{2674-1334}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{batteries}{%
	\gdef\@journal{batteries}
	\gdef\@journalfull{Batteries}
	\gdef\@journalshort{Batteries}
	\gdef\@doiabbr{batteries}
	\gdef\@ISSN{2313-0105}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bcrc}{%
	\gdef\@journal{bcrc}
	\gdef\@journalfull{Breast Cancer Research and Care}
	\gdef\@journalshort{Breast Cancer Res. Care}
	\gdef\@doiabbr{bcrc}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bdcc}{%
	\gdef\@journal{bdcc}
	\gdef\@journalfull{Big Data and Cognitive Computing}
	\gdef\@journalshort{Big Data Cogn. Comput.}
	\gdef\@doiabbr{bdcc}
	\gdef\@ISSN{2504-2289}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{behavsci}{%
	\gdef\@journal{behavsci}
	\gdef\@journalfull{Behavioral Sciences}
	\gdef\@journalshort{Behav. Sci.}
	\gdef\@doiabbr{bs}
	\gdef\@ISSN{2076-328X}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{beverages}{%
	\gdef\@journal{beverages}
	\gdef\@journalfull{Beverages}
	\gdef\@journalshort{Beverages}
	\gdef\@doiabbr{beverages}
	\gdef\@ISSN{2306-5710}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bioactives}{%
	\gdef\@journal{bioactives}
	\gdef\@journalfull{Bioactives}
	\gdef\@journalshort{Bioactives}
	\gdef\@doiabbr{bioactives}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biochem}{%
	\gdef\@journal{biochem}
	\gdef\@journalfull{BioChem}
	\gdef\@journalshort{BioChem}
	\gdef\@doiabbr{biochem}
	\gdef\@ISSN{2673-6411}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bioengineering}{%
	\gdef\@journal{bioengineering}
	\gdef\@journalfull{Bioengineering}
	\gdef\@journalshort{Bioengineering}
	\gdef\@doiabbr{bioengineering}
	\gdef\@ISSN{2306-5354}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biologics}{%
	\gdef\@journal{biologics}
	\gdef\@journalfull{Biologics}
	\gdef\@journalshort{Biologics}
	\gdef\@doiabbr{biologics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biology}{%
	\gdef\@journal{biology}
	\gdef\@journalfull{Biology}
	\gdef\@journalshort{Biology}
	\gdef\@doiabbr{biology}
	\gdef\@ISSN{2079-7737}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biomass}{%
	\gdef\@journal{biomass}
	\gdef\@journalfull{Biomass}
	\gdef\@journalshort{Biomass}
	\gdef\@doiabbr{biomass}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biomechanics}{%
	\gdef\@journal{biomechanics}
	\gdef\@journalfull{Biomechanics}
	\gdef\@journalshort{Biomechanics}
	\gdef\@doiabbr{biomechanics}
	\gdef\@ISSN{2673-7078}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biomed}{%
	\gdef\@journal{biomed}
	\gdef\@journalfull{BioMed}
	\gdef\@journalshort{BioMed}
	\gdef\@doiabbr{biomed}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biomedicines}{%
	\gdef\@journal{biomedicines}
	\gdef\@journalfull{Biomedicines}
	\gdef\@journalshort{Biomedicines}
	\gdef\@doiabbr{biomedicines}
	\gdef\@ISSN{2227-9059}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biomedinformatics}{%
	\gdef\@journal{biomedinformatics}
	\gdef\@journalfull{BioMedInformatics}
	\gdef\@journalshort{BioMedInformatics}
	\gdef\@doiabbr{biomedinformatics}
	\gdef\@ISSN{2673-7426}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biomimetics}{%
	\gdef\@journal{biomimetics}
	\gdef\@journalfull{Biomimetics}
	\gdef\@journalshort{Biomimetics}
	\gdef\@doiabbr{biomimetics}
	\gdef\@ISSN{2313-7673}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biomolecules}{%
	\gdef\@journal{biomolecules}
	\gdef\@journalfull{Biomolecules}
	\gdef\@journalshort{Biomolecules}
	\gdef\@doiabbr{biom}
	\gdef\@ISSN{2218-273X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biophysica}{%
	\gdef\@journal{biophysica}
	\gdef\@journalfull{Biophysica}
	\gdef\@journalshort{Biophysica}
	\gdef\@doiabbr{biophysica}
	\gdef\@ISSN{2673-4125}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bioresourbioprod}{%
	\gdef\@journal{bioresourbioprod}
	\gdef\@journalfull{Bioresources and Bioproducts}
	\gdef\@journalshort{Bioresour. Bioprod.}
	\gdef\@doiabbr{bioresourbioprod}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biosensors}{%
	\gdef\@journal{biosensors}
	\gdef\@journalfull{Biosensors}
	\gdef\@journalshort{Biosensors}
	\gdef\@doiabbr{bios}
	\gdef\@ISSN{2079-6374}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biosphere}{%
	\gdef\@journal{biosphere}
	\gdef\@journalfull{Biosphere}
	\gdef\@journalshort{Biosphere}
	\gdef\@doiabbr{biosphere}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{biotech}{%
	\gdef\@journal{biotech}
	\gdef\@journalfull{BioTech}
	\gdef\@journalshort{BioTech}
	\gdef\@doiabbr{biotech}
	\gdef\@ISSN{2673-6284}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{birds}{%
	\gdef\@journal{birds}
	\gdef\@journalfull{Birds}
	\gdef\@journalshort{Birds}
	\gdef\@doiabbr{birds}
	\gdef\@ISSN{2673-6004}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{blockchains}{%
	\gdef\@journal{blockchains}
	\gdef\@journalfull{Blockchains}
	\gdef\@journalshort{Blockchains}
	\gdef\@doiabbr{blockchains}
	\gdef\@ISSN{2813-5288}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bloods}{%
	\gdef\@journal{bloods}
	\gdef\@journalfull{Bloods}
	\gdef\@journalshort{Bloods}
	\gdef\@doiabbr{bloods}
	\gdef\@ISSN{2673-415X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{blsf}{%
	\gdef\@journal{blsf}
	\gdef\@journalfull{Biology and Life Sciences Forum}
	\gdef\@journalshort{Biol. Life Sci. Forum}
	\gdef\@doiabbr{blsf}
	\gdef\@ISSN{2673-9976}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{brainsci}{%
	\gdef\@journal{brainsci}
	\gdef\@journalfull{Brain Sciences}
	\gdef\@journalshort{Brain Sci.}
	\gdef\@doiabbr{brainsci}
	\gdef\@ISSN{2076-3425}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{breath}{%
	\gdef\@journal{breath}
	\gdef\@journalfull{Breath}
	\gdef\@journalshort{Breath}
	\gdef\@doiabbr{breath}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{bse}{%
	\gdef\@journal{bse}
	\gdef\@journalfull{Biomedical Science and Engineering}
	\gdef\@journalshort{Biomed. Sci. Eng.}
	\gdef\@doiabbr{bse}
	\gdef\@ISSN{2531-9892}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{buildings}{%
	\gdef\@journal{buildings}
	\gdef\@journalfull{Buildings}
	\gdef\@journalshort{Buildings}
	\gdef\@doiabbr{buildings}
	\gdef\@ISSN{2075-5309}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{businesses}{%
	\gdef\@journal{businesses}
	\gdef\@journalfull{Businesses}
	\gdef\@journalshort{Businesses}
	\gdef\@doiabbr{businesses}
	\gdef\@ISSN{2673-7116}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{cancers}{%
	\gdef\@journal{cancers}
	\gdef\@journalfull{Cancers}
	\gdef\@journalshort{Cancers}
	\gdef\@doiabbr{cancers}
	\gdef\@ISSN{2072-6694}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{carbon}{%
	\gdef\@journal{carbon}
	\gdef\@journalfull{C}
	\gdef\@journalshort{C}
	\gdef\@doiabbr{c}
	\gdef\@ISSN{2311-5629}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cardio}{%
	\gdef\@journal{cardio}
	\gdef\@journalfull{Cardio}
	\gdef\@journalshort{Cardio}
	\gdef\@doiabbr{cardio}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cardiogenetics}{%
	\gdef\@journal{cardiogenetics}
	\gdef\@journalfull{Cardiogenetics}
	\gdef\@journalshort{Cardiogenetics}
	\gdef\@doiabbr{cardiogenetics}
	\gdef\@ISSN{2035-8148}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cardiovascmed}{%
	\gdef\@journal{cardiovascmed}
	\gdef\@journalfull{Cardiovascular Medicine}
	\gdef\@journalshort{Cardiovasc. Med.}
	\gdef\@doiabbr{cardiovascmed}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{catalogs}{%
	\gdef\@journal{catalogs}
	\gdef\@journalfull{Catalogs}
	\gdef\@journalshort{Catalogs}
	\gdef\@doiabbr{catalogs}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{catalysts}{%
	\gdef\@journal{catalysts}
	\gdef\@journalfull{Catalysts}
	\gdef\@journalshort{Catalysts}
	\gdef\@doiabbr{catal}
	\gdef\@ISSN{2073-4344}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cdr}{%
	\gdef\@journal{cdr}
	\gdef\@journalfull{Chest Disease Reports}
	\gdef\@journalshort{Chest Dis. Rep.}
	\gdef\@doiabbr{cdr}
	\gdef\@ISSN{2039-4772}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cells}{%
	\gdef\@journal{cells}
	\gdef\@journalfull{Cells}
	\gdef\@journalshort{Cells}
	\gdef\@doiabbr{cells}
	\gdef\@ISSN{2073-4409}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ceramics}{%
	\gdef\@journal{ceramics}
	\gdef\@journalfull{Ceramics}
	\gdef\@journalshort{Ceramics}
	\gdef\@doiabbr{ceramics}
	\gdef\@ISSN{2571-6131}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{challenges}{%
	\gdef\@journal{challenges}
	\gdef\@journalfull{Challenges---Journal of Planetary Health}
	\gdef\@journalshort{Challenges}
	\gdef\@doiabbr{challe}
	\gdef\@ISSN{2078-1547}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{chemeco}{%
	\gdef\@journal{chemeco}
	\gdef\@journalfull{ChemEco}
	\gdef\@journalshort{ChemEco}
	\gdef\@doiabbr{chemeco}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{chemengineering}{%
	\gdef\@journal{chemengineering}
	\gdef\@journalfull{ChemEngineering}
	\gdef\@journalshort{ChemEngineering}
	\gdef\@doiabbr{chemengineering}
	\gdef\@ISSN{2305-7084}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{chemistry}{%
	\gdef\@journal{chemistry}
	\gdef\@journalfull{Chemistry}
	\gdef\@journalshort{Chemistry}
	\gdef\@doiabbr{chemistry}
	\gdef\@ISSN{2624-8549}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{chemosensors}{%
	\gdef\@journal{chemosensors}
	\gdef\@journalfull{Chemosensors}
	\gdef\@journalshort{Chemosensors}
	\gdef\@doiabbr{chemosensors}
	\gdef\@ISSN{2227-9040}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{chemproc}{%
	\gdef\@journal{chemproc}
	\gdef\@journalfull{Chemistry Proceedings}
	\gdef\@journalshort{Chem. Proc.}
	\gdef\@doiabbr{chemproc}
	\gdef\@ISSN{2673-4583}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{chicagojournal}{%
	\gdef\@journal{chicagojournal}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{children}{%
	\gdef\@journal{children}
	\gdef\@journalfull{Children}
	\gdef\@journalshort{Children}
	\gdef\@doiabbr{children}
	\gdef\@ISSN{2227-9067}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{chips}{%
	\gdef\@journal{chips}
	\gdef\@journalfull{Chips}
	\gdef\@journalshort{Chips}
	\gdef\@doiabbr{chips}
	\gdef\@ISSN{2674-0729}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cimb}{%
	\gdef\@journal{cimb}
	\gdef\@journalfull{Current Issues in Molecular Biology}
	\gdef\@journalshort{Curr. Issues Mol. Biol.}
	\gdef\@doiabbr{cimb}
	\gdef\@ISSN{1467-3045}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{civileng}{%
	\gdef\@journal{civileng}
	\gdef\@journalfull{CivilEng}
	\gdef\@journalshort{CivilEng}
	\gdef\@doiabbr{civileng}
	\gdef\@ISSN{2673-4109}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cleantechnol}{%
	\gdef\@journal{cleantechnol}
	\gdef\@journalfull{Clean Technologies}
	\gdef\@journalshort{Clean Technol.}
	\gdef\@doiabbr{cleantechnol}
	\gdef\@ISSN{2571-8797}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{climate}{%
	\gdef\@journal{climate}
	\gdef\@journalfull{Climate}
	\gdef\@journalshort{Climate}
	\gdef\@doiabbr{cli}
	\gdef\@ISSN{2225-1154}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{clinbioenerg}{%
	\gdef\@journal{clinbioenerg}
	\gdef\@journalfull{Clinical Bioenergetics}
	\gdef\@journalshort{Clin. Bioenerg.}
	\gdef\@doiabbr{clinbioenerg}
	\gdef\@ISSN{3042-5158}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{clinpract}{%
	\gdef\@journal{clinpract}
	\gdef\@journalfull{Clinics and Practice}
	\gdef\@journalshort{Clin. Pract.}
	\gdef\@doiabbr{clinpract}
	\gdef\@ISSN{2039-7283}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{clockssleep}{%
	\gdef\@journal{clockssleep}
	\gdef\@journalfull{Clocks \& Sleep}
	\gdef\@journalshort{Clocks\&Sleep}
	\gdef\@doiabbr{clockssleep}
	\gdef\@ISSN{2624-5175}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cmd}{%
	\gdef\@journal{cmd}
	\gdef\@journalfull{Corrosion and Materials Degradation}
	\gdef\@journalshort{Corros. Mater. Degrad.}
	\gdef\@doiabbr{cmd}
	\gdef\@ISSN{2624-5558}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cmtr}{%
	\gdef\@journal{cmtr}
	\gdef\@journalfull{Craniomaxillofacial Trauma \& Reconstruction}
	\gdef\@journalshort{Craniomaxillofac. Trauma Reconstr.}
	\gdef\@doiabbr{cmtr}
	\gdef\@ISSN{1943-3883}
	\gdef\@societyowner{AO Foundation}
	\gdef\@journaltype{ACS}}
\DeclareOption{coasts}{%
	\gdef\@journal{coasts}
	\gdef\@journalfull{Coasts}
	\gdef\@journalshort{Coasts}
	\gdef\@doiabbr{coasts}
	\gdef\@ISSN{2673-964X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{coatings}{%
	\gdef\@journal{coatings}
	\gdef\@journalfull{Coatings}
	\gdef\@journalshort{Coatings}
	\gdef\@doiabbr{coatings}
	\gdef\@ISSN{2079-6412}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{colloids}{%
	\gdef\@journal{colloids}
	\gdef\@journalfull{Colloids and Interfaces}
	\gdef\@journalshort{Colloids Interfaces}
	\gdef\@doiabbr{colloids}
	\gdef\@ISSN{2504-5377}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{colorants}{%
	\gdef\@journal{colorants}
	\gdef\@journalfull{Colorants}
	\gdef\@journalshort{Colorants}
	\gdef\@doiabbr{colorants}
	\gdef\@ISSN{2079-6447}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{commodities}{%
	\gdef\@journal{commodities}
	\gdef\@journalfull{Commodities}
	\gdef\@journalshort{Commodities}
	\gdef\@doiabbr{commodities}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{complexities}{%
	\gdef\@journal{complexities}
	\gdef\@journalfull{Complexities}
	\gdef\@journalshort{Complexities}
	\gdef\@doiabbr{complexities}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{complications}{%
	\gdef\@journal{complications}
	\gdef\@journalfull{Complications}
	\gdef\@journalshort{Complications}
	\gdef\@doiabbr{complications}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{compounds}{%
	\gdef\@journal{compounds}
	\gdef\@journalfull{Compounds}
	\gdef\@journalshort{Compounds}
	\gdef\@doiabbr{compounds}
	\gdef\@ISSN{2673-6918}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{computation}{%
	\gdef\@journal{computation}
	\gdef\@journalfull{Computation}
	\gdef\@journalshort{Computation}
	\gdef\@doiabbr{computation}
	\gdef\@ISSN{2079-3197}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{computers}{%
	\gdef\@journal{computers}
	\gdef\@journalfull{Computers}
	\gdef\@journalshort{Computers}
	\gdef\@doiabbr{computers}
	\gdef\@ISSN{2073-431X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{condensedmatter}{%
	\gdef\@journal{condensedmatter}
	\gdef\@journalfull{Condensed Matter}
	\gdef\@journalshort{Condens. Matter}
	\gdef\@doiabbr{condmat}
	\gdef\@ISSN{2410-3896}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{conservation}{%
	\gdef\@journal{conservation}
	\gdef\@journalfull{Conservation}
	\gdef\@journalshort{Conservation}
	\gdef\@doiabbr{conservation}
	\gdef\@ISSN{2673-7159}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{constrmater}{%
	\gdef\@journal{constrmater}
	\gdef\@journalfull{Construction Materials}
	\gdef\@journalshort{Constr. Mater.}
	\gdef\@doiabbr{constrmater}
	\gdef\@ISSN{2673-7108}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cosmetics}{%
	\gdef\@journal{cosmetics}
	\gdef\@journalfull{Cosmetics}
	\gdef\@journalshort{Cosmetics}
	\gdef\@doiabbr{cosmetics}
	\gdef\@ISSN{2079-9284}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{covid}{%
	\gdef\@journal{covid}
	\gdef\@journalfull{COVID}
	\gdef\@journalshort{COVID}
	\gdef\@doiabbr{covid}
	\gdef\@ISSN{2673-8112}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{crops}{%
	\gdef\@journal{crops}
	\gdef\@journalfull{Crops}
	\gdef\@journalshort{Crops}
	\gdef\@doiabbr{crops}
	\gdef\@ISSN{2673-7655}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cryo}{%
	\gdef\@journal{cryo}
	\gdef\@journalfull{Cryo}
	\gdef\@journalshort{Cryo}
	\gdef\@doiabbr{cryo}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cryptography}{%
	\gdef\@journal{cryptography}
	\gdef\@journalfull{Cryptography}
	\gdef\@journalshort{Cryptography}
	\gdef\@doiabbr{cryptography}
	\gdef\@ISSN{2410-387X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{crystals}{%
	\gdef\@journal{crystals}
	\gdef\@journalfull{Crystals}
	\gdef\@journalshort{Crystals}
	\gdef\@doiabbr{cryst}
	\gdef\@ISSN{2073-4352}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{csmf}{%
	\gdef\@journal{csmf}
	\gdef\@journalfull{Computer Sciences \& Mathematics Forum}
	\gdef\@journalshort{Comput. Sci. Math. Forum}
	\gdef\@doiabbr{csmf}
	\gdef\@ISSN{2813-0324}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ctn}{%
	\gdef\@journal{ctn}
	\gdef\@journalfull{Clinical and Translational Neuroscience}
	\gdef\@journalshort{Clin. Transl. Neurosci.}
	\gdef\@doiabbr{ctn}
	\gdef\@ISSN{2514-183X}
	\gdef\@societyowner{Swiss Federation of Clinical Neuro-Societies}
	\gdef\@journaltype{ACS}}
\DeclareOption{culture}{%
	\gdef\@journal{culture}
	\gdef\@journalfull{Culture}
	\gdef\@journalshort{Culture}
	\gdef\@doiabbr{culture}
	\gdef\@ISSN{3042-8165}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{curroncol}{%
	\gdef\@journal{curroncol}
	\gdef\@journalfull{Current Oncology}
	\gdef\@journalshort{Curr. Oncol.}
	\gdef\@doiabbr{curroncol}
	\gdef\@ISSN{1718-7729}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{cyber}{%
	\gdef\@journal{cyber}
	\gdef\@journalfull{Cyber}
	\gdef\@journalshort{Cyber}
	\gdef\@doiabbr{cyber}
	\gdef\@ISSN{2624-800X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dairy}{%
	\gdef\@journal{dairy}
	\gdef\@journalfull{Dairy}
	\gdef\@journalshort{Dairy}
	\gdef\@doiabbr{dairy}
	\gdef\@ISSN{2624-862X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{data}{%
	\gdef\@journal{data}
	\gdef\@journalfull{Data}
	\gdef\@journalshort{Data}
	\gdef\@doiabbr{data}
	\gdef\@ISSN{2306-5729}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ddc}{%
	\gdef\@journal{ddc}
	\gdef\@journalfull{Drugs and Drug Candidates}
	\gdef\@journalshort{Drugs Drug Candidates}
	\gdef\@doiabbr{ddc}
	\gdef\@ISSN{2813-2998}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dentistry}{%
	\gdef\@journal{dentistry}
	\gdef\@journalfull{Dentistry Journal}
	\gdef\@journalshort{Dent. J.}
	\gdef\@doiabbr{dj}
	\gdef\@ISSN{2304-6767}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dermato}{%
	\gdef\@journal{dermato}
	\gdef\@journalfull{Dermato}
	\gdef\@journalshort{Dermato}
	\gdef\@doiabbr{dermato}
	\gdef\@ISSN{2673-6179}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dermatopathology}{%
	\gdef\@journal{dermatopathology}
	\gdef\@journalfull{Dermatopathology}
	\gdef\@journalshort{Dermatopathology}
	\gdef\@doiabbr{dermatopathology}
	\gdef\@ISSN{2296-3529}
	\gdef\@societyowner{European Society of Dermatopathology}
	\gdef\@journaltype{ACS}}
\DeclareOption{designs}{%
	\gdef\@journal{designs}
	\gdef\@journalfull{Designs}
	\gdef\@journalshort{Designs}
	\gdef\@doiabbr{designs}
	\gdef\@ISSN{2411-9660}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{devices}{%
	\gdef\@journal{devices}
	\gdef\@journalfull{Devices}
	\gdef\@journalshort{Devices}
	\gdef\@doiabbr{devices}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dgg}{%
	\gdef\@journal{dgg}
	\gdef\@journalfull{Digital Games and Gaming}
	\gdef\@journalshort{Digit. Games Gaming}
	\gdef\@doiabbr{dgg}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dhi}{%
	\gdef\@journal{dhi}
	\gdef\@journalfull{Digital Health and Innovation}
	\gdef\@journalshort{Digit. Health Innov.}
	\gdef\@doiabbr{dhi}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{diabetology}{%
	\gdef\@journal{diabetology}
	\gdef\@journalfull{Diabetology}
	\gdef\@journalshort{Diabetology}
	\gdef\@doiabbr{diabetology}
	\gdef\@ISSN{2673-4540}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{diagnostics}{%
	\gdef\@journal{diagnostics}
	\gdef\@journalfull{Diagnostics}
	\gdef\@journalshort{Diagnostics}
	\gdef\@doiabbr{diagnostics}
	\gdef\@ISSN{2075-4418}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dietetics}{%
	\gdef\@journal{dietetics}
	\gdef\@journalfull{Dietetics}
	\gdef\@journalshort{Dietetics}
	\gdef\@doiabbr{dietetics}
	\gdef\@ISSN{2674-0311}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{digital}{%
	\gdef\@journal{digital}
	\gdef\@journalfull{Digital}
	\gdef\@journalshort{Digital}
	\gdef\@doiabbr{digital}
	\gdef\@ISSN{2673-6470}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{disabilities}{%
	\gdef\@journal{disabilities}
	\gdef\@journalfull{Disabilities}
	\gdef\@journalshort{Disabilities}
	\gdef\@doiabbr{disabilities}
	\gdef\@ISSN{2673-7272}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{diseases}{%
	\gdef\@journal{diseases}
	\gdef\@journalfull{Diseases}
	\gdef\@journalshort{Diseases}
	\gdef\@doiabbr{diseases}
	\gdef\@ISSN{2079-9721}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{diversity}{%
	\gdef\@journal{diversity}
	\gdef\@journalfull{Diversity}
	\gdef\@journalshort{Diversity}
	\gdef\@doiabbr{d}
	\gdef\@ISSN{1424-2818}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dna}{%
	\gdef\@journal{dna}
	\gdef\@journalfull{DNA}
	\gdef\@journalshort{DNA}
	\gdef\@doiabbr{dna}
	\gdef\@ISSN{2673-8856}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{drones}{%
	\gdef\@journal{drones}
	\gdef\@journalfull{Drones}
	\gdef\@journalshort{Drones}
	\gdef\@doiabbr{drones}
	\gdef\@ISSN{2504-446X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{drugreact}{%
	\gdef\@journal{drugreact}
	\gdef\@journalfull{Drug Reactions}
	\gdef\@journalshort{Drug React.}
	\gdef\@doiabbr{drugreact}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{drylandsci}{%
	\gdef\@journal{drylandsci}
	\gdef\@journalfull{Dryland Science}
	\gdef\@journalshort{Dryland Sci.}
	\gdef\@doiabbr{drylandsci}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{dynamics}{%
	\gdef\@journal{dynamics}
	\gdef\@journalfull{Dynamics}
	\gdef\@journalshort{Dynamics}
	\gdef\@doiabbr{dynamics}
	\gdef\@ISSN{2673-8716}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{earth}{%
	\gdef\@journal{earth}
	\gdef\@journalfull{Earth}
	\gdef\@journalshort{Earth}
	\gdef\@doiabbr{earth}
	\gdef\@ISSN{2673-4834}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ebj}{%
	\gdef\@journal{ebj}
	\gdef\@journalfull{European Burn Journal}
	\gdef\@journalshort{Eur. Burn J.}
	\gdef\@doiabbr{ebj}
	\gdef\@ISSN{2673-1991}
	\gdef\@societyowner{European Burns Association}
	\gdef\@journaltype{ACS}}
\DeclareOption{ece}{%
	\gdef\@journal{ece}
	\gdef\@journalfull{Environmental Chemical Engineering}
	\gdef\@journalshort{Environ. Chem. Eng.}
	\gdef\@doiabbr{ece}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ecm}{%
	\gdef\@journal{ecm}
	\gdef\@journalfull{Emergency Care and Medicine}
	\gdef\@journalshort{Emerg. Care Med.}
	\gdef\@doiabbr{ecm}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{eco-environsci}{%
	\gdef\@journal{eco-environsci}
	\gdef\@journalfull{Eco-Environmental Sciences}
	\gdef\@journalshort{Eco-Environ. Sci.}
	\gdef\@doiabbr{eco-environsci}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ecologies}{%
	\gdef\@journal{ecologies}
	\gdef\@journalfull{Ecologies}
	\gdef\@journalshort{Ecologies}
	\gdef\@doiabbr{ecologies}
	\gdef\@ISSN{2673-4133}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{econometrics}{%
	\gdef\@journal{econometrics}
	\gdef\@journalfull{Econometrics}
	\gdef\@journalshort{Econometrics}
	\gdef\@doiabbr{econometrics}
	\gdef\@ISSN{2225-1146}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{economies}{%
	\gdef\@journal{economies}
	\gdef\@journalfull{Economies}
	\gdef\@journalshort{Economies}
	\gdef\@doiabbr{economies}
	\gdef\@ISSN{2227-7099}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{edm}{%
	\gdef\@journal{edm}
	\gdef\@journalfull{Entropic and Disordered Matter}
	\gdef\@journalshort{Entropic Disord. Matter}
	\gdef\@doiabbr{edm}
	\gdef\@ISSN{3042-7592}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{education}{%
	\gdef\@journal{education}
	\gdef\@journalfull{Education Sciences}
	\gdef\@journalshort{Educ. Sci.}
	\gdef\@doiabbr{educsci}
	\gdef\@ISSN{2227-7102}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{eesp}{%
	\gdef\@journal{eesp}
	\gdef\@journalfull{Environmental and Earth Sciences Proceedings}
	\gdef\@journalshort{Environ. Earth Sci. Proc.}
	\gdef\@doiabbr{eesp}
	\gdef\@ISSN{3042-5743}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ejihpe}{%
	\gdef\@journal{ejihpe}
	\gdef\@journalfull{European Journal of Investigation in Health, Psychology and Education}
	\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}
	\gdef\@doiabbr{ejihpe}
	\gdef\@ISSN{2254-9625}
	\gdef\@societyowner{Spanish Scientific Society for Research and Training in Health Sciences}
	\gdef\@journaltype{APA}}
\DeclareOption{electricity}{%
	\gdef\@journal{electricity}
	\gdef\@journalfull{Electricity}
	\gdef\@journalshort{Electricity}
	\gdef\@doiabbr{electricity}
	\gdef\@ISSN{2673-4826}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{electrochem}{%
	\gdef\@journal{electrochem}
	\gdef\@journalfull{Electrochem}
	\gdef\@journalshort{Electrochem}
	\gdef\@doiabbr{electrochem}
	\gdef\@ISSN{2673-3293}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{electronicmat}{%
	\gdef\@journal{electronicmat}
	\gdef\@journalfull{Electronic Materials}
	\gdef\@journalshort{Electron. Mater.}
	\gdef\@doiabbr{electronicmat}
	\gdef\@ISSN{2673-3978}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{electronics}{%
	\gdef\@journal{electronics}
	\gdef\@journalfull{Electronics}
	\gdef\@journalshort{Electronics}
	\gdef\@doiabbr{electronics}
	\gdef\@ISSN{2079-9292}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{embodiedintell}{%
	\gdef\@journal{embodiedintell}
	\gdef\@journalfull{Embodied Intelligence}
	\gdef\@journalshort{Embodied Intell.}
	\gdef\@doiabbr{embodiedintell}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{encyclopedia}{%
	\gdef\@journal{encyclopedia}
	\gdef\@journalfull{Encyclopedia}
	\gdef\@journalshort{Encyclopedia}
	\gdef\@doiabbr{encyclopedia}
	\gdef\@ISSN{2673-8392}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{endocrines}{%
	\gdef\@journal{endocrines}
	\gdef\@journalfull{Endocrines}
	\gdef\@journalshort{Endocrines}
	\gdef\@doiabbr{endocrines}
	\gdef\@ISSN{2673-396X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{energies}{%
	\gdef\@journal{energies}
	\gdef\@journalfull{Energies}
	\gdef\@journalshort{Energies}
	\gdef\@doiabbr{en}
	\gdef\@ISSN{1996-1073}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{eng}{%
	\gdef\@journal{eng}
	\gdef\@journalfull{Eng}
	\gdef\@journalshort{Eng}
	\gdef\@doiabbr{eng}
	\gdef\@ISSN{2673-4117}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{engproc}{%
	\gdef\@journal{engproc}
	\gdef\@journalfull{Engineering Proceedings}
	\gdef\@journalshort{Eng. Proc.}
	\gdef\@doiabbr{engproc}
	\gdef\@ISSN{2673-4591}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{entomology}{%
	\gdef\@journal{entomology}
	\gdef\@journalfull{Entomology}
	\gdef\@journalshort{Entomology}
	\gdef\@doiabbr{entomology}
	\gdef\@ISSN{2813-0502}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{entropy}{%
	\gdef\@journal{entropy}
	\gdef\@journalfull{Entropy}
	\gdef\@journalshort{Entropy}
	\gdef\@doiabbr{e}
	\gdef\@ISSN{1099-4300}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{environments}{%
	\gdef\@journal{environments}
	\gdef\@journalfull{Environments}
	\gdef\@journalshort{Environments}
	\gdef\@doiabbr{environments}
	\gdef\@ISSN{2076-3298}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{environremediat}{%
	\gdef\@journal{environremediat}
	\gdef\@journalfull{Environmental Remediation}
	\gdef\@journalshort{Environ. Remediat.}
	\gdef\@doiabbr{environremediat}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{enzymology}{%
	\gdef\@journal{enzymology}
	\gdef\@journalfull{Enzymology}
	\gdef\@journalshort{Enzymology}
	\gdef\@doiabbr{enzymology}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{epidemiologia}{%
	\gdef\@journal{epidemiologia}
	\gdef\@journalfull{Epidemiologia}
	\gdef\@journalshort{Epidemiologia}
	\gdef\@doiabbr{epidemiologia}
	\gdef\@ISSN{2673-3986}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{epigenomes}{%
	\gdef\@journal{epigenomes}
	\gdef\@journalfull{Epigenomes}
	\gdef\@journalshort{Epigenomes}
	\gdef\@doiabbr{epigenomes}
	\gdef\@ISSN{2075-4655}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{epilepsy}{%
	\gdef\@journal{epilepsy}
	\gdef\@journalfull{Epilepsy}
	\gdef\@journalshort{Epilepsy}
	\gdef\@doiabbr{epilepsy}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{esa}{%
	\gdef\@journal{esa}
	\gdef\@journalfull{Energy Storage and Applications}
	\gdef\@journalshort{Energy Storage Appl.}
	\gdef\@doiabbr{esa}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{est}{%
	\gdef\@journal{est}
	\gdef\@journalfull{Electrochemical Science and Technology}
	\gdef\@journalshort{Electrochem. Sci. Technol.}
	\gdef\@doiabbr{est}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{famsci}{%
	\gdef\@journal{famsci}
	\gdef\@journalfull{Family Sciences}
	\gdef\@journalshort{Fam. Sci.}
	\gdef\@doiabbr{famsci}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{fclam}{%
	\gdef\@journal{fclam}
	\gdef\@journalfull{Future Collections, Libraries, Archives, and Museums}
	\gdef\@journalshort{Future Collect. Libr. Arch. Mus.}
	\gdef\@doiabbr{fclam}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{fermentation}{%
	\gdef\@journal{fermentation}
	\gdef\@journalfull{Fermentation}
	\gdef\@journalshort{Fermentation}
	\gdef\@doiabbr{fermentation}
	\gdef\@ISSN{2311-5637}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fibers}{%
	\gdef\@journal{fibers}
	\gdef\@journalfull{Fibers}
	\gdef\@journalshort{Fibers}
	\gdef\@doiabbr{fib}
	\gdef\@ISSN{2079-6439}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fintech}{%
	\gdef\@journal{fintech}
	\gdef\@journalfull{FinTech}
	\gdef\@journalshort{FinTech}
	\gdef\@doiabbr{fintech}
	\gdef\@ISSN{2674-1032}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fire}{%
	\gdef\@journal{fire}
	\gdef\@journalfull{Fire}
	\gdef\@journalshort{Fire}
	\gdef\@doiabbr{fire}
	\gdef\@ISSN{2571-6255}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fishes}{%
	\gdef\@journal{fishes}
	\gdef\@journalfull{Fishes}
	\gdef\@journalshort{Fishes}
	\gdef\@doiabbr{fishes}
	\gdef\@ISSN{2410-3888}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fluids}{%
	\gdef\@journal{fluids}
	\gdef\@journalfull{Fluids}
	\gdef\@journalshort{Fluids}
	\gdef\@doiabbr{fluids}
	\gdef\@ISSN{2311-5521}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{foodeng}{%
	\gdef\@journal{foodeng}
	\gdef\@journalfull{Food Engineering}
	\gdef\@journalshort{Food Eng.}
	\gdef\@doiabbr{foodeng}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{foods}{%
	\gdef\@journal{foods}
	\gdef\@journalfull{Foods}
	\gdef\@journalshort{Foods}
	\gdef\@doiabbr{foods}
	\gdef\@ISSN{2304-8158}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{forecasting}{%
	\gdef\@journal{forecasting}
	\gdef\@journalfull{Forecasting}
	\gdef\@journalshort{Forecasting}
	\gdef\@doiabbr{forecast}
	\gdef\@ISSN{2571-9394}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{forensicsci}{%
	\gdef\@journal{forensicsci}
	\gdef\@journalfull{Forensic Sciences}
	\gdef\@journalshort{Forensic Sci.}
	\gdef\@doiabbr{forensicsci}
	\gdef\@ISSN{2673-6756}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{forests}{%
	\gdef\@journal{forests}
	\gdef\@journalfull{Forests}
	\gdef\@journalshort{Forests}
	\gdef\@doiabbr{f}
	\gdef\@ISSN{1999-4907}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fossstud}{%
	\gdef\@journal{fossstud}
	\gdef\@journalfull{Fossil Studies}
	\gdef\@journalshort{Foss. Stud.}
	\gdef\@doiabbr{fossils}
	\gdef\@ISSN{2813-6284}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{foundations}{%
	\gdef\@journal{foundations}
	\gdef\@journalfull{Foundations}
	\gdef\@journalshort{Foundations}
	\gdef\@doiabbr{foundations}
	\gdef\@ISSN{2673-9321}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fractalfract}{%
	\gdef\@journal{fractalfract}
	\gdef\@journalfull{Fractal and Fractional}
	\gdef\@journalshort{Fractal Fract.}
	\gdef\@doiabbr{fractalfract}
	\gdef\@ISSN{2504-3110}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{freshwater}{%
	\gdef\@journal{freshwater}
	\gdef\@journalfull{Freshwater}
	\gdef\@journalshort{Freshwater}
	\gdef\@doiabbr{freshwater}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{fuels}{%
	\gdef\@journal{fuels}
	\gdef\@journalfull{Fuels}
	\gdef\@journalshort{Fuels}
	\gdef\@doiabbr{fuels}
	\gdef\@ISSN{2673-3994}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{future}{%
	\gdef\@journal{future}
	\gdef\@journalfull{Future}
	\gdef\@journalshort{Future}
	\gdef\@doiabbr{future}
	\gdef\@ISSN{2813-2882}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{futureinternet}{%
	\gdef\@journal{futureinternet}
	\gdef\@journalfull{Future Internet}
	\gdef\@journalshort{Future Internet}
	\gdef\@doiabbr{fi}
	\gdef\@ISSN{1999-5903}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{futurepharmacol}{%
	\gdef\@journal{futurepharmacol}
	\gdef\@journalfull{Future Pharmacology}
	\gdef\@journalshort{Future Pharmacol.}
	\gdef\@doiabbr{futurepharmacol}
	\gdef\@ISSN{2673-9879}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{futurephys}{%
	\gdef\@journal{futurephys}
	\gdef\@journalfull{Future Physics}
	\gdef\@journalshort{Future Phys.}
	\gdef\@doiabbr{futurephys}
	\gdef\@ISSN{2624-6503}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{futuretransp}{%
	\gdef\@journal{futuretransp}
	\gdef\@journalfull{Future Transportation}
	\gdef\@journalshort{Future Transp.}
	\gdef\@doiabbr{futuretransp}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{galaxies}{%
	\gdef\@journal{galaxies}
	\gdef\@journalfull{Galaxies}
	\gdef\@journalshort{Galaxies}
	\gdef\@doiabbr{galaxies}
	\gdef\@ISSN{2075-4434}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{games}{%
	\gdef\@journal{games}
	\gdef\@journalfull{Games}
	\gdef\@journalshort{Games}
	\gdef\@doiabbr{g}
	\gdef\@ISSN{2073-4336}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{gases}{%
	\gdef\@journal{gases}
	\gdef\@journalfull{Gases}
	\gdef\@journalshort{Gases}
	\gdef\@doiabbr{gases}
	\gdef\@ISSN{2673-5628}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{gastroent}{%
	\gdef\@journal{gastroent}
	\gdef\@journalfull{Gastroenterology Insights}
	\gdef\@journalshort{Gastroenterol. Insights}
	\gdef\@doiabbr{gastroent}
	\gdef\@ISSN{2036-7422}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{gastrointestdisord}{%
	\gdef\@journal{gastrointestdisord}
	\gdef\@journalfull{Gastrointestinal Disorders}
	\gdef\@journalshort{Gastrointest. Disord.}
	\gdef\@doiabbr{gidisord}
	\gdef\@ISSN{2624-5647}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{gastronomy}{%
	\gdef\@journal{gastronomy}
	\gdef\@journalfull{Gastronomy}
	\gdef\@journalshort{Gastronomy}
	\gdef\@doiabbr{gastronomy}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{gels}{%
	\gdef\@journal{gels}
	\gdef\@journalfull{Gels}
	\gdef\@journalshort{Gels}
	\gdef\@doiabbr{gels}
	\gdef\@ISSN{2310-2861}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{genealogy}{%
	\gdef\@journal{genealogy}
	\gdef\@journalfull{Genealogy}
	\gdef\@journalshort{Genealogy}
	\gdef\@doiabbr{genealogy}
	\gdef\@ISSN{2313-5778}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{genes}{%
	\gdef\@journal{genes}
	\gdef\@journalfull{Genes}
	\gdef\@journalshort{Genes}
	\gdef\@doiabbr{genes}
	\gdef\@ISSN{2073-4425}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geochem}{%
	\gdef\@journal{geochem}
	\gdef\@journalfull{GeoChem}
	\gdef\@journalshort{GeoChem}
	\gdef\@doiabbr{geochem}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geographies}{%
	\gdef\@journal{geographies}
	\gdef\@journalfull{Geographies}
	\gdef\@journalshort{Geographies}
	\gdef\@doiabbr{geographies}
	\gdef\@ISSN{2673-7086}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geohazards}{%
	\gdef\@journal{geohazards}
	\gdef\@journalfull{GeoHazards}
	\gdef\@journalshort{GeoHazards}
	\gdef\@doiabbr{geohazards}
	\gdef\@ISSN{2624-795X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geomatics}{%
	\gdef\@journal{geomatics}
	\gdef\@journalfull{Geomatics}
	\gdef\@journalshort{Geomatics}
	\gdef\@doiabbr{geomatics}
	\gdef\@ISSN{2673-7418}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geometry}{%
	\gdef\@journal{geometry}
	\gdef\@journalfull{Geometry}
	\gdef\@journalshort{Geometry}
	\gdef\@doiabbr{geometry}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geosciences}{%
	\gdef\@journal{geosciences}
	\gdef\@journalfull{Geosciences}
	\gdef\@journalshort{Geosciences}
	\gdef\@doiabbr{geosciences}
	\gdef\@ISSN{2076-3263}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geotechnics}{%
	\gdef\@journal{geotechnics}
	\gdef\@journalfull{Geotechnics}
	\gdef\@journalshort{Geotechnics}
	\gdef\@doiabbr{geotechnics}
	\gdef\@ISSN{2673-7094}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{geriatrics}{%
	\gdef\@journal{geriatrics}
	\gdef\@journalfull{Geriatrics}
	\gdef\@journalshort{Geriatrics}
	\gdef\@doiabbr{geriatrics}
	\gdef\@ISSN{2308-3417}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{germs}{%
	\gdef\@journal{germs}
	\gdef\@journalfull{Germs}
	\gdef\@journalshort{Germs}
	\gdef\@doiabbr{germs}
	\gdef\@ISSN{2248-2997}
	\gdef\@societyowner{Infection Science Forum}
	\gdef\@journaltype{ACS}}
\DeclareOption{glacies}{%
	\gdef\@journal{glacies}
	\gdef\@journalfull{Glacies}
	\gdef\@journalshort{Glacies}
	\gdef\@doiabbr{glacies}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{govpol}{%
	\gdef\@journal{govpol}
	\gdef\@journalfull{Governance \& Policy}
	\gdef\@journalshort{Gov. Policy}
	\gdef\@doiabbr{govpol}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{grainsci}{%
	\gdef\@journal{grainsci}
	\gdef\@journalfull{Grain Science}
	\gdef\@journalshort{Grain Sci.}
	\gdef\@doiabbr{grainsci}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{grasses}{%
	\gdef\@journal{grasses}
	\gdef\@journalfull{Grasses}
	\gdef\@journalshort{Grasses}
	\gdef\@doiabbr{grasses}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{green}{%
	\gdef\@journal{green}
	\gdef\@journalfull{Green}
	\gdef\@journalshort{Green}
	\gdef\@doiabbr{green}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{greenhealth}{%
	\gdef\@journal{greenhealth}
	\gdef\@journalfull{Green Health}
	\gdef\@journalshort{Green Health}
	\gdef\@doiabbr{greenhealth}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{gucdd}{%
	\gdef\@journal{gucdd}
	\gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}
	\gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}
	\gdef\@doiabbr{gucdd}
	\gdef\@ISSN{}
	\gdef\@societyowner{Gout, Hyperuricemia and Crystal Associated Disease Network}
	\gdef\@journaltype{ACS}}
\DeclareOption{gynecolcancer}{%
	\gdef\@journal{gynecolcancer}
	\gdef\@journalfull{Gynecologic Cancer}
	\gdef\@journalshort{Gynecol. Cancer}
	\gdef\@doiabbr{gynecolcancer}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hardware}{%
	\gdef\@journal{hardware}
	\gdef\@journalfull{Hardware}
	\gdef\@journalshort{Hardware}
	\gdef\@doiabbr{hardware}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hazardousmatters}{%
	\gdef\@journal{hazardousmatters}
	\gdef\@journalfull{Hazardous Matters}
	\gdef\@journalshort{Hazard. Matters}
	\gdef\@doiabbr{hazardousmatters}
	\gdef\@ISSN{0014-0014}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{healthcare}{%
	\gdef\@journal{healthcare}
	\gdef\@journalfull{Healthcare}
	\gdef\@journalshort{Healthcare}
	\gdef\@doiabbr{healthcare}
	\gdef\@ISSN{2227-9032}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{healthcmater}{%
	\gdef\@journal{healthcmater}
	\gdef\@journalfull{Healthcare Materials}
	\gdef\@journalshort{Healthc. Mater.}
	\gdef\@doiabbr{healthcmater}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hearts}{%
	\gdef\@journal{hearts}
	\gdef\@journalfull{Hearts}
	\gdef\@journalshort{Hearts}
	\gdef\@doiabbr{hearts}
	\gdef\@ISSN{2673-3846}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hemato}{%
	\gdef\@journal{hemato}
	\gdef\@journalfull{Hemato}
	\gdef\@journalshort{Hemato}
	\gdef\@doiabbr{hemato}
	\gdef\@ISSN{2673-6357}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hematolrep}{%
	\gdef\@journal{hematolrep}
	\gdef\@journalfull{Hematology Reports}
	\gdef\@journalshort{Hematol. Rep.}
	\gdef\@doiabbr{hematolrep}
	\gdef\@ISSN{2038-8330}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hep}{%
	\gdef\@journal{hep}
	\gdef\@journalfull{Health Economics and Policy}
	\gdef\@journalshort{Health Econ. Policy}
	\gdef\@doiabbr{hep}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{heritage}{%
	\gdef\@journal{heritage}
	\gdef\@journalfull{Heritage}
	\gdef\@journalshort{Heritage}
	\gdef\@doiabbr{heritage}
	\gdef\@ISSN{2571-9408}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{higheredu}{%
	\gdef\@journal{higheredu}
	\gdef\@journalfull{Trends in Higher Education}
	\gdef\@journalshort{Trends High. Educ.}
	\gdef\@doiabbr{higheredu}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{highthroughput}{%
	\gdef\@journal{highthroughput}
	\gdef\@journalfull{High-Throughput}
	\gdef\@journalshort{High-Throughput}
	\gdef\@doiabbr{ht}
	\gdef\@ISSN{2571-5135}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{histories}{%
	\gdef\@journal{histories}
	\gdef\@journalfull{Histories}
	\gdef\@journalshort{Histories}
	\gdef\@doiabbr{histories}
	\gdef\@ISSN{2409-9252}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{hls}{%
	\gdef\@journal{hls}
	\gdef\@journalfull{Healthcare in Low-Resource Settings}
	\gdef\@journalshort{Healthc. Low-Resour. Settings}
	\gdef\@doiabbr{hls}
	\gdef\@ISSN{2281-7824}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{horticulturae}{%
	\gdef\@journal{horticulturae}
	\gdef\@journalfull{Horticulturae}
	\gdef\@journalshort{Horticulturae}
	\gdef\@doiabbr{horticulturae}
	\gdef\@ISSN{2311-7524}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hospitals}{%
	\gdef\@journal{hospitals}
	\gdef\@journalfull{Hospitals}
	\gdef\@journalshort{Hospitals}
	\gdef\@doiabbr{hospitals}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{humanities}{%
	\gdef\@journal{humanities}
	\gdef\@journalfull{Humanities}
	\gdef\@journalshort{Humanities}
	\gdef\@doiabbr{h}
	\gdef\@ISSN{2076-0787}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{humanoids}{%
	\gdef\@journal{humanoids}
	\gdef\@journalfull{Humanoids---A Journal of Humanoid Robots}
	\gdef\@journalshort{Humanoids}
	\gdef\@doiabbr{humanoids}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{humans}{%
	\gdef\@journal{humans}
	\gdef\@journalfull{Humans}
	\gdef\@journalshort{Humans}
	\gdef\@doiabbr{humans}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{hydrobiology}{%
	\gdef\@journal{hydrobiology}
	\gdef\@journalfull{Hydrobiology}
	\gdef\@journalshort{Hydrobiology}
	\gdef\@doiabbr{hydrobiology}
	\gdef\@ISSN{2673-9917}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hydrogen}{%
	\gdef\@journal{hydrogen}
	\gdef\@journalfull{Hydrogen}
	\gdef\@journalshort{Hydrogen}
	\gdef\@doiabbr{hydrogen}
	\gdef\@ISSN{2673-4141}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hydrology}{%
	\gdef\@journal{hydrology}
	\gdef\@journalfull{Hydrology}
	\gdef\@journalshort{Hydrology}
	\gdef\@doiabbr{hydrology}
	\gdef\@ISSN{2306-5338}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hydrometeorology}{%
	\gdef\@journal{hydrometeorology}
	\gdef\@journalfull{Hydrometeorology}
	\gdef\@journalshort{Hydrometeorology}
	\gdef\@doiabbr{hydrometeorology}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hydropower}{%
	\gdef\@journal{hydropower}
	\gdef\@journalfull{Hydropower}
	\gdef\@journalshort{Hydropower}
	\gdef\@doiabbr{hydropower}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{hygiene}{%
	\gdef\@journal{hygiene}
	\gdef\@journalfull{Hygiene}
	\gdef\@journalshort{Hygiene}
	\gdef\@doiabbr{hygiene}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{idhm}{%
	\gdef\@journal{idhm}
	\gdef\@journalfull{Infectious Diseases and Herbal Medicine}
	\gdef\@journalshort{Infect. Dis. Herb. Med.}
	\gdef\@doiabbr{idhm}
	\gdef\@ISSN{2724-5284}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{idr}{%
	\gdef\@journal{idr}
	\gdef\@journalfull{Infectious Disease Reports}
	\gdef\@journalshort{Infect. Dis. Rep.}
	\gdef\@doiabbr{idr}
	\gdef\@ISSN{2036-7449}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{iic}{%
	\gdef\@journal{iic}
	\gdef\@journalfull{Intelligent Infrastructure and Construction}
	\gdef\@journalshort{Intell. Infrastruct. Constr.}
	\gdef\@doiabbr{iic}
	\gdef\@ISSN{3042-4720}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijcs}{%
	\gdef\@journal{ijcs}
	\gdef\@journalfull{International Journal of Cognitive Sciences}
	\gdef\@journalshort{Int. J. Cogn. Sci.}
	\gdef\@doiabbr{ijcs}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{ijem}{%
	\gdef\@journal{ijem}
	\gdef\@journalfull{International Journal of Environmental Medicine}
	\gdef\@journalshort{Int. J. Environ. Med.}
	\gdef\@doiabbr{ijem}
	\gdef\@ISSN{3042-7681}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijerph}{%
	\gdef\@journal{ijerph}
	\gdef\@journalfull{International Journal of Environmental Research and Public Health}
	\gdef\@journalshort{Int. J. Environ. Res. Public Health}
	\gdef\@doiabbr{ijerph}
	\gdef\@ISSN{1660-4601}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijfs}{%
	\gdef\@journal{ijfs}
	\gdef\@journalfull{International Journal of Financial Studies}
	\gdef\@journalshort{Int. J. Financ. Stud.}
	\gdef\@doiabbr{ijfs}
	\gdef\@ISSN{2227-7072}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{ijgi}{%
	\gdef\@journal{ijgi}
	\gdef\@journalfull{ISPRS International Journal of Geo-Information}
	\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}
	\gdef\@doiabbr{ijgi}
	\gdef\@ISSN{2220-9964}
	\gdef\@societyowner{International Society for Photogrammetry and Remote Sensing}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijmd}{%
	\gdef\@journal{ijmd}
	\gdef\@journalfull{International Journal of Medical Devices}
	\gdef\@journalshort{Int. J. Med. Devices}
	\gdef\@doiabbr{ijmd}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijms}{%
	\gdef\@journal{ijms}
	\gdef\@journalfull{International Journal of Molecular Sciences}
	\gdef\@journalshort{Int. J. Mol. Sci.}
	\gdef\@doiabbr{ijms}
	\gdef\@ISSN{1422-0067}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijns}{%
	\gdef\@journal{ijns}
	\gdef\@journalfull{International Journal of Neonatal Screening}
	\gdef\@journalshort{Int. J. Neonatal Screen.}
	\gdef\@doiabbr{ijns}
	\gdef\@ISSN{2409-515X}
	\gdef\@societyowner{International Society for Neonatal Screening}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijom}{%
	\gdef\@journal{ijom}
	\gdef\@journalfull{International Journal of Orofacial Myology and Myofunctional Therapy}
	\gdef\@journalshort{Int. J. Orofac. Myol. Myofunct. Ther.}
	\gdef\@doiabbr{ijom}
	\gdef\@ISSN{}
	\gdef\@societyowner{International Association of Orofacial Myology}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijp}{%
	\gdef\@journal{ijp}
	\gdef\@journalfull{International Journal of Phenomics}
	\gdef\@journalshort{Int. J. Phenomics}
	\gdef\@doiabbr{ijp}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijpb}{%
	\gdef\@journal{ijpb}
	\gdef\@journalfull{International Journal of Plant Biology}
	\gdef\@journalshort{Int. J. Plant Biol.}
	\gdef\@doiabbr{ijpb}
	\gdef\@ISSN{2037-0164}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijt}{%
	\gdef\@journal{ijt}
	\gdef\@journalfull{International Journal of Topology}
	\gdef\@journalshort{Int. J. Topol.}
	\gdef\@doiabbr{ijt}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijtm}{%
	\gdef\@journal{ijtm}
	\gdef\@journalfull{International Journal of Translational Medicine}
	\gdef\@journalshort{Int. J. Transl. Med.}
	\gdef\@doiabbr{ijtm}
	\gdef\@ISSN{2673-8937}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijtpp}{%
	\gdef\@journal{ijtpp}
	\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}
	\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}
	\gdef\@doiabbr{ijtpp}
	\gdef\@ISSN{2504-186X}
	\gdef\@societyowner{European Turbomachinery Society}
	\gdef\@journaltype{ACS}}
\DeclareOption{ijtst}{%
	\gdef\@journal{ijtst}
	\gdef\@journalfull{International Journal of Thermofluid Science and Technology}
	\gdef\@journalshort{Int. J. Thermofluid Sci. Technol.}
	\gdef\@doiabbr{ijtst}
	\gdef\@ISSN{3043-1107}
	\gdef\@societyowner{Nanjing University of Aeronautics and Astronautics}
	\gdef\@journaltype{ACS}}
\DeclareOption{ime}{%
	\gdef\@journal{ime}
	\gdef\@journalfull{International Medical Education}
	\gdef\@journalshort{Int. Med. Educ.}
	\gdef\@doiabbr{ime}
	\gdef\@ISSN{2813-141X}
	\gdef\@societyowner{Academic Society for International Medical Education}
	\gdef\@journaltype{ACS}}
\DeclareOption{immuno}{%
	\gdef\@journal{immuno}
	\gdef\@journalfull{Immuno}
	\gdef\@journalshort{Immuno}
	\gdef\@doiabbr{immuno}
	\gdef\@ISSN{2673-5601}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{industries}{%
	\gdef\@journal{industries}
	\gdef\@journalfull{Industries}
	\gdef\@journalshort{Industries}
	\gdef\@doiabbr{industries}
	\gdef\@ISSN{3042-9021}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{inflammj}{%
	\gdef\@journal{inflammj}
	\gdef\@journalfull{Inflammation Journal}
	\gdef\@journalshort{Inflamm. J.}
	\gdef\@doiabbr{inflammj}
	\gdef\@ISSN{3043-0348}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{informatics}{%
	\gdef\@journal{informatics}
	\gdef\@journalfull{Informatics}
	\gdef\@journalshort{Informatics}
	\gdef\@doiabbr{informatics}
	\gdef\@ISSN{2227-9709}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{information}{%
	\gdef\@journal{information}
	\gdef\@journalfull{Information}
	\gdef\@journalshort{Information}
	\gdef\@doiabbr{info}
	\gdef\@ISSN{2078-2489}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{infrastructures}{%
	\gdef\@journal{infrastructures}
	\gdef\@journalfull{Infrastructures}
	\gdef\@journalshort{Infrastructures}
	\gdef\@doiabbr{infrastructures}
	\gdef\@ISSN{2412-3811}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{inorganics}{%
	\gdef\@journal{inorganics}
	\gdef\@journalfull{Inorganics}
	\gdef\@journalshort{Inorganics}
	\gdef\@doiabbr{inorganics}
	\gdef\@ISSN{2304-6740}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{insects}{%
	\gdef\@journal{insects}
	\gdef\@journalfull{Insects}
	\gdef\@journalshort{Insects}
	\gdef\@doiabbr{insects}
	\gdef\@ISSN{2075-4450}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{instruments}{%
	\gdef\@journal{instruments}
	\gdef\@journalfull{Instruments}
	\gdef\@journalshort{Instruments}
	\gdef\@doiabbr{instruments}
	\gdef\@ISSN{2410-390X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{inventions}{%
	\gdef\@journal{inventions}
	\gdef\@journalfull{Inventions}
	\gdef\@journalshort{Inventions}
	\gdef\@doiabbr{inventions}
	\gdef\@ISSN{2411-5134}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{investment}{%
	\gdef\@journal{investment}
	\gdef\@journalfull{Investment}
	\gdef\@journalshort{Investment}
	\gdef\@doiabbr{investment}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{iot}{%
	\gdef\@journal{iot}
	\gdef\@journalfull{IoT}
	\gdef\@journalshort{IoT}
	\gdef\@doiabbr{iot}
	\gdef\@ISSN{2624-831X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{iron}{%
	\gdef\@journal{iron}
	\gdef\@journalfull{Iron}
	\gdef\@journalshort{Iron}
	\gdef\@doiabbr{iron}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{j}{%
	\gdef\@journal{j}
	\gdef\@journalfull{J}
	\gdef\@journalshort{J}
	\gdef\@doiabbr{j}
	\gdef\@ISSN{2571-8800}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jaestheticmed}{%
	\gdef\@journal{jaestheticmed}
	\gdef\@journalfull{Journal of Aesthetic Medicine}
	\gdef\@journalshort{J. Aesthetic Med.}
	\gdef\@doiabbr{jaestheticmed}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jal}{%
	\gdef\@journal{jal}
	\gdef\@journalfull{Journal of Ageing and Longevity}
	\gdef\@journalshort{J. Ageing Longev.}
	\gdef\@doiabbr{jal}
	\gdef\@ISSN{2673-9259}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{japma}{%
	\gdef\@journal{japma}
	\gdef\@journalfull{Journal of the American Podiatric Medical Association}
	\gdef\@journalshort{J. Am. Podiatr. Med. Assoc.}
	\gdef\@doiabbr{japma}
	\gdef\@ISSN{1930-8264}
	\gdef\@societyowner{American Podiatric Medical Association}
	\gdef\@journaltype{ACS}}
\DeclareOption{jcdd}{%
	\gdef\@journal{jcdd}
	\gdef\@journalfull{Journal of Cardiovascular Development and Disease}
	\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}
	\gdef\@doiabbr{jcdd}
	\gdef\@ISSN{2308-3425}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jcm}{%
	\gdef\@journal{jcm}
	\gdef\@journalfull{Journal of Clinical Medicine}
	\gdef\@journalshort{J. Clin. Med.}
	\gdef\@doiabbr{jcm}
	\gdef\@ISSN{2077-0383}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jcp}{%
	\gdef\@journal{jcp}
	\gdef\@journalfull{Journal of Cybersecurity and Privacy}
	\gdef\@journalshort{J. Cybersecur. Priv.}
	\gdef\@doiabbr{jcp}
	\gdef\@ISSN{2624-800X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jcrm}{%
	\gdef\@journal{jcrm}
	\gdef\@journalfull{Journal of CardioRenal Medicine}
	\gdef\@journalshort{J. CardioRenal Med.}
	\gdef\@doiabbr{jcrm}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jcs}{%
	\gdef\@journal{jcs}
	\gdef\@journalfull{Journal of Composites Science}
	\gdef\@journalshort{J. Compos. Sci.}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2504-477X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jcto}{%
	\gdef\@journal{jcto}
	\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}
	\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}
	\gdef\@doiabbr{jcto}
	\gdef\@ISSN{2813-1053}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jdad}{%
	\gdef\@journal{jdad}
	\gdef\@journalfull{Journal of Dementia and Alzheimer’s Disease}
	\gdef\@journalshort{J. Dement. Alzheimer's Dis.}
	\gdef\@doiabbr{jdad}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jdb}{%
	\gdef\@journal{jdb}
	\gdef\@journalfull{Journal of Developmental Biology}
	\gdef\@journalshort{J. Dev. Biol.}
	\gdef\@doiabbr{jdb}
	\gdef\@ISSN{2221-3759}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jdcp}{%
	\gdef\@journal{jdcp}
	\gdef\@journalfull{Journal of Disease Control and Prevention}
	\gdef\@journalshort{J. Dis. Control Prev.}
	\gdef\@doiabbr{jdcp}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jdream}{%
	\gdef\@journal{jdream}
	\gdef\@journalfull{Journal of Interdisciplinary Research Applied to Medicine}
	\gdef\@journalshort{J. Interdiscip. Res. Appl. Med.}
	\gdef\@doiabbr{jdream}
	\gdef\@ISSN{2532-7518}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jemr}{%
	\gdef\@journal{jemr}
	\gdef\@journalfull{Journal of Eye Movement Research}
	\gdef\@journalshort{J. Eye Mov. Res.}
	\gdef\@doiabbr{jemr}
	\gdef\@ISSN{1995-8692}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jeta}{%
	\gdef\@journal{jeta}
	\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}
	\gdef\@journalshort{J. Exp. Theor. Anal.}
	\gdef\@doiabbr{jeta}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jfb}{%
	\gdef\@journal{jfb}
	\gdef\@journalfull{Journal of Functional Biomaterials}
	\gdef\@journalshort{J. Funct. Biomater.}
	\gdef\@doiabbr{jfb}
	\gdef\@ISSN{2079-4983}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jfmk}{%
	\gdef\@journal{jfmk}
	\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}
	\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}
	\gdef\@doiabbr{jfmk}
	\gdef\@ISSN{2411-5142}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jfth}{%
	\gdef\@journal{jfth}
	\gdef\@journalfull{Journal of Fast-Track Health}
	\gdef\@journalshort{J. Fast-Track Health}
	\gdef\@doiabbr{jfth}
	\gdef\@ISSN{3043-0844}
	\gdef\@societyowner{Fast-Track Health}
	\gdef\@journaltype{ACS}}
\DeclareOption{jgbg}{%
	\gdef\@journal{jgbg}
	\gdef\@journalfull{Journal of Genome Biotechnology and Genetics}
	\gdef\@journalshort{J. Genome Biotechnol. Genet.}
	\gdef\@doiabbr{jgbg}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jgg}{%
	\gdef\@journal{jgg}
	\gdef\@journalfull{Journal of Gerontology and Geriatrics}
	\gdef\@journalshort{J. Gerontol. Geriatr.}
	\gdef\@doiabbr{jgg}
	\gdef\@ISSN{2499-6564}
	\gdef\@societyowner{Italian Society of Gerontology and Geriatrics}
	\gdef\@journaltype{ACS}}
\DeclareOption{jimaging}{%
	\gdef\@journal{jimaging}
	\gdef\@journalfull{Journal of Imaging}
	\gdef\@journalshort{J. Imaging}
	\gdef\@doiabbr{jimaging}
	\gdef\@ISSN{2313-433X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jintelligence}{%
	\gdef\@journal{jintelligence}
	\gdef\@journalfull{Journal of Intelligence}
	\gdef\@journalshort{J. Intell.}
	\gdef\@doiabbr{jintelligence}
	\gdef\@ISSN{2079-3200}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{jissn}{%
	\gdef\@journal{jissn}
	\gdef\@journalfull{Journal of the International Society of Sports Nutrition}
	\gdef\@journalshort{J. Int. Soc. Sports Nutr.}
	\gdef\@doiabbr{jissn}
	\gdef\@ISSN{1550-2783}
	\gdef\@societyowner{International Society of Sports Nutrition (ISSN)}
	\gdef\@journaltype{ACS}}
\DeclareOption{jlpea}{%
	\gdef\@journal{jlpea}
	\gdef\@journalfull{Journal of Low Power Electronics and Applications}
	\gdef\@journalshort{J. Low Power Electron. Appl.}
	\gdef\@doiabbr{jlpea}
	\gdef\@ISSN{2079-9268}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jmahp}{%
	\gdef\@journal{jmahp}
	\gdef\@journalfull{Journal of Market Access \& Health Policy}
	\gdef\@journalshort{J. Mark. Access Health Policy}
	\gdef\@doiabbr{jmahp}
	\gdef\@ISSN{2001-6689}
	\gdef\@societyowner{Market Access Society}
	\gdef\@journaltype{ACS}}
\DeclareOption{jmmp}{%
	\gdef\@journal{jmmp}
	\gdef\@journalfull{Journal of Manufacturing and Materials Processing}
	\gdef\@journalshort{J. Manuf. Mater. Process.}
	\gdef\@doiabbr{jmmp}
	\gdef\@ISSN{2504-4494}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jmms}{%
	\gdef\@journal{jmms}
	\gdef\@journalfull{Journal of Mind and Medical Sciences}
	\gdef\@journalshort{J. Mind Med. Sci.}
	\gdef\@doiabbr{jmms}
	\gdef\@ISSN{2392-7674}
	\gdef\@societyowner{Journal of Mind and Medical Sciences}
	\gdef\@journaltype{ACS}}
\DeclareOption{jmp}{%
	\gdef\@journal{jmp}
	\gdef\@journalfull{Journal of Molecular Pathology}
	\gdef\@journalshort{J. Mol. Pathol.}
	\gdef\@doiabbr{jmp}
	\gdef\@ISSN{2673-5261}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jmse}{%
	\gdef\@journal{jmse}
	\gdef\@journalfull{Journal of Marine Science and Engineering}
	\gdef\@journalshort{J. Mar. Sci. Eng.}
	\gdef\@doiabbr{jmse}
	\gdef\@ISSN{2077-1312}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jne}{%
	\gdef\@journal{jne}
	\gdef\@journalfull{Journal of Nuclear Engineering}
	\gdef\@journalshort{J. Nucl. Eng.}
	\gdef\@doiabbr{jne}
	\gdef\@ISSN{2673-4362}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jnt}{%
	\gdef\@journal{jnt}
	\gdef\@journalfull{Journal of Nanotheranostics}
	\gdef\@journalshort{J. Nanotheranostics}
	\gdef\@doiabbr{jnt}
	\gdef\@ISSN{2624-845X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jof}{%
	\gdef\@journal{jof}
	\gdef\@journalfull{Journal of Fungi}
	\gdef\@journalshort{J. Fungi}
	\gdef\@doiabbr{jof}
	\gdef\@ISSN{2309-608X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{joi}{%
	\gdef\@journal{joi}
	\gdef\@journalfull{Journal of Innovation}
	\gdef\@journalshort{J. Innov.}
	\gdef\@doiabbr{joi}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{joitmc}{%
	\gdef\@journal{joitmc}
	\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}
	\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}
	\gdef\@doiabbr{joitmc}
	\gdef\@ISSN{2199-8531}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{joma}{%
	\gdef\@journal{joma}
	\gdef\@journalfull{Journal of the Oman Medical Association}
	\gdef\@journalshort{J. Oman Med. Assoc.}
	\gdef\@doiabbr{joma}
	\gdef\@ISSN{2813-8759}
	\gdef\@societyowner{Oman Medical Association}
	\gdef\@journaltype{ACS}}
\DeclareOption{jop}{%
	\gdef\@journal{jop}
	\gdef\@journalfull{Journal of Parks}
	\gdef\@journalshort{J. Parks}
	\gdef\@doiabbr{jop}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{joptm}{%
	\gdef\@journal{joptm}
	\gdef\@journalfull{Journal of Optical Materials}
	\gdef\@journalshort{J. Opt. Mater.}
	\gdef\@doiabbr{joptm}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jor}{%
	\gdef\@journal{jor}
	\gdef\@journalfull{Journal of Respiration}
	\gdef\@journalshort{J. Respir.}
	\gdef\@doiabbr{jor}
	\gdef\@ISSN{2673-527X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{journalmedia}{%
	\gdef\@journal{journalmedia}
	\gdef\@journalfull{Journalism and Media}
	\gdef\@journalshort{Journal. Media}
	\gdef\@doiabbr{journalmedia}
	\gdef\@ISSN{2673-5172}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{jox}{%
	\gdef\@journal{jox}
	\gdef\@journalfull{Journal of Xenobiotics}
	\gdef\@journalshort{J. Xenobiotics}
	\gdef\@doiabbr{jox}
	\gdef\@ISSN{2039-4713}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jpbi}{%
	\gdef\@journal{jpbi}
	\gdef\@journalfull{Journal of Pharmaceutical and BioTech Industry}
	\gdef\@journalshort{J. Pharm. BioTech Ind.}
	\gdef\@doiabbr{jpbi}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jphytomed}{%
	\gdef\@journal{jphytomed}
	\gdef\@journalfull{Journal of Phytomedicine}
	\gdef\@journalshort{J. Phytomed.}
	\gdef\@doiabbr{jphytomed}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jpm}{%
	\gdef\@journal{jpm}
	\gdef\@journalfull{Journal of Personalized Medicine}
	\gdef\@journalshort{J. Pers. Med.}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{2075-4426}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jrfm}{%
	\gdef\@journal{jrfm}
	\gdef\@journalfull{Journal of Risk and Financial Management}
	\gdef\@journalshort{J. Risk Financ. Manag.}
	\gdef\@doiabbr{jrfm}
	\gdef\@ISSN{1911-8074}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{jsam}{%
	\gdef\@journal{jsam}
	\gdef\@journalfull{Journal of Strategic and Applied Marketing}
	\gdef\@journalshort{J. Strateg. Appl. Mark.}
	\gdef\@doiabbr{jsam}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{jsan}{%
	\gdef\@journal{jsan}
	\gdef\@journalfull{Journal of Sensor and Actuator Networks}
	\gdef\@journalshort{J. Sens. Actuator Netw.}
	\gdef\@doiabbr{jsan}
	\gdef\@ISSN{2224-2708}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jtaer}{%
	\gdef\@journal{jtaer}
	\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}
	\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}
	\gdef\@doiabbr{jtaer}
	\gdef\@ISSN{0718-1876}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jvd}{%
	\gdef\@journal{jvd}
	\gdef\@journalfull{Journal of Vascular Diseases}
	\gdef\@journalshort{J. Vasc. Dis.}
	\gdef\@doiabbr{jvd}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{jzbg}{%
	\gdef\@journal{jzbg}
	\gdef\@journalfull{Journal of Zoological and Botanical Gardens}
	\gdef\@journalshort{J. Zool. Bot. Gard.}
	\gdef\@doiabbr{jzbg}
	\gdef\@ISSN{2673-5636}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{kidneydial}{%
	\gdef\@journal{kidneydial}
	\gdef\@journalfull{Kidney and Dialysis}
	\gdef\@journalshort{Kidney Dial.}
	\gdef\@doiabbr{kidneydial}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{kinasesphosphatases}{%
	\gdef\@journal{kinasesphosphatases}
	\gdef\@journalfull{Kinases and Phosphatases}
	\gdef\@journalshort{Kinases Phosphatases}
	\gdef\@doiabbr{kinasesphosphatases}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{knowledge}{%
	\gdef\@journal{knowledge}
	\gdef\@journalfull{Knowledge}
	\gdef\@journalshort{Knowledge}
	\gdef\@doiabbr{knowledge}
	\gdef\@ISSN{2673-9585}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{labmed}{%
	\gdef\@journal{labmed}
	\gdef\@journalfull{LabMed}
	\gdef\@journalshort{LabMed}
	\gdef\@doiabbr{labmed}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{laboratories}{%
	\gdef\@journal{laboratories}
	\gdef\@journalfull{Laboratories}
	\gdef\@journalshort{Laboratories}
	\gdef\@doiabbr{laboratories}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{lam}{%
	\gdef\@journal{lam}
	\gdef\@journalfull{Low-Altitude Mobility}
	\gdef\@journalshort{Low-Alt. Mobil.}
	\gdef\@doiabbr{lam}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{land}{%
	\gdef\@journal{land}
	\gdef\@journalfull{Land}
	\gdef\@journalshort{Land}
	\gdef\@doiabbr{land}
	\gdef\@ISSN{2073-445X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{langtechnol}{%
	\gdef\@journal{langtechnol}
	\gdef\@journalfull{Language Technology}
	\gdef\@journalshort{Lang. Technol.}
	\gdef\@doiabbr{langtechnol}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{	ACS	}}
\DeclareOption{languages}{%
	\gdef\@journal{languages}
	\gdef\@journalfull{Languages}
	\gdef\@journalshort{Languages}
	\gdef\@doiabbr{languages}
	\gdef\@ISSN{2226-471X}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{lasers}{%
	\gdef\@journal{lasers}
	\gdef\@journalfull{Lasers}
	\gdef\@journalshort{Lasers}
	\gdef\@doiabbr{lasers}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{laws}{%
	\gdef\@journal{laws}
	\gdef\@journalfull{Laws}
	\gdef\@journalshort{Laws}
	\gdef\@doiabbr{laws}
	\gdef\@ISSN{2075-471X}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{legumes}{%
	\gdef\@journal{legumes}
	\gdef\@journalfull{Legumes}
	\gdef\@journalshort{Legumes}
	\gdef\@doiabbr{legumes}
	\gdef\@ISSN{3043-0739}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{life}{%
	\gdef\@journal{life}
	\gdef\@journalfull{Life}
	\gdef\@journalshort{Life}
	\gdef\@doiabbr{life}
	\gdef\@ISSN{2075-1729}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{lights}{%
	\gdef\@journal{lights}
	\gdef\@journalfull{Lights}
	\gdef\@journalshort{Lights}
	\gdef\@doiabbr{lights}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{limnolrev}{%
	\gdef\@journal{limnolrev}
	\gdef\@journalfull{Limnological Review}
	\gdef\@journalshort{Limnol. Rev.}
	\gdef\@doiabbr{limnolrev}
	\gdef\@ISSN{2300-7575}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{lipidology}{%
	\gdef\@journal{lipidology}
	\gdef\@journalfull{Lipidology}
	\gdef\@journalshort{Lipidology}
	\gdef\@doiabbr{lipidology}
	\gdef\@ISSN{2813-7086}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{liquids}{%
	\gdef\@journal{liquids}
	\gdef\@journalfull{Liquids}
	\gdef\@journalshort{Liquids}
	\gdef\@doiabbr{liquids}
	\gdef\@ISSN{2673-8015}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{literature}{%
	\gdef\@journal{literature}
	\gdef\@journalfull{Literature}
	\gdef\@journalshort{Literature}
	\gdef\@doiabbr{literature}
	\gdef\@ISSN{2410-9789}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{livers}{%
	\gdef\@journal{livers}
	\gdef\@journalfull{Livers}
	\gdef\@journalshort{Livers}
	\gdef\@doiabbr{livers}
	\gdef\@ISSN{2673-4389}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{logics}{%
	\gdef\@journal{logics}
	\gdef\@journalfull{Logics}
	\gdef\@journalshort{Logics}
	\gdef\@doiabbr{logics}
	\gdef\@ISSN{2813-0405}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{logistics}{%
	\gdef\@journal{logistics}
	\gdef\@journalfull{Logistics}
	\gdef\@journalshort{Logistics}
	\gdef\@doiabbr{logistics}
	\gdef\@ISSN{2305-6290}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{lubricants}{%
	\gdef\@journal{lubricants}
	\gdef\@journalfull{Lubricants}
	\gdef\@journalshort{Lubricants}
	\gdef\@doiabbr{lubricants}
	\gdef\@ISSN{2075-4442}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{lymphatics}{%
	\gdef\@journal{lymphatics}
	\gdef\@journalfull{Lymphatics}
	\gdef\@journalshort{Lymphatics}
	\gdef\@doiabbr{lymphatics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{machines}{%
	\gdef\@journal{machines}
	\gdef\@journalfull{Machines}
	\gdef\@journalshort{Machines}
	\gdef\@doiabbr{machines}
	\gdef\@ISSN{2075-1702}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{macromol}{%
	\gdef\@journal{macromol}
	\gdef\@journalfull{Macromol}
	\gdef\@journalshort{Macromol}
	\gdef\@doiabbr{macromol}
	\gdef\@ISSN{2673-6209}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{magnetism}{%
	\gdef\@journal{magnetism}
	\gdef\@journalfull{Magnetism}
	\gdef\@journalshort{Magnetism}
	\gdef\@doiabbr{magnetism}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{magnetochemistry}{%
	\gdef\@journal{magnetochemistry}
	\gdef\@journalfull{Magnetochemistry}
	\gdef\@journalshort{Magnetochemistry}
	\gdef\@doiabbr{magnetochemistry}
	\gdef\@ISSN{2312-7481}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{make}{%
	\gdef\@journal{make}
	\gdef\@journalfull{Machine Learning and Knowledge Extraction}
	\gdef\@journalshort{Mach. Learn. Knowl. Extr.}
	\gdef\@doiabbr{make}
	\gdef\@ISSN{2504-4990}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{marinedrugs}{%
	\gdef\@journal{marinedrugs}
	\gdef\@journalfull{Marine Drugs}
	\gdef\@journalshort{Mar. Drugs}
	\gdef\@doiabbr{md}
	\gdef\@ISSN{1660-3397}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{maritime}{%
	\gdef\@journal{maritime}
	\gdef\@journalfull{Maritime}
	\gdef\@journalshort{Maritime}
	\gdef\@doiabbr{maritime}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{materials}{%
	\gdef\@journal{materials}
	\gdef\@journalfull{Materials}
	\gdef\@journalshort{Materials}
	\gdef\@doiabbr{ma}
	\gdef\@ISSN{1996-1944}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{materproc}{%
	\gdef\@journal{materproc}
	\gdef\@journalfull{Materials Proceedings}
	\gdef\@journalshort{Mater. Proc.}
	\gdef\@doiabbr{materproc}
	\gdef\@ISSN{2673-4605}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mathematics}{%
	\gdef\@journal{mathematics}
	\gdef\@journalfull{Mathematics}
	\gdef\@journalshort{Mathematics}
	\gdef\@doiabbr{math}
	\gdef\@ISSN{2227-7390}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mca}{%
	\gdef\@journal{mca}
	\gdef\@journalfull{Mathematical and Computational Applications}
	\gdef\@journalshort{Math. Comput. Appl.}
	\gdef\@doiabbr{mca}
	\gdef\@ISSN{2297-8747}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mcb}{%
	\gdef\@journal{mcb}
	\gdef\@journalfull{Mathematical and Computational Biology}
	\gdef\@journalshort{Math. Comput. Biol.}
	\gdef\@doiabbr{mcb}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{measurements}{%
	\gdef\@journal{measurements}
	\gdef\@journalfull{Measurements}
	\gdef\@journalshort{Measurements}
	\gdef\@doiabbr{measurements}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{meb}{%
	\gdef\@journal{meb}
	\gdef\@journalfull{Medical Ethics and Bioethics}
	\gdef\@journalshort{Med. Ethics Bioeth.}
	\gdef\@doiabbr{meb}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{medicina}{%
	\gdef\@journal{medicina}
	\gdef\@journalfull{Medicina}
	\gdef\@journalshort{Medicina}
	\gdef\@doiabbr{medicina}
	\gdef\@ISSN{1648-9144}
	\gdef\@societyowner{Lithuanian University of Health Sciences}
	\gdef\@journaltype{ACS}}
\DeclareOption{medicines}{%
	\gdef\@journal{medicines}
	\gdef\@journalfull{Medicines}
	\gdef\@journalshort{Medicines}
	\gdef\@doiabbr{medicines}
	\gdef\@ISSN{2305-6320}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{medsci}{%
	\gdef\@journal{medsci}
	\gdef\@journalfull{Medical Sciences}
	\gdef\@journalshort{Med. Sci.}
	\gdef\@doiabbr{medsci}
	\gdef\@ISSN{2076-3271}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{membranes}{%
	\gdef\@journal{membranes}
	\gdef\@journalfull{Membranes}
	\gdef\@journalshort{Membranes}
	\gdef\@doiabbr{membranes}
	\gdef\@ISSN{2077-0375}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{merits}{%
	\gdef\@journal{merits}
	\gdef\@journalfull{Merits}
	\gdef\@journalshort{Merits}
	\gdef\@doiabbr{merits}
	\gdef\@ISSN{2673-8104}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{metabolites}{%
	\gdef\@journal{metabolites}
	\gdef\@journalfull{Metabolites}
	\gdef\@journalshort{Metabolites}
	\gdef\@doiabbr{metabo}
	\gdef\@ISSN{2218-1989}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{metals}{%
	\gdef\@journal{metals}
	\gdef\@journalfull{Metals}
	\gdef\@journalshort{Metals}
	\gdef\@doiabbr{met}
	\gdef\@ISSN{2075-4701}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{metamaterialsadv}{%
	\gdef\@journal{metamaterialsadv}
	\gdef\@journalfull{Metamaterials Advances}
	\gdef\@journalshort{Metamaterials Adv.}
	\gdef\@doiabbr{metamaterialsadv}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{meteorology}{%
	\gdef\@journal{meteorology}
	\gdef\@journalfull{Meteorology}
	\gdef\@journalshort{Meteorology}
	\gdef\@doiabbr{meteorology}
	\gdef\@ISSN{2674-0494}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{methane}{%
	\gdef\@journal{methane}
	\gdef\@journalfull{Methane}
	\gdef\@journalshort{Methane}
	\gdef\@doiabbr{methane}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{metrics}{%
	\gdef\@journal{metrics}
	\gdef\@journalfull{Metrics}
	\gdef\@journalshort{Metrics}
	\gdef\@doiabbr{metrics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{metrology}{%
	\gdef\@journal{metrology}
	\gdef\@journalfull{Metrology}
	\gdef\@journalshort{Metrology}
	\gdef\@doiabbr{metrology}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{micro}{%
	\gdef\@journal{micro}
	\gdef\@journalfull{Micro}
	\gdef\@journalshort{Micro}
	\gdef\@doiabbr{micro}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{microarrays}{%
	\gdef\@journal{microarrays}
	\gdef\@journalfull{Microarrays}
	\gdef\@journalshort{Microarrays}
	\gdef\@doiabbr{microarrays}
	\gdef\@ISSN{2076-3905}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{microbiolres}{%
	\gdef\@journal{microbiolres}
	\gdef\@journalfull{Microbiology Research}
	\gdef\@journalshort{Microbiol. Res.}
	\gdef\@doiabbr{microbiolres}
	\gdef\@ISSN{2036-7481}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{microchem}{%
	\gdef\@journal{microchem}
	\gdef\@journalfull{Microchem}
	\gdef\@journalshort{Microchem}
	\gdef\@doiabbr{microchem}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{microelectronics}{%
	\gdef\@journal{microelectronics}
	\gdef\@journalfull{Microelectronics}
	\gdef\@journalshort{Microelectronics}
	\gdef\@doiabbr{microelectronics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{micromachines}{%
	\gdef\@journal{micromachines}
	\gdef\@journalfull{Micromachines}
	\gdef\@journalshort{Micromachines}
	\gdef\@doiabbr{mi}
	\gdef\@ISSN{2072-666X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{microorganisms}{%
	\gdef\@journal{microorganisms}
	\gdef\@journalfull{Microorganisms}
	\gdef\@journalshort{Microorganisms}
	\gdef\@doiabbr{microorganisms}
	\gdef\@ISSN{2076-2607}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{microplastics}{%
	\gdef\@journal{microplastics}
	\gdef\@journalfull{Microplastics}
	\gdef\@journalshort{Microplastics}
	\gdef\@doiabbr{microplastics}
	\gdef\@ISSN{2673-8929}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{microwave}{%
	\gdef\@journal{microwave}
	\gdef\@journalfull{Microwave}
	\gdef\@journalshort{Microwave}
	\gdef\@doiabbr{microwave}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{minerals}{%
	\gdef\@journal{minerals}
	\gdef\@journalfull{Minerals}
	\gdef\@journalshort{Minerals}
	\gdef\@doiabbr{min}
	\gdef\@ISSN{2075-163X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mining}{%
	\gdef\@journal{mining}
	\gdef\@journalfull{Mining}
	\gdef\@journalshort{Mining}
	\gdef\@doiabbr{mining}
	\gdef\@ISSN{2673-6489}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mmphys}{%
	\gdef\@journal{mmphys}
	\gdef\@journalfull{Modern Mathematical Physics}
	\gdef\@journalshort{Mod. Math. Phys.}
	\gdef\@doiabbr{mmphys}
	\gdef\@ISSN{3042-5034}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{modelling}{%
	\gdef\@journal{modelling}
	\gdef\@journalfull{Modelling}
	\gdef\@journalshort{Modelling}
	\gdef\@doiabbr{modelling}
	\gdef\@ISSN{2673-3951}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{molbank}{%
	\gdef\@journal{molbank}
	\gdef\@journalfull{Molbank}
	\gdef\@journalshort{Molbank}
	\gdef\@doiabbr{M}
	\gdef\@ISSN{1422-8599}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{molecules}{%
	\gdef\@journal{molecules}
	\gdef\@journalfull{Molecules}
	\gdef\@journalshort{Molecules}
	\gdef\@doiabbr{molecules}
	\gdef\@ISSN{1420-3049}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mollusca}{%
	\gdef\@journal{mollusca}
	\gdef\@journalfull{Mollusca}
	\gdef\@journalshort{Mollusca}
	\gdef\@doiabbr{mollusca}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mps}{%
	\gdef\@journal{mps}
	\gdef\@journalfull{Methods and Protocols}
	\gdef\@journalshort{Methods Protoc.}
	\gdef\@doiabbr{mps}
	\gdef\@ISSN{2409-9279}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{msf}{%
	\gdef\@journal{msf}
	\gdef\@journalfull{Medical Sciences Forum}
	\gdef\@journalshort{Med. Sci. Forum}
	\gdef\@doiabbr{msf}
	\gdef\@ISSN{2673-9992}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mti}{%
	\gdef\@journal{mti}
	\gdef\@journalfull{Multimodal Technologies and Interaction}
	\gdef\@journalshort{Multimodal Technol. Interact.}
	\gdef\@doiabbr{mti}
	\gdef\@ISSN{2414-4088}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{multimedia}{%
	\gdef\@journal{multimedia}
	\gdef\@journalfull{Multimedia}
	\gdef\@journalshort{Multimedia}
	\gdef\@doiabbr{multimedia}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{muscles}{%
	\gdef\@journal{muscles}
	\gdef\@journalfull{Muscles}
	\gdef\@journalshort{Muscles}
	\gdef\@doiabbr{muscles}
	\gdef\@ISSN{2813-0413}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{musculoskeletsci}{%
	\gdef\@journal{musculoskeletsci}
	\gdef\@journalfull{Musculoskeletal Sciences}
	\gdef\@journalshort{Musculoskelet. Sci.}
	\gdef\@doiabbr{musculoskeletsci}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{mutation}{%
	\gdef\@journal{mutation}
	\gdef\@journalfull{Mutation}
	\gdef\@journalshort{Mutation}
	\gdef\@doiabbr{mutation}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{nanoenergyadv}{%
	\gdef\@journal{nanoenergyadv}
	\gdef\@journalfull{Nanoenergy Advances}
	\gdef\@journalshort{Nanoenergy Adv.}
	\gdef\@doiabbr{nanoenergyadv}
	\gdef\@ISSN{2673-706X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{nanomanufacturing}{%
	\gdef\@journal{nanomanufacturing}
	\gdef\@journalfull{Nanomanufacturing}
	\gdef\@journalshort{Nanomanufacturing}
	\gdef\@doiabbr{nanomanufacturing}
	\gdef\@ISSN{2673-687X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{nanomaterials}{%
	\gdef\@journal{nanomaterials}
	\gdef\@journalfull{Nanomaterials}
	\gdef\@journalshort{Nanomaterials}
	\gdef\@doiabbr{nano}
	\gdef\@ISSN{2079-4991}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ncrna}{%
	\gdef\@journal{ncrna}
	\gdef\@journalfull{Non-Coding RNA}
	\gdef\@journalshort{Non-Coding RNA}
	\gdef\@doiabbr{ncrna}
	\gdef\@ISSN{2311-553X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ndt}{%
	\gdef\@journal{ndt}
	\gdef\@journalfull{NDT}
	\gdef\@journalshort{NDT}
	\gdef\@doiabbr{ndt}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{network}{%
	\gdef\@journal{network}
	\gdef\@journalfull{Network}
	\gdef\@journalshort{Network}
	\gdef\@doiabbr{network}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{neuroglia}{%
	\gdef\@journal{neuroglia}
	\gdef\@journalfull{Neuroglia}
	\gdef\@journalshort{Neuroglia}
	\gdef\@doiabbr{neuroglia}
	\gdef\@ISSN{2571-6980}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{neuroimaging}{%
	\gdef\@journal{neuroimaging}
	\gdef\@journalfull{Neuroimaging}
	\gdef\@journalshort{Neuroimaging}
	\gdef\@doiabbr{neuroimaging}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{neurolint}{%
	\gdef\@journal{neurolint}
	\gdef\@journalfull{Neurology International}
	\gdef\@journalshort{Neurol. Int.}
	\gdef\@doiabbr{neurolint}
	\gdef\@ISSN{2035-8377}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{neurosci}{%
	\gdef\@journal{neurosci}
	\gdef\@journalfull{NeuroSci}
	\gdef\@journalshort{NeuroSci}
	\gdef\@doiabbr{neurosci}
	\gdef\@ISSN{2673-4087}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{nitrogen}{%
	\gdef\@journal{nitrogen}
	\gdef\@journalfull{Nitrogen}
	\gdef\@journalshort{Nitrogen}
	\gdef\@doiabbr{nitrogen}
	\gdef\@ISSN{2504-3129}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{numbertheory}{%
	\gdef\@journal{numbertheory}
	\gdef\@journalfull{Number Theory}
	\gdef\@journalshort{Number Theory}
	\gdef\@doiabbr{numbertheory}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{nursrep}{%
	\gdef\@journal{nursrep}
	\gdef\@journalfull{Nursing Reports}
	\gdef\@journalshort{Nurs. Rep.}
	\gdef\@doiabbr{nursrep}
	\gdef\@ISSN{2039-4403}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{nutraceuticals}{%
	\gdef\@journal{nutraceuticals}
	\gdef\@journalfull{Nutraceuticals}
	\gdef\@journalshort{Nutraceuticals}
	\gdef\@doiabbr{nutraceuticals}
	\gdef\@ISSN{1661-3821}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{nutrients}{%
	\gdef\@journal{nutrients}
	\gdef\@journalfull{Nutrients}
	\gdef\@journalshort{Nutrients}
	\gdef\@doiabbr{nu}
	\gdef\@ISSN{2072-6643}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{obesities}{%
	\gdef\@journal{obesities}
	\gdef\@journalfull{Obesities}
	\gdef\@journalshort{Obesities}
	\gdef\@doiabbr{obesities}
	\gdef\@ISSN{2673-4168}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{occuphealth}{%
	\gdef\@journal{occuphealth}
	\gdef\@journalfull{Occupational Health}
	\gdef\@journalshort{Occup. Health}
	\gdef\@doiabbr{occuphealth}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{oceans}{%
	\gdef\@journal{oceans}
	\gdef\@journalfull{Oceans}
	\gdef\@journalshort{Oceans}
	\gdef\@doiabbr{oceans}
	\gdef\@ISSN{2673-1924}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ohbm}{%
	\gdef\@journal{ohbm}
	\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}
	\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balanc. Med.}
	\gdef\@doiabbr{ohbm}
	\gdef\@ISSN{2504-463X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{onco}{%
	\gdef\@journal{onco}
	\gdef\@journalfull{Onco}
	\gdef\@journalshort{Onco}
	\gdef\@doiabbr{onco}
	\gdef\@ISSN{2673-7523}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{opermanag}{%
	\gdef\@journal{opermanag}
	\gdef\@journalfull{Operations Management}
	\gdef\@journalshort{Oper. Manag.}
	\gdef\@doiabbr{opermanag}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{optics}{%
	\gdef\@journal{optics}
	\gdef\@journalfull{Optics}
	\gdef\@journalshort{Optics}
	\gdef\@doiabbr{opt}
	\gdef\@ISSN{2673-3269}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{optoelectronics}{%
	\gdef\@journal{optoelectronics}
	\gdef\@journalfull{Optoelectronics}
	\gdef\@journalshort{Optoelectronics}
	\gdef\@doiabbr{optoelectronics}
	\gdef\@ISSN{3043-1700}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{oral}{%
	\gdef\@journal{oral}
	\gdef\@journalfull{Oral}
	\gdef\@journalshort{Oral}
	\gdef\@doiabbr{oral}
	\gdef\@ISSN{2673-6373}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{organics}{%
	\gdef\@journal{organics}
	\gdef\@journalfull{Organics}
	\gdef\@journalshort{Organics}
	\gdef\@doiabbr{org}
	\gdef\@ISSN{2673-401X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{organoids}{%
	\gdef\@journal{organoids}
	\gdef\@journalfull{Organoids}
	\gdef\@journalshort{Organoids}
	\gdef\@doiabbr{organoids}
	\gdef\@ISSN{2674-1172}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{osteology}{%
	\gdef\@journal{osteology}
	\gdef\@journalfull{Osteology}
	\gdef\@journalshort{Osteology}
	\gdef\@doiabbr{osteology}
	\gdef\@ISSN{2673-4036}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{oxygen}{%
	\gdef\@journal{oxygen}
	\gdef\@journalfull{Oxygen}
	\gdef\@journalshort{Oxygen}
	\gdef\@doiabbr{oxygen}
	\gdef\@ISSN{2673-9801}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pandemics}{%
	\gdef\@journal{pandemics}
	\gdef\@journalfull{Pandemics}
	\gdef\@journalshort{Pandemics}
	\gdef\@doiabbr{pandemics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{parasites}{%
	\gdef\@journal{parasites}
	\gdef\@journalfull{Parasites}
	\gdef\@journalshort{Parasites}
	\gdef\@doiabbr{parasites}
	\gdef\@ISSN{2673-5946}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{parasitologia}{%
	\gdef\@journal{parasitologia}
	\gdef\@journalfull{Parasitologia}
	\gdef\@journalshort{Parasitologia}
	\gdef\@doiabbr{parasitologia}
	\gdef\@ISSN{2673-6772}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{particles}{%
	\gdef\@journal{particles}
	\gdef\@journalfull{Particles}
	\gdef\@journalshort{Particles}
	\gdef\@doiabbr{particles}
	\gdef\@ISSN{2571-712X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pathogens}{%
	\gdef\@journal{pathogens}
	\gdef\@journalfull{Pathogens}
	\gdef\@journalshort{Pathogens}
	\gdef\@doiabbr{pathogens}
	\gdef\@ISSN{2076-0817}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pathophysiology}{%
	\gdef\@journal{pathophysiology}
	\gdef\@journalfull{Pathophysiology}
	\gdef\@journalshort{Pathophysiology}
	\gdef\@doiabbr{pathophysiology}
	\gdef\@ISSN{0928-4680}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{peacestud}{%
	\gdef\@journal{peacestud}
	\gdef\@journalfull{Peace Studies}
	\gdef\@journalshort{Peace Stud.}
	\gdef\@doiabbr{peacestud}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{pediatrrep}{%
	\gdef\@journal{pediatrrep}
	\gdef\@journalfull{Pediatric Reports}
	\gdef\@journalshort{Pediatr. Rep.}
	\gdef\@doiabbr{pediatric}
	\gdef\@ISSN{2036-7503}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pets}{%
	\gdef\@journal{pets}
	\gdef\@journalfull{Pets}
	\gdef\@journalshort{Pets}
	\gdef\@doiabbr{pets}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pharmaceuticals}{%
	\gdef\@journal{pharmaceuticals}
	\gdef\@journalfull{Pharmaceuticals}
	\gdef\@journalshort{Pharmaceuticals}
	\gdef\@doiabbr{ph}
	\gdef\@ISSN{1424-8247}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pharmaceutics}{%
	\gdef\@journal{pharmaceutics}
	\gdef\@journalfull{Pharmaceutics}
	\gdef\@journalshort{Pharmaceutics}
	\gdef\@doiabbr{pharmaceutics}
	\gdef\@ISSN{1999-4923}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pharmacoepidemiology}{%
	\gdef\@journal{pharmacoepidemiology}
	\gdef\@journalfull{Pharmacoepidemiology}
	\gdef\@journalshort{Pharmacoepidemiology}
	\gdef\@doiabbr{pharma}
	\gdef\@ISSN{2813-0618}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pharmacy}{%
	\gdef\@journal{pharmacy}
	\gdef\@journalfull{Pharmacy}
	\gdef\@journalshort{Pharmacy}
	\gdef\@doiabbr{pharmacy}
	\gdef\@ISSN{2226-4787}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{phc}{%
	\gdef\@journal{phc}
	\gdef\@journalfull{Primary and Hospital Care}
	\gdef\@journalshort{Prim. Hosp. Care}
	\gdef\@doiabbr{phc}
	\gdef\@ISSN{3042-9897}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{philosophies}{%
	\gdef\@journal{philosophies}
	\gdef\@journalfull{Philosophies}
	\gdef\@journalshort{Philosophies}
	\gdef\@doiabbr{philosophies}
	\gdef\@ISSN{2409-9287}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{photochem}{%
	\gdef\@journal{photochem}
	\gdef\@journalfull{Photochem}
	\gdef\@journalshort{Photochem}
	\gdef\@doiabbr{photochem}
	\gdef\@ISSN{2673-7256}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{photonics}{%
	\gdef\@journal{photonics}
	\gdef\@journalfull{Photonics}
	\gdef\@journalshort{Photonics}
	\gdef\@doiabbr{photonics}
	\gdef\@ISSN{2304-6732}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{photovoltaics}{%
	\gdef\@journal{photovoltaics}
	\gdef\@journalfull{Photovoltaics}
	\gdef\@journalshort{Photovoltaics}
	\gdef\@doiabbr{photovoltaics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{phycology}{%
	\gdef\@journal{phycology}
	\gdef\@journalfull{Phycology}
	\gdef\@journalshort{Phycology}
	\gdef\@doiabbr{phycology}
	\gdef\@ISSN{2673-9410}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{physchem}{%
	\gdef\@journal{physchem}
	\gdef\@journalfull{Physchem}
	\gdef\@journalshort{Physchem}
	\gdef\@doiabbr{physchem}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{physics}{%
	\gdef\@journal{physics}
	\gdef\@journalfull{Physics}
	\gdef\@journalshort{Physics}
	\gdef\@doiabbr{physics}
	\gdef\@ISSN{2624-8174}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{physiologia}{%
	\gdef\@journal{physiologia}
	\gdef\@journalfull{Physiologia}
	\gdef\@journalshort{Physiologia}
	\gdef\@doiabbr{physiologia}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pjm}{%
	\gdef\@journal{pjm}
	\gdef\@journalfull{Pyramid Journal of Medicine}
	\gdef\@journalshort{Pyramid J. Med.}
	\gdef\@doiabbr{pjm}
	\gdef\@ISSN{2612-2332}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{plants}{%
	\gdef\@journal{plants}
	\gdef\@journalfull{Plants}
	\gdef\@journalshort{Plants}
	\gdef\@doiabbr{plants}
	\gdef\@ISSN{2223-7747}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{plasma}{%
	\gdef\@journal{plasma}
	\gdef\@journalfull{Plasma}
	\gdef\@journalshort{Plasma}
	\gdef\@doiabbr{plasma}
	\gdef\@ISSN{2571-6182}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{platforms}{%
	\gdef\@journal{platforms}
	\gdef\@journalfull{Platforms}
	\gdef\@journalshort{Platforms}
	\gdef\@doiabbr{platforms}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pmh}{%
	\gdef\@journal{pmh}
	\gdef\@journalfull{Project Management Horizons}
	\gdef\@journalshort{Proj. Manag. Horiz.}
	\gdef\@doiabbr{pmh}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{pnr}{%
	\gdef\@journal{pnr}
	\gdef\@journalfull{Pediatric Nursing Research}
	\gdef\@journalshort{Pediatr. Nurs. Res.}
	\gdef\@doiabbr{pnr}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{pollutants}{%
	\gdef\@journal{pollutants}
	\gdef\@journalfull{Pollutants}
	\gdef\@journalshort{Pollutants}
	\gdef\@doiabbr{pollutants}
	\gdef\@ISSN{2673-4672}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{polymers}{%
	\gdef\@journal{polymers}
	\gdef\@journalfull{Polymers}
	\gdef\@journalshort{Polymers}
	\gdef\@doiabbr{polym}
	\gdef\@ISSN{2073-4360}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{polysaccharides}{%
	\gdef\@journal{polysaccharides}
	\gdef\@journalfull{Polysaccharides}
	\gdef\@journalshort{Polysaccharides}
	\gdef\@doiabbr{polysaccharides}
	\gdef\@ISSN{2673-4176}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{populations}{%
	\gdef\@journal{populations}
	\gdef\@journalfull{Populations}
	\gdef\@journalshort{Populations}
	\gdef\@doiabbr{populations}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{poultry}{%
	\gdef\@journal{poultry}
	\gdef\@journalfull{Poultry}
	\gdef\@journalshort{Poultry}
	\gdef\@doiabbr{poultry}
	\gdef\@ISSN{2674-1164}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{powders}{%
	\gdef\@journal{powders}
	\gdef\@journalfull{Powders}
	\gdef\@journalshort{Powders}
	\gdef\@doiabbr{powders}
	\gdef\@ISSN{2674-0516}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ppi}{%
	\gdef\@journal{ppi}
	\gdef\@journalfull{Plant Protection Insights}
	\gdef\@journalshort{Plant Prot. Insights}
	\gdef\@doiabbr{ppi}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{precision}{%
	\gdef\@journal{precision}
	\gdef\@journalfull{Precision---Journal of Precision Engineering}
	\gdef\@journalshort{Precision}
	\gdef\@doiabbr{precision}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{precisoncol}{%
	\gdef\@journal{precisoncol}
	\gdef\@journalfull{Precision Oncology}
	\gdef\@journalshort{Precis. Oncol.}
	\gdef\@doiabbr{precisoncol}
	\gdef\@ISSN{3042-7614}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{preprints}{%
	\gdef\@journal{preprints}
	\gdef\@journalfull{Preprints}
	\gdef\@journalshort{Preprints}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{preprintsapa}{%
	\gdef\@journal{preprintsapa}
	\gdef\@journalfull{Preprints}
	\gdef\@journalshort{Preprints}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{preprintschicago}{%
	\gdef\@journal{preprintschicago}
	\gdef\@journalfull{Preprints}
	\gdef\@journalshort{Preprints}
	\gdef\@doiabbr{}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{prevhealthc}{%
	\gdef\@journal{prevhealthc}
	\gdef\@journalfull{Preventive Healthcare}
	\gdef\@journalshort{Prev. Healthc.}
	\gdef\@doiabbr{prevhealthc}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{proceedings}{%
	\gdef\@journal{proceedings}
	\gdef\@journalfull{Proceedings}
	\gdef\@journalshort{Proceedings}
	\gdef\@doiabbr{proceedings}
	\gdef\@ISSN{2504-3900}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{processes}{%
	\gdef\@journal{processes}
	\gdef\@journalfull{Processes}
	\gdef\@journalshort{Processes}
	\gdef\@doiabbr{pr}
	\gdef\@ISSN{2227-9717}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{prosthesis}{%
	\gdef\@journal{prosthesis}
	\gdef\@journalfull{Prosthesis}
	\gdef\@journalshort{Prosthesis}
	\gdef\@doiabbr{prosthesis}
	\gdef\@ISSN{2673-1592}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{proteomes}{%
	\gdef\@journal{proteomes}
	\gdef\@journalfull{Proteomes}
	\gdef\@journalshort{Proteomes}
	\gdef\@doiabbr{proteomes}
	\gdef\@ISSN{2227-7382}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{psf}{%
	\gdef\@journal{psf}
	\gdef\@journalfull{Physical Sciences Forum}
	\gdef\@journalshort{Phys. Sci. Forum}
	\gdef\@doiabbr{psf}
	\gdef\@ISSN{2673-9984}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{psychiatryint}{%
	\gdef\@journal{psychiatryint}
	\gdef\@journalfull{Psychiatry International}
	\gdef\@journalshort{Psychiatry Int.}
	\gdef\@doiabbr{psychiatryint}
	\gdef\@ISSN{2673-5318}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{psychoactives}{%
	\gdef\@journal{psychoactives}
	\gdef\@journalfull{Psychoactives}
	\gdef\@journalshort{Psychoactives}
	\gdef\@doiabbr{psychoactives}
	\gdef\@ISSN{2813-1851}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{psycholint}{%
	\gdef\@journal{psycholint}
	\gdef\@journalfull{Psychology International}
	\gdef\@journalshort{Psychol. Int.}
	\gdef\@doiabbr{psycholint}
	\gdef\@ISSN{2813-9844}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{publications}{%
	\gdef\@journal{publications}
	\gdef\@journalfull{Publications}
	\gdef\@journalshort{Publications}
	\gdef\@doiabbr{publications}
	\gdef\@ISSN{2304-6775}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{purification}{%
	\gdef\@journal{purification}
	\gdef\@journalfull{Purification}
	\gdef\@journalshort{Purification}
	\gdef\@doiabbr{purification}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{quantumrep}{%
	\gdef\@journal{quantumrep}
	\gdef\@journalfull{Quantum Reports}
	\gdef\@journalshort{Quantum Rep.}
	\gdef\@doiabbr{quantum}
	\gdef\@ISSN{2624-960X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{quaternary}{%
	\gdef\@journal{quaternary}
	\gdef\@journalfull{Quaternary}
	\gdef\@journalshort{Quaternary}
	\gdef\@doiabbr{quat}
	\gdef\@ISSN{2571-550X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{qubs}{%
	\gdef\@journal{qubs}
	\gdef\@journalfull{Quantum Beam Science}
	\gdef\@journalshort{Quantum Beam Sci.}
	\gdef\@doiabbr{qubs}
	\gdef\@ISSN{2412-382X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{radiation}{%
	\gdef\@journal{radiation}
	\gdef\@journalfull{Radiation}
	\gdef\@journalshort{Radiation}
	\gdef\@doiabbr{radiation}
	\gdef\@ISSN{2673-592X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{rareearths}{%
	\gdef\@journal{rareearths}
	\gdef\@journalfull{Rare Earths}
	\gdef\@journalshort{Rare Earths}
	\gdef\@doiabbr{rareearths}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{rdt}{%
	\gdef\@journal{rdt}
	\gdef\@journalfull{Rare Diseases and Therapeutics}
	\gdef\@journalshort{Rare Dis. Ther.}
	\gdef\@doiabbr{rdt}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{reactions}{%
	\gdef\@journal{reactions}
	\gdef\@journalfull{Reactions}
	\gdef\@journalshort{Reactions}
	\gdef\@doiabbr{reactions}
	\gdef\@ISSN{2624-781X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{realestate}{%
	\gdef\@journal{realestate}
	\gdef\@journalfull{Real Estate}
	\gdef\@journalshort{Real Estate}
	\gdef\@doiabbr{realestate}
	\gdef\@ISSN{2813-8090}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{receptors}{%
	\gdef\@journal{receptors}
	\gdef\@journalfull{Receptors}
	\gdef\@journalshort{Receptors}
	\gdef\@doiabbr{receptors}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{recycling}{%
	\gdef\@journal{recycling}
	\gdef\@journalfull{Recycling}
	\gdef\@journalshort{Recycling}
	\gdef\@doiabbr{recycling}
	\gdef\@ISSN{2313-4321}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{regeneration}{%
	\gdef\@journal{regeneration}
	\gdef\@journalfull{Regeneration}
	\gdef\@journalshort{Regeneration}
	\gdef\@doiabbr{regeneration}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{religions}{%
	\gdef\@journal{religions}
	\gdef\@journalfull{Religions}
	\gdef\@journalshort{Religions}
	\gdef\@doiabbr{rel}
	\gdef\@ISSN{2077-1444}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{remotesensing}{%
	\gdef\@journal{remotesensing}
	\gdef\@journalfull{Remote Sensing}
	\gdef\@journalshort{Remote Sens.}
	\gdef\@doiabbr{rs}
	\gdef\@ISSN{2072-4292}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{reports}{%
	\gdef\@journal{reports}
	\gdef\@journalfull{Reports}
	\gdef\@journalshort{Reports}
	\gdef\@doiabbr{reports}
	\gdef\@ISSN{2571-841X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{reprodmed}{%
	\gdef\@journal{reprodmed}
	\gdef\@journalfull{Reproductive Medicine}
	\gdef\@journalshort{Reprod. Med.}
	\gdef\@doiabbr{reprodmed}
	\gdef\@ISSN{2673-3897}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{resources}{%
	\gdef\@journal{resources}
	\gdef\@journalfull{Resources}
	\gdef\@journalshort{Resources}
	\gdef\@doiabbr{resources}
	\gdef\@ISSN{2079-9276}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{rheumato}{%
	\gdef\@journal{rheumato}
	\gdef\@journalfull{Rheumato}
	\gdef\@journalshort{Rheumato}
	\gdef\@doiabbr{rheumato}
	\gdef\@ISSN{2674-0621}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{risks}{%
	\gdef\@journal{risks}
	\gdef\@journalfull{Risks}
	\gdef\@journalshort{Risks}
	\gdef\@doiabbr{risks}
	\gdef\@ISSN{2227-9091}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{rjpm}{%
	\gdef\@journal{rjpm}
	\gdef\@journalfull{Romanian Journal of Preventive Medicine}
	\gdef\@journalshort{Rom. J. Prev. Med.}
	\gdef\@doiabbr{rjpm}
	\gdef\@ISSN{3091-101X}
	\gdef\@societyowner{Romanian Society of Preventive Medicine}
	\gdef\@journaltype{ACS}}
\DeclareOption{robotics}{%
	\gdef\@journal{robotics}
	\gdef\@journalfull{Robotics}
	\gdef\@journalshort{Robotics}
	\gdef\@doiabbr{robotics}
	\gdef\@ISSN{2218-6581}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{rsee}{%
	\gdef\@journal{rsee}
	\gdef\@journalfull{Regional Science and Environmental Economics}
	\gdef\@journalshort{Reg. Sci. Environ. Econ.}
	\gdef\@doiabbr{rsee}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{ruminants}{%
	\gdef\@journal{ruminants}
	\gdef\@journalfull{Ruminants}
	\gdef\@journalshort{Ruminants}
	\gdef\@doiabbr{ruminants}
	\gdef\@ISSN{2673-933X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{safety}{%
	\gdef\@journal{safety}
	\gdef\@journalfull{Safety}
	\gdef\@journalshort{Safety}
	\gdef\@doiabbr{safety}
	\gdef\@ISSN{2313-576X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sanpp}{%
	\gdef\@journal{sanpp}
	\gdef\@journalfull{Swiss Archives of Neurology, Psychiatry and Psychotherapy}
	\gdef\@journalshort{Swiss Arch. Neurol. Psychiatry Psychother.}
	\gdef\@doiabbr{sanpp}
	\gdef\@ISSN{2297-7007}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sbf}{%
	\gdef\@journal{sbf}
	\gdef\@journalfull{Sustainable Banking and Finance}
	\gdef\@journalshort{Sustain. Bank. Finance}
	\gdef\@doiabbr{sbf}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{sca}{%
	\gdef\@journal{sca}
	\gdef\@journalfull{Stem Cell Advances}
	\gdef\@journalshort{Stem Cell Adv.}
	\gdef\@doiabbr{sca}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sci}{%
	\gdef\@journal{sci}
	\gdef\@journalfull{Sci}
	\gdef\@journalshort{Sci}
	\gdef\@doiabbr{sci}
	\gdef\@ISSN{2413-4155}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sciedu}{%
	\gdef\@journal{sciedu}
	\gdef\@journalfull{Trends in Science Education}
	\gdef\@journalshort{Trends Sci. Educ.}
	\gdef\@doiabbr{sciedu}
	\gdef\@ISSN{3043-1344}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{scipharm}{%
	\gdef\@journal{scipharm}
	\gdef\@journalfull{Scientia Pharmaceutica}
	\gdef\@journalshort{Sci. Pharm.}
	\gdef\@doiabbr{scipharm}
	\gdef\@ISSN{2218-0532}
	\gdef\@societyowner{\"{O}sterreichische Pharmazeutische Gesellschaft}
	\gdef\@journaltype{ACS}}
\DeclareOption{sclerosis}{%
	\gdef\@journal{sclerosis}
	\gdef\@journalfull{Sclerosis}
	\gdef\@journalshort{Sclerosis}
	\gdef\@doiabbr{sclerosis}
	\gdef\@ISSN{2813-3064}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{seeds}{%
	\gdef\@journal{seeds}
	\gdef\@journalfull{Seeds}
	\gdef\@journalshort{Seeds}
	\gdef\@doiabbr{seeds}
	\gdef\@ISSN{2674-1024}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sensors}{%
	\gdef\@journal{sensors}
	\gdef\@journalfull{Sensors}
	\gdef\@journalshort{Sensors}
	\gdef\@doiabbr{s}
	\gdef\@ISSN{1424-8220}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{senssyst}{%
	\gdef\@journal{senssyst}
	\gdef\@journalfull{Sensory Systems}
	\gdef\@journalshort{Sens. Syst.}
	\gdef\@doiabbr{senssyst}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}	
\DeclareOption{separations}{%
	\gdef\@journal{separations}
	\gdef\@journalfull{Separations}
	\gdef\@journalshort{Separations}
	\gdef\@doiabbr{separations}
	\gdef\@ISSN{2297-8739}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sexes}{%
	\gdef\@journal{sexes}
	\gdef\@journalfull{Sexes}
	\gdef\@journalshort{Sexes}
	\gdef\@doiabbr{sexes}
	\gdef\@ISSN{2411-5118}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sgf}{%
	\gdef\@journal{sgf}
	\gdef\@journalfull{Surgery in Geriatrics and Frailty}
	\gdef\@journalshort{Surg. Geriatr. Frailty}
	\gdef\@doiabbr{sgf}
	\gdef\@ISSN{3035-5478}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{shi}{%
	\gdef\@journal{shi}
	\gdef\@journalfull{Semiconductors and Heterogeneous Integration}
	\gdef\@journalshort{Semicond. Heterog. Integr.}
	\gdef\@doiabbr{shi}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{signals}{%
	\gdef\@journal{signals}
	\gdef\@journalfull{Signals}
	\gdef\@journalshort{Signals}
	\gdef\@doiabbr{signals}
	\gdef\@ISSN{2624-6120}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sinusitis}{%
	\gdef\@journal{sinusitis}
	\gdef\@journalfull{Sinusitis}
	\gdef\@journalshort{Sinusitis}
	\gdef\@doiabbr{sinusitis}
	\gdef\@ISSN{2309-107X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{siuj}{%
	\gdef\@journal{siuj}
	\gdef\@journalfull{Soci\'{e}t\'{e} Internationale d'Urologie Journal}
	\gdef\@journalshort{Soc. Int. Urol. J.}
	\gdef\@doiabbr{siuj}
	\gdef\@ISSN{2563-6499}
	\gdef\@societyowner{Soci\'{e}t\'{e} Internationale d'Urologie}
	\gdef\@journaltype{ACS}}
\DeclareOption{skins}{%
	\gdef\@journal{skins}
	\gdef\@journalfull{Skins}
	\gdef\@journalshort{Skins}
	\gdef\@doiabbr{skins}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{smartcities}{%
	\gdef\@journal{smartcities}
	\gdef\@journalfull{Smart Cities}
	\gdef\@journalshort{Smart Cities}
	\gdef\@doiabbr{smartcities}
	\gdef\@ISSN{2624-6511}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{smartfish}{%
	\gdef\@journal{smartfish}
	\gdef\@journalfull{Smart Fisheries}
	\gdef\@journalshort{Smart Fish.}
	\gdef\@doiabbr{smartfish}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{smartgrids}{%
	\gdef\@journal{smartgrids}
	\gdef\@journalfull{Smart Grids}
	\gdef\@journalshort{Smart Grids}
	\gdef\@doiabbr{smartgrids}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sna}{%
	\gdef\@journal{sna}
	\gdef\@journalfull{Sinusitis and Asthma}
	\gdef\@journalshort{Sinusitis Asthma}
	\gdef\@doiabbr{sna}
	\gdef\@ISSN{2624-7003}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{societies}{%
	\gdef\@journal{societies}
	\gdef\@journalfull{Societies}
	\gdef\@journalshort{Societies}
	\gdef\@doiabbr{soc}
	\gdef\@ISSN{2075-4698}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{socsci}{%
	\gdef\@journal{socsci}
	\gdef\@journalfull{Social Sciences}
	\gdef\@journalshort{Soc. Sci.}
	\gdef\@doiabbr{socsci}
	\gdef\@ISSN{2076-0760}
	\gdef\@societyowner{}
	\gdef\@journaltype{Chicago}}
\DeclareOption{software}{%
	\gdef\@journal{software}
	\gdef\@journalfull{Software}
	\gdef\@journalshort{Software}
	\gdef\@doiabbr{software}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{soilsystems}{%
	\gdef\@journal{soilsystems}
	\gdef\@journalfull{Soil Systems}
	\gdef\@journalshort{Soil Syst.}
	\gdef\@doiabbr{soilsystems}
	\gdef\@ISSN{2571-8789}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{solar}{%
	\gdef\@journal{solar}
	\gdef\@journalfull{Solar}
	\gdef\@journalshort{Solar}
	\gdef\@doiabbr{solar}
	\gdef\@ISSN{2673-9941}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{solids}{%
	\gdef\@journal{solids}
	\gdef\@journalfull{Solids}
	\gdef\@journalshort{Solids}
	\gdef\@doiabbr{solids}
	\gdef\@ISSN{2673-6497}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{spectroscj}{%
	\gdef\@journal{spectroscj}
	\gdef\@journalfull{Spectroscopy Journal}
	\gdef\@journalshort{Spectrosc. J.}
	\gdef\@doiabbr{spectroscj}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sports}{%
	\gdef\@journal{sports}
	\gdef\@journalfull{Sports}
	\gdef\@journalshort{Sports}
	\gdef\@doiabbr{sports}
	\gdef\@ISSN{2075-4663}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{standards}{%
	\gdef\@journal{standards}
	\gdef\@journalfull{Standards}
	\gdef\@journalshort{Standards}
	\gdef\@doiabbr{standards}
	\gdef\@ISSN{2305-6703}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{stats}{%
	\gdef\@journal{stats}
	\gdef\@journalfull{Stats}
	\gdef\@journalshort{Stats}
	\gdef\@doiabbr{stats}
	\gdef\@ISSN{2571-905X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{std}{%
	\gdef\@journal{std}
	\gdef\@journalfull{Surgical Techniques Development}
	\gdef\@journalshort{Surg. Tech. Dev.}
	\gdef\@doiabbr{std}
	\gdef\@ISSN{2038-9582}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sti}{%
	\gdef\@journal{sti}
	\gdef\@journalfull{Spatio-Temporal Intelligence}
	\gdef\@journalshort{Spatio-Temporal Intell.}
	\gdef\@doiabbr{sti}
	\gdef\@ISSN{3043-1883}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{stomatology}{%
	\gdef\@journal{stomatology}
	\gdef\@journalfull{Stomatology}
	\gdef\@journalshort{Stomatology}
	\gdef\@doiabbr{stomatology}
	\gdef\@ISSN{3043-2243}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{stratsediment}{%
	\gdef\@journal{stratsediment}
	\gdef\@journalfull{Stratigraphy and Sedimentology}
	\gdef\@journalshort{Stratigr. Sedimentol.}
	\gdef\@doiabbr{stratsediment}
	\gdef\@ISSN{3042-884X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{stresses}{%
	\gdef\@journal{stresses}
	\gdef\@journalfull{Stresses}
	\gdef\@journalshort{Stresses}
	\gdef\@doiabbr{stresses}
	\gdef\@ISSN{2673-7140}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{strokerep}{%
	\gdef\@journal{strokerep}
	\gdef\@journalfull{Stroke Reports}
	\gdef\@journalshort{Stroke Rep.}
	\gdef\@doiabbr{strokerep}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{superintelligence}{%
	\gdef\@journal{superintelligence}
	\gdef\@journalfull{Journal of Superintelligence}
	\gdef\@journalshort{J. Superintelligence}
	\gdef\@doiabbr{superintelligence}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{surfaces}{%
	\gdef\@journal{surfaces}
	\gdef\@journalfull{Surfaces}
	\gdef\@journalshort{Surfaces}
	\gdef\@doiabbr{surfaces}
	\gdef\@ISSN{2571-9637}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{surgeries}{%
	\gdef\@journal{surgeries}
	\gdef\@journalfull{Surgeries}
	\gdef\@journalshort{Surgeries}
	\gdef\@doiabbr{surgeries}
	\gdef\@ISSN{2017-2017}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{susagric}{%
	\gdef\@journal{susagric}
	\gdef\@journalfull{Sustainable Agriculture}
	\gdef\@journalshort{Sustain. Agric.}
	\gdef\@doiabbr{susagric}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{suschem}{%
	\gdef\@journal{suschem}
	\gdef\@journalfull{Sustainable Chemistry}
	\gdef\@journalshort{Sustain. Chem.}
	\gdef\@doiabbr{suschem}
	\gdef\@ISSN{2673-4079}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{susenvmgmt}{%
	\gdef\@journal{susenvmgmt}
	\gdef\@journalfull{Sustainable Environmental Management}
	\gdef\@journalshort{Sustain. Environ. Manag.}
	\gdef\@doiabbr{susenvmgmt}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sustainability}{%
	\gdef\@journal{sustainability}
	\gdef\@journalfull{Sustainability}
	\gdef\@journalshort{Sustainability}
	\gdef\@doiabbr{su}
	\gdef\@ISSN{2071-1050}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sustainfoods}{%
	\gdef\@journal{sustainfoods}
	\gdef\@journalfull{Sustainable Foods}
	\gdef\@journalshort{Sustain. Foods}
	\gdef\@doiabbr{sustainfoods}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{sustainpackag}{%
	\gdef\@journal{sustainpackag}
	\gdef\@journalfull{Sustainable Packaging}
	\gdef\@journalshort{Sustain. Packag.}
	\gdef\@doiabbr{sustainpackag}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{symmetry}{%
	\gdef\@journal{symmetry}
	\gdef\@journalfull{Symmetry}
	\gdef\@journalshort{Symmetry}
	\gdef\@doiabbr{sym}
	\gdef\@ISSN{2073-8994}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{synbio}{%
	\gdef\@journal{synbio}
	\gdef\@journalfull{SynBio}
	\gdef\@journalshort{SynBio}
	\gdef\@doiabbr{synbio}
	\gdef\@ISSN{2674-0583}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{systems}{%
	\gdef\@journal{systems}
	\gdef\@journalfull{Systems}
	\gdef\@journalshort{Systems}
	\gdef\@doiabbr{systems}
	\gdef\@ISSN{2079-8954}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{tae}{%
	\gdef\@journal{tae}
	\gdef\@journalfull{Theoretical and Applied Ergonomics}
	\gdef\@journalshort{Theor. Appl. Ergon.}
	\gdef\@doiabbr{tae}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{targets}{%
	\gdef\@journal{targets}
	\gdef\@journalfull{Targets}
	\gdef\@journalshort{Targets}
	\gdef\@doiabbr{targets}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{taxonomy}{%
	\gdef\@journal{taxonomy}
	\gdef\@journalfull{Taxonomy}
	\gdef\@journalshort{Taxonomy}
	\gdef\@doiabbr{taxonomy}
	\gdef\@ISSN{2673-6500}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{technologies}{%
	\gdef\@journal{technologies}
	\gdef\@journalfull{Technologies}
	\gdef\@journalshort{Technologies}
	\gdef\@doiabbr{technologies}
	\gdef\@ISSN{2227-7080}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{telecom}{%
	\gdef\@journal{telecom}
	\gdef\@journalfull{Telecom}
	\gdef\@journalshort{Telecom}
	\gdef\@doiabbr{telecom}
	\gdef\@ISSN{2673-4001}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{Test}
	\gdef\@journalshort{Test}
	\gdef\@doiabbr{test}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{textiles}{%
	\gdef\@journal{textiles}
	\gdef\@journalfull{Textiles}
	\gdef\@journalshort{Textiles}
	\gdef\@doiabbr{textiles}
	\gdef\@ISSN{2673-7248}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{thalassrep}{%
	\gdef\@journal{thalassrep}
	\gdef\@journalfull{Thalassemia Reports}
	\gdef\@journalshort{Thalass. Rep.}
	\gdef\@doiabbr{thalassrep}
	\gdef\@ISSN{2039-4365}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{therapeutics}{%
	\gdef\@journal{therapeutics}
	\gdef\@journalfull{Therapeutics}
	\gdef\@journalshort{Therapeutics}
	\gdef\@doiabbr{therapeutics}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{thermo}{%
	\gdef\@journal{thermo}
	\gdef\@journalfull{Thermo}
	\gdef\@journalshort{Thermo}
	\gdef\@doiabbr{thermo}
	\gdef\@ISSN{2673-7264}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{timespace}{%
	\gdef\@journal{timespace}
	\gdef\@journalfull{Time and Space}
	\gdef\@journalshort{Time Space}
	\gdef\@doiabbr{timespace}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{tomography}{%
	\gdef\@journal{tomography}
	\gdef\@journalfull{Tomography}
	\gdef\@journalshort{Tomography}
	\gdef\@doiabbr{tomography}
	\gdef\@ISSN{2379-139X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{totalenviron}{%
	\gdef\@journal{totalenviron}
	\gdef\@journalfull{Total Environment}
	\gdef\@journalshort{Total Environ.}
	\gdef\@doiabbr{totalenviron}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{tourismhosp}{%
	\gdef\@journal{tourismhosp}
	\gdef\@journalfull{Tourism and Hospitality}
	\gdef\@journalshort{Tour. Hosp.}
	\gdef\@doiabbr{tourhosp}
	\gdef\@ISSN{2673-5768}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{toxics}{%
	\gdef\@journal{toxics}
	\gdef\@journalfull{Toxics}
	\gdef\@journalshort{Toxics}
	\gdef\@doiabbr{toxics}
	\gdef\@ISSN{2305-6304}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{toxins}{%
	\gdef\@journal{toxins}
	\gdef\@journalfull{Toxins}
	\gdef\@journalshort{Toxins}
	\gdef\@doiabbr{toxins}
	\gdef\@ISSN{2072-6651}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{tph}{%
	\gdef\@journal{tph}
	\gdef\@journalfull{Trends in Public Health}
	\gdef\@journalshort{Trends Public Health}
	\gdef\@doiabbr{tph}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{transplantology}{%
	\gdef\@journal{transplantology}
	\gdef\@journalfull{Transplantology}
	\gdef\@journalshort{Transplantology}
	\gdef\@doiabbr{transplantology}
	\gdef\@ISSN{2673-3943}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{transportation}{%
	\gdef\@journal{transportation}
	\gdef\@journalfull{Transportation}
	\gdef\@journalshort{Transportation}
	\gdef\@doiabbr{transportation}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{traumacare}{%
	\gdef\@journal{traumacare}
	\gdef\@journalfull{Trauma Care}
	\gdef\@journalshort{Trauma Care}
	\gdef\@doiabbr{traumacare}
	\gdef\@ISSN{2673-866X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{traumas}{%
	\gdef\@journal{traumas}
	\gdef\@journalfull{Traumas}
	\gdef\@journalshort{Traumas}
	\gdef\@doiabbr{traumas}
	\gdef\@ISSN{2673-7477}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{treeres}{%
	\gdef\@journal{treeres}
	\gdef\@journalfull{Tree Research}
	\gdef\@journalshort{Tree Res.}
	\gdef\@doiabbr{treeres}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{tri}{%
	\gdef\@journal{tri}
	\gdef\@journalfull{Tea Research and Innovation}
	\gdef\@journalshort{Tea Res. Innov.}
	\gdef\@doiabbr{tri}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{tropicalmed}{%
	\gdef\@journal{tropicalmed}
	\gdef\@journalfull{Tropical Medicine and Infectious Disease}
	\gdef\@journalshort{Trop. Med. Infect. Dis.}
	\gdef\@doiabbr{tropicalmed}
	\gdef\@ISSN{2414-6366}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{universe}{%
	\gdef\@journal{universe}
	\gdef\@journalfull{Universe}
	\gdef\@journalshort{Universe}
	\gdef\@doiabbr{universe}
	\gdef\@ISSN{2218-1997}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{urbansci}{%
	\gdef\@journal{urbansci}
	\gdef\@journalfull{Urban Science}
	\gdef\@journalshort{Urban Sci.}
	\gdef\@doiabbr{urbansci}
	\gdef\@ISSN{2413-8851}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{uro}{%
	\gdef\@journal{uro}
	\gdef\@journalfull{Uro}
	\gdef\@journalshort{Uro}
	\gdef\@doiabbr{uro}
	\gdef\@ISSN{2673-4397}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{vaccines}{%
	\gdef\@journal{vaccines}
	\gdef\@journalfull{Vaccines}
	\gdef\@journalshort{Vaccines}
	\gdef\@doiabbr{vaccines}
	\gdef\@ISSN{2076-393X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{vehicles}{%
	\gdef\@journal{vehicles}
	\gdef\@journalfull{Vehicles}
	\gdef\@journalshort{Vehicles}
	\gdef\@doiabbr{vehicles}
	\gdef\@ISSN{2624-8921}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{veinslymphat}{%
	\gdef\@journal{veinslymphat}
	\gdef\@journalfull{Veins and Lymphatics}
	\gdef\@journalshort{Veins Lymphat.}
	\gdef\@doiabbr{veinslymphat}
	\gdef\@ISSN{2279-7483}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{venereology}{%
	\gdef\@journal{venereology}
	\gdef\@journalfull{Venereology}
	\gdef\@journalshort{Venereology}
	\gdef\@doiabbr{venereology}
	\gdef\@ISSN{2674-0710}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{vetsci}{%
	\gdef\@journal{vetsci}
	\gdef\@journalfull{Veterinary Sciences}
	\gdef\@journalshort{Vet. Sci.}
	\gdef\@doiabbr{vetsci}
	\gdef\@ISSN{2306-7381}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{vibration}{%
	\gdef\@journal{vibration}
	\gdef\@journalfull{Vibration}
	\gdef\@journalshort{Vibration}
	\gdef\@doiabbr{vibration}
	\gdef\@ISSN{2571-631X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{virtualworlds}{%
	\gdef\@journal{virtualworlds}
	\gdef\@journalfull{Virtual Worlds}
	\gdef\@journalshort{Virtual Worlds}
	\gdef\@doiabbr{virtualworlds}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{viruses}{%
	\gdef\@journal{viruses}
	\gdef\@journalfull{Viruses}
	\gdef\@journalshort{Viruses}
	\gdef\@doiabbr{v}
	\gdef\@ISSN{1999-4915}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{vision}{%
	\gdef\@journal{vision}
	\gdef\@journalfull{Vision}
	\gdef\@journalshort{Vision}
	\gdef\@doiabbr{vision}
	\gdef\@ISSN{2411-5150}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{vsd}{%
	\gdef\@journal{vsd}
	\gdef\@journalfull{Veterinary Science Development}
	\gdef\@journalshort{Vet. Sci. Dev.}
	\gdef\@doiabbr{vsd}
	\gdef\@ISSN{2001-0370}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{waste}{%
	\gdef\@journal{waste}
	\gdef\@journalfull{Waste}
	\gdef\@journalshort{Waste}
	\gdef\@doiabbr{waste}
	\gdef\@ISSN{2813-0391}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{water}{%
	\gdef\@journal{water}
	\gdef\@journalfull{Water}
	\gdef\@journalshort{Water}
	\gdef\@doiabbr{w}
	\gdef\@ISSN{2073-4441}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{welding}{%
	\gdef\@journal{welding}
	\gdef\@journalfull{Welding}
	\gdef\@journalshort{Welding}
	\gdef\@doiabbr{welding}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{wem}{%
	\gdef\@journal{wem}
	\gdef\@journalfull{Wildlife Ecology and Management}
	\gdef\@journalshort{Wildl. Ecol. Manag.}
	\gdef\@doiabbr{wem}
	\gdef\@ISSN{1234-4321}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{wetlres}{%
	\gdef\@journal{wetlres}
	\gdef\@journalfull{Wetland Research}
	\gdef\@journalshort{Wetl. Res.}
	\gdef\@doiabbr{wetlres}
	\gdef\@ISSN{}
	\gdef\@societyowner{}	
	\gdef\@journaltype{ACS}}
\DeclareOption{wevj}{%
	\gdef\@journal{wevj}
	\gdef\@journalfull{World Electric Vehicle Journal}
	\gdef\@journalshort{World Electr. Veh. J.}
	\gdef\@doiabbr{wevj}
	\gdef\@ISSN{2032-6653}
	\gdef\@societyowner{World Electric Vehicle Association}
	\gdef\@journaltype{ACS}}
\DeclareOption{wild}{%
	\gdef\@journal{wild}
	\gdef\@journalfull{Wild}
	\gdef\@journalshort{Wild}
	\gdef\@doiabbr{wild}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{wind}{%
	\gdef\@journal{wind}
	\gdef\@journalfull{Wind}
	\gdef\@journalshort{Wind}
	\gdef\@doiabbr{wind}
	\gdef\@ISSN{2674-032X}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{winestud}{%
	\gdef\@journal{winestud}
	\gdef\@journalfull{Wine Studies}
	\gdef\@journalshort{Wine Stud.}
	\gdef\@doiabbr{winestud}
	\gdef\@ISSN{2039-4446}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{women}{%
	\gdef\@journal{women}
	\gdef\@journalfull{Women}
	\gdef\@journalshort{Women}
	\gdef\@doiabbr{women}
	\gdef\@ISSN{2673-4184}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{world}{%
	\gdef\@journal{world}
	\gdef\@journalfull{World}
	\gdef\@journalshort{World}
	\gdef\@doiabbr{world}
	\gdef\@ISSN{2673-4060}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{xmanagement}{%
	\gdef\@journal{xmanagement}
	\gdef\@journalfull{Xmanagement}
	\gdef\@journalshort{Xmanagement}
	\gdef\@doiabbr{xmanagement}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{xscience}{%
	\gdef\@journal{xscience}
	\gdef\@journalfull{Xscience}
	\gdef\@journalshort{Xscience}
	\gdef\@doiabbr{xscience}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{youth}{%
	\gdef\@journal{youth}
	\gdef\@journalfull{Youth}
	\gdef\@journalshort{Youth}
	\gdef\@doiabbr{youth}
	\gdef\@ISSN{2673-995X}
	\gdef\@societyowner{}
	\gdef\@journaltype{APA}}
\DeclareOption{zoonoticdis}{%
	\gdef\@journal{zoonoticdis}
	\gdef\@journalfull{Zoonotic Diseases}
	\gdef\@journalshort{Zoonotic Dis.}
	\gdef\@doiabbr{zoonoticdis}
	\gdef\@ISSN{2813-0227}
	\gdef\@societyowner{}
	\gdef\@journaltype{ACS}}
\DeclareOption{zoos}{%
	\gdef\@journal{zoos}
	\gdef\@journalfull{Zoos}
	\gdef\@journalshort{Zoos}
	\gdef\@doiabbr{zoos}
	\gdef\@ISSN{}
	\gdef\@societyowner{}	
	\gdef\@journaltype{ACS}}

==> Definitions/luatex-core.tex <==
%% Updated on 28 August 2026
%% LuaLaTeX core — always loaded by mdpi-luatex.cls (Definitions/luatex-core.tex).
%% Pagella-missing character mappings: Definitions/unicode-luatex.tex (class option unicode).
%% Check: python _check_unicode_needed.py <main>.tex
\RequirePackage{newunicodechar}
\newfontfamily\mdpiextfont{Times New Roman}[
  BoldFont = {Times New Roman Bold},
  ItalicFont = {Times New Roman Italic},
  BoldItalicFont = {Times New Roman Bold Italic},
]
%% Preserve NFSS series/shape so text \textbf/\textit/\bfseries\textit work.
\makeatletter
\DeclareRobustCommand{\mdpiextchar}[1]{%
  \begingroup
    \let\mdpi@ext@series\f@series
    \let\mdpi@ext@shape\f@shape
    \mdpiextfont
    \fontseries{\mdpi@ext@series}%
    \fontshape{\mdpi@ext@shape}%
    \selectfont
    #1%
  \endgroup
}
%% Circled digits: Pagella and Times New Roman both lack U+2460--U+2468.
%% STIX ships with TeX Live and has real glyphs for them. Synthesising the
%% circle with \textcircled instead emits a Figure structure element carrying
%% no Alt/ActualText, which fails PDF/UA-2 (a Figure must have one of them),
%% and it drops the code point from the text layer.
\newfontfamily\mdpicirclefont{STIX-Regular.otf}[
  BoldFont = {STIX-Bold.otf},
  ItalicFont = {STIX-Italic.otf},
  BoldItalicFont = {STIX-BoldItalic.otf},
]
\DeclareRobustCommand{\mdpicirclechar}[1]{%
  \begingroup
    \let\mdpi@ext@series\f@series
    \let\mdpi@ext@shape\f@shape
    \mdpicirclefont
    \fontseries{\mdpi@ext@series}%
    \fontshape{\mdpi@ext@shape}%
    \selectfont
    #1%
  \endgroup
}
%% Pagella Math lacks misc symbols (U+25A0--U+27CD, U+2605, wasysym math, etc.).
%% Do NOT use a second \setmathfont (e.g. XITS Math): it rewires the math stack.
%% Fallback: \text{} + DejaVu Sans / STIX Two Math; code points are decimal Unicode.
\newfontfamily\mdpimathsymfont{DejaVu Sans}
\newfontfamily\mdpimathsymfontext{STIX Two Math}
%% Math-mode Unicode fallback (newunicodechar is text-only).
%% Default letter-like italic; honour upright/bold via mathfamattr or classic \fam.
\ExplSyntaxOn
\bool_new:N \l__mdpi_ext_bold_bool
\bool_new:N \l__mdpi_ext_up_bool
\int_new:N \g__mdpi_ext_fam_rm_int
\int_new:N \g__mdpi_ext_fam_bf_int
\int_new:N \g__mdpi_ext_fam_it_int
\int_gset:Nn \g__mdpi_ext_fam_rm_int { 5 }
\int_gset:Nn \g__mdpi_ext_fam_bf_int { 6 }
\int_gset:Nn \g__mdpi_ext_fam_it_int { 7 }
%% Decide style while still in math (\fam / mathfamattr are valid only there).
\cs_new_protected:Npn \__mdpi_ext_mathstyleselect_decide:
  {
    \bool_set_false:N \l__mdpi_ext_bold_bool
    \bool_set_false:N \l__mdpi_ext_up_bool
    \bool_if_exist:NT \l__mdpi_boldmath_bool
      {
        \bool_if:NT \l__mdpi_boldmath_bool
          { \bool_set_true:N \l__mdpi_ext_bold_bool }
      }
    \cs_if_exist:NTF \mathfamattr
      {
        \int_compare:nNnTF { \mathfamattr } = { -"7FFFFFFF }
          { \__mdpi_ext_mathstyleselect_fam: }
          { \__mdpi_ext_mathstyleselect_attr: }
      }
      { \__mdpi_ext_mathstyleselect_fam: }
  }
\cs_new_protected:Npn \__mdpi_ext_mathstyleselect_apply:
  {
    \bool_if:NT \l__mdpi_ext_bold_bool { \bfseries }
    \bool_if:NTF \l__mdpi_ext_up_bool { \upshape } { \itshape }
  }
\cs_new_protected:Npn \__mdpi_ext_mathstyleselect_attr:
  {
    \int_case:nnF { \mathfamattr }
      {
        { \c__l_uni_math_attribute_symup_int }
          { \bool_set_true:N \l__mdpi_ext_up_bool }
        { \c__l_uni_math_attribute_symbfup_int }
          {
            \bool_set_true:N \l__mdpi_ext_bold_bool
            \bool_set_true:N \l__mdpi_ext_up_bool
          }
        { \c__l_uni_math_attribute_symbf_int }
          {
            \bool_set_true:N \l__mdpi_ext_bold_bool
            \bool_set_true:N \l__mdpi_ext_up_bool
          }
        { \c__l_uni_math_attribute_symbfit_int }
          { \bool_set_true:N \l__mdpi_ext_bold_bool }
        { \c__l_uni_math_attribute_symit_int }
          { }
        { \c__l_uni_math_attribute_symnormal_int }
          { }
      }
      {
        \cs_if_exist:cT { c__l_uni_math_attribute_symmdpibm_int }
          {
            \int_compare:nNnT
              { \mathfamattr } =
              { \use:c { c__l_uni_math_attribute_symmdpibm_int } }
              { \bool_set_true:N \l__mdpi_ext_bold_bool }
          }
      }
  }
\cs_new_protected:Npn \__mdpi_ext_mathstyleselect_fam:
  {
    \int_compare:nNnTF { \fam } = { \g__mdpi_ext_fam_rm_int }
      { \bool_set_true:N \l__mdpi_ext_up_bool }
      {
        \int_compare:nNnTF { \fam } = { \g__mdpi_ext_fam_bf_int }
          {
            \bool_set_true:N \l__mdpi_ext_bold_bool
            \bool_set_true:N \l__mdpi_ext_up_bool
          }
          {
            \int_compare:nNnTF { \fam } = { \g__mdpi_ext_fam_it_int }
              { }
              {
                \int_compare:nNnT { \fam } > { -1 }
                  { \bool_set_true:N \l__mdpi_ext_up_bool }
              }
          }
      }
  }
\cs_new_protected:Npn \mdpiextmathchar #1
  {
    \__mdpi_ext_mathstyleselect_decide:
    \text
      {
        \mdpiextfont
        \__mdpi_ext_mathstyleselect_apply:
        #1
      }
  }
\cs_new_protected:Npn \__mdpi_mathsym_ord:n #1
  {
    \mathord
      {
        \text
          {
            \mdpimathsymfont
            \char_generate:nn {#1} { 12 }
          }
      }
  }
\cs_new_protected:Npn \__mdpi_mathsym_ord_ext:n #1
  {
    \mathord
      {
        \text
          {
            \mdpimathsymfontext
            \char_generate:nn {#1} { 12 }
          }
      }
  }
\cs_new_protected:Npn \__mdpi_mathsym_rel:n #1
  {
    \mathrel
      {
        \text
          {
            \mdpimathsymfont
            \char_generate:nn {#1} { 12 }
          }
      }
  }
\cs_new_protected:Npn \__mdpi_declare_mathsym_ord:nn #1#2
  {
    \cs_if_exist:NTF #1
      { \RenewDocumentCommand #1 { } { \__mdpi_mathsym_ord:n {#2} } }
      { \NewDocumentCommand #1 { } { \__mdpi_mathsym_ord:n {#2} } }
  }
\cs_new_protected:Npn \__mdpi_declare_mathsym_ord_ext:nn #1#2
  {
    \RenewDocumentCommand #1 { } { \__mdpi_mathsym_ord_ext:n {#2} }
  }
\cs_new_protected:Npn \__mdpi_declare_mathsym_rel:nn #1#2
  {
    \RenewDocumentCommand #1 { } { \__mdpi_mathsym_rel:n {#2} }
  }
\cs_new_protected:Npn \__mdpi_declare_mathsym_ifmmode_ord:Nn #1#2
  {
    \cs_if_exist:cF { mdpi@orig \cs_to_str:N #1 }
      { \cs_set_eq:cN { mdpi@orig \cs_to_str:N #1 } #1 }
    \RenewDocumentCommand #1 { }
      {
        \ifmmode
          \__mdpi_mathsym_ord:n {#2}
        \else
          \use:c { mdpi@orig \cs_to_str:N #1 }
        \fi
      }
  }
\cs_new_protected:Npn \__mdpi_install_mathsym_fallbacks:
  {
    \__mdpi_declare_mathsym_ord:nn \square { 9633 }
    \__mdpi_declare_mathsym_ord:nn \blacksquare { 9632 }
    \__mdpi_declare_mathsym_ord:nn \bigstar { 9733 }
    \__mdpi_declare_mathsym_ord:nn \blacktriangle { 9652 }
    \__mdpi_declare_mathsym_ord:nn \blacktriangledown { 9662 }
    \__mdpi_declare_mathsym_ord:nn \triangledown { 9663 }
    \__mdpi_declare_mathsym_ord_ext:nn \diagup { 10187 }
    \__mdpi_declare_mathsym_ord_ext:nn \diagdown { 10189 }
    \__mdpi_declare_mathsym_rel:nn \vartriangle { 9653 }
    \__mdpi_declare_mathsym_ifmmode_ord:Nn \male { 9794 }
    \__mdpi_declare_mathsym_ifmmode_ord:Nn \female { 9792 }
    \__mdpi_declare_mathsym_ifmmode_ord:Nn \sun { 9788 }
    \__mdpi_declare_mathsym_ifmmode_ord:Nn \rightmoon { 9789 }
    \__mdpi_declare_mathsym_ifmmode_ord:Nn \leftmoon { 9790 }
    \__mdpi_declare_mathsym_ifmmode_ord:Nn \euro { 8364 }
  }
\ExplSyntaxOff
%% #2 must stay outside \lowercase (it would be case-folded along with the ~),
%% and only one \lowercase may do the ~ substitution: a nested second one folds
%% an uppercase target down to its lowercase code point, so \mathcode and \def
%% end up on different characters and the uppercase half silently breaks.
\newcommand\mdpi@mathfallback[2]{%
  \gdef\mdpi@mchar@tmp{%
    \ifmmode
      \mdpiextmathchar{#2}%
    \else
      \mdpiextchar{#2}%
    \fi
  }%
  \begingroup
  \lccode`\~="#1\relax
  \catcode`\~=\active
  \lowercase{%
    \endgroup
    \mathcode`~="8000
    \expandafter\gdef\expandafter~\expandafter{\mdpi@mchar@tmp}%
  }%
}
\AtBeginDocument{%
  \mdpi@mathfallback{A7B0}{Ʞ}% U+A7B0–U+A7BF (Pagella Math lacks glyphs)
  \mdpi@mathfallback{A7B1}{Ʇ}%
  \mdpi@mathfallback{A7B2}{Ʝ}%
  \mdpi@mathfallback{A7B3}{Ꭓ}%
  \mdpi@mathfallback{A7B4}{Ꞵ}%
  \mdpi@mathfallback{A7B5}{ꞵ}%
  \mdpi@mathfallback{A7B6}{Ꞷ}%
  \mdpi@mathfallback{A7B7}{ꞷ}%
  \mdpi@mathfallback{A7B8}{Ꞹ}%
  \mdpi@mathfallback{A7B9}{ꞹ}%
  \mdpi@mathfallback{A7BA}{Ꞻ}%
  \mdpi@mathfallback{A7BB}{ꞻ}%
  \mdpi@mathfallback{A7BC}{Ꞽ}%
  \mdpi@mathfallback{A7BD}{ꞽ}%
  \mdpi@mathfallback{A7BE}{Ꞿ}%
  \mdpi@mathfallback{A7BF}{ꞿ}%
}
\makeatother


==> Definitions/mdpi-extra-langs.tex <==
%% mdpi-extra-langs.tex — babel/fonts bundle (mdpi-luatex.cls option extralangs or \MDPIextralangs)

\ExplSyntaxOn
\cs_new_protected:Npn \mdpi_setup_hebrew:
 {
  \babelprovide[onchar=ids fonts]{hebrew}
  \babelfont[hebrew]{rm}[
    Renderer=HarfBuzz,
    ItalicFont={Times New Roman},
    BoldFont={Times New Roman Bold},
  ]{Times New Roman}
  \providecommand\texthebrew{\foreignlanguage{hebrew}}
  \newfontfamily\hebrewfont{Times New Roman}[
    Script=Hebrew,
    Renderer=HarfBuzz,
    ItalicFont={Times New Roman},
    BoldFont={Times New Roman Bold},
  ]
 }
\cs_new_protected:Npn \mdpi_setup_arabic:
 {
  \babelprovide[onchar=ids fonts]{arabic}
  \babelfont[arabic]{rm}[
    Renderer=HarfBuzz,
    ItalicFont={Times New Roman},
    BoldFont={Times New Roman Bold},
  ]{Times New Roman}
  \providecommand\textarabic{\foreignlanguage{arabic}}
  \newfontfamily\arabicfont{Times New Roman}[
    Script=Arabic,
    Renderer=HarfBuzz,
    ItalicFont={Times New Roman},
    BoldFont={Times New Roman Bold},
  ]
 }
\cs_new_protected:Npn \mdpi_setup_russian:
 {
  \babelprovide[onchar=ids fonts]{russian}
  \babelfont[russian]{rm}[Renderer=HarfBuzz]{Times New Roman}
  \newfontfamily\rufont{Palatino Linotype}[Script=Cyrillic]
 }
\cs_new_protected:Npn \mdpi_setup_cjk:
 {
  \babelprovide[onchar=ids fonts]{chinese-simplified}
  \babelfont[chinese-simplified]{rm}[Renderer=HarfBuzz]{SimSun}
  \newfontfamily\simsun{SimSun}
  \newfontfamily\koreanfont{Malgun Gothic}
 }
\cs_new_protected:Npn \mdpi_setup_extralangs:
 {
  \RequirePackage[bidi=basic,layout=tabular,english]{babel}
  \mdpi_setup_hebrew:
  \mdpi_setup_arabic:
  \mdpi_setup_russian:
  \mdpi_setup_cjk:
  \newfontfamily\rmfont{Times New Roman}
  \newfontfamily\cambria{Cambria Math} % Cambria Math font letters
 }
\ExplSyntaxOff


==> Definitions/unicode-luatex.tex <==
%% Updated on 28 August 2026
%% Pagella-missing character mappings — loaded by mdpi-luatex.cls with class option unicode.
%%   \documentclass[...,unicode]{Definitions/mdpi-luatex}
%% Requires luatex-core.tex (\mdpiextchar, newunicodechar).
%% --- Diacritic compositions (Pagella lacks precomposed glyph) ---
\newunicodechar{ȩ}{\mdpiextchar{ȩ}}  % U+0229
%% Latin Extended Additional U+1E00--U+1EFF
\newunicodechar{Ḁ}{\mdpiextchar{Ḁ}}  % U+1E00
\newunicodechar{ḁ}{\mdpiextchar{ḁ}}  % U+1E01
\newunicodechar{Ḃ}{\mdpiextchar{Ḃ}}  % U+1E02
\newunicodechar{ḃ}{\mdpiextchar{ḃ}}  % U+1E03
\newunicodechar{Ḅ}{\mdpiextchar{Ḅ}}  % U+1E04
\newunicodechar{ḅ}{\mdpiextchar{ḅ}}  % U+1E05
\newunicodechar{Ḇ}{\mdpiextchar{Ḇ}}  % U+1E06
\newunicodechar{ḇ}{\mdpiextchar{ḇ}}  % U+1E07
\newunicodechar{Ḉ}{\mdpiextchar{Ḉ}}  % U+1E08
\newunicodechar{ḉ}{\mdpiextchar{ḉ}}  % U+1E09
\newunicodechar{Ḋ}{\mdpiextchar{Ḋ}}  % U+1E0A
\newunicodechar{ḋ}{\mdpiextchar{ḋ}}  % U+1E0B
\newunicodechar{Ḑ}{\mdpiextchar{Ḑ}}  % U+1E10
\newunicodechar{ḑ}{\mdpiextchar{ḑ}}  % U+1E11
\newunicodechar{Ḓ}{\mdpiextchar{Ḓ}}  % U+1E12
\newunicodechar{ḓ}{\mdpiextchar{ḓ}}  % U+1E13
\newunicodechar{Ḕ}{\mdpiextchar{Ḕ}}  % U+1E14
\newunicodechar{ḕ}{\mdpiextchar{ḕ}}  % U+1E15
\newunicodechar{Ḗ}{\mdpiextchar{Ḗ}}  % U+1E16
\newunicodechar{ḗ}{\mdpiextchar{ḗ}}  % U+1E17
\newunicodechar{Ḙ}{\mdpiextchar{Ḙ}}  % U+1E18
\newunicodechar{ḙ}{\mdpiextchar{ḙ}}  % U+1E19
\newunicodechar{Ḛ}{\mdpiextchar{Ḛ}}  % U+1E1A
\newunicodechar{ḛ}{\mdpiextchar{ḛ}}  % U+1E1B
\newunicodechar{Ḝ}{\mdpiextchar{Ḝ}}  % U+1E1C
\newunicodechar{ḝ}{\mdpiextchar{ḝ}}  % U+1E1D
%\newunicodechar{Ḟ}{\mdpiextchar{Ḟ}}  % U+1E1E
\newunicodechar{Ḟ}{\.{F}}  % U+1E1E
%\newunicodechar{ḟ}{\mdpiextchar{ḟ}}  % U+1E1F
\newunicodechar{ḟ}{\.{f}}  % U+1E1F
%\newunicodechar{Ḡ}{\mdpiextchar{Ḡ}}  % U+1E20
\newunicodechar{Ḡ}{\-{G}}  % U+1E20
\newunicodechar{ḡ}{\mdpiextchar{ḡ}}  % U+1E21
\newunicodechar{ḡ}{\-{g}}  % U+1E21
\newunicodechar{Ḣ}{\mdpiextchar{Ḣ}}  % U+1E22
\newunicodechar{ḣ}{\mdpiextchar{ḣ}}  % U+1E23
\newunicodechar{Ḩ}{\mdpiextchar{Ḩ}}  % U+1E28
\newunicodechar{ḩ}{\mdpiextchar{ḩ}}  % U+1E29
\newunicodechar{Ḭ}{\mdpiextchar{Ḭ}}  % U+1E2C
\newunicodechar{ḭ}{\mdpiextchar{ḭ}}  % U+1E2D
\newunicodechar{Ḱ}{\mdpiextchar{Ḱ}}  % U+1E30
\newunicodechar{ḱ}{\mdpiextchar{ḱ}}  % U+1E31
\newunicodechar{Ḳ}{\mdpiextchar{Ḳ}}  % U+1E32
\newunicodechar{ḳ}{\mdpiextchar{ḳ}}  % U+1E33
\newunicodechar{Ḵ}{\mdpiextchar{Ḵ}}  % U+1E34
\newunicodechar{ḵ}{\mdpiextchar{ḵ}}  % U+1E35
\newunicodechar{Ḻ}{\mdpiextchar{Ḻ}}  % U+1E3A
\newunicodechar{ḻ}{\mdpiextchar{ḻ}}  % U+1E3B
\newunicodechar{Ḽ}{\mdpiextchar{Ḽ}}  % U+1E3C
\newunicodechar{ḽ}{\mdpiextchar{ḽ}}  % U+1E3D
\newunicodechar{Ḿ}{\mdpiextchar{Ḿ}}  % U+1E3E
\newunicodechar{ḿ}{\mdpiextchar{ḿ}}  % U+1E3F
%\newunicodechar{Ṁ}{\mdpiextchar{Ṁ}}  % U+1E40
\newunicodechar{Ṁ}{\.{M}}  % U+1E40
%\newunicodechar{ṁ}{\mdpiextchar{ṁ}}  % U+1E41
\newunicodechar{ṁ}{\.{m}}  % U+1E41
\newunicodechar{Ṉ}{\mdpiextchar{Ṉ}}  % U+1E48
\newunicodechar{ṉ}{\mdpiextchar{ṉ}}  % U+1E49
\newunicodechar{Ṋ}{\mdpiextchar{Ṋ}}  % U+1E4A
\newunicodechar{ṋ}{\mdpiextchar{ṋ}}  % U+1E4B
\newunicodechar{Ṍ}{\mdpiextchar{Ṍ}}  % U+1E4C
\newunicodechar{ṍ}{\mdpiextchar{ṍ}}  % U+1E4D
\newunicodechar{Ṏ}{\mdpiextchar{Ṏ}}  % U+1E4E
\newunicodechar{ṏ}{\mdpiextchar{ṏ}}  % U+1E4F
\newunicodechar{Ṑ}{\mdpiextchar{Ṑ}}  % U+1E50
\newunicodechar{ṑ}{\mdpiextchar{ṑ}}  % U+1E51
\newunicodechar{Ṓ}{\mdpiextchar{Ṓ}}  % U+1E52
\newunicodechar{ṓ}{\mdpiextchar{ṓ}}  % U+1E53
\newunicodechar{Ṕ}{\mdpiextchar{Ṕ}}  % U+1E54
\newunicodechar{ṕ}{\mdpiextchar{ṕ}}  % U+1E55
%\newunicodechar{Ṗ}{\mdpiextchar{Ṗ}}  % U+1E56
\newunicodechar{Ṗ}{\.{P}}  % U+1E56
%\newunicodechar{ṗ}{\mdpiextchar{ṗ}}  % U+1E57
\newunicodechar{ṗ}{\.{p}}  % U+1E57
\newunicodechar{Ṟ}{\mdpiextchar{Ṟ}}  % U+1E5E
\newunicodechar{ṟ}{\mdpiextchar{ṟ}}  % U+1E5F
%\newunicodechar{Ṡ}{\mdpiextchar{Ṡ}}  % U+1E60
\newunicodechar{Ṡ}{\.{S}}  % U+1E60
%\newunicodechar{ṡ}{\mdpiextchar{ṡ}}  % U+1E61
\newunicodechar{ṡ}{\.{s}}  % U+1E61
\newunicodechar{Ṥ}{\mdpiextchar{Ṥ}}  % U+1E64
\newunicodechar{ṥ}{\mdpiextchar{ṥ}}  % U+1E65
\newunicodechar{Ṧ}{\mdpiextchar{Ṧ}}  % U+1E66
\newunicodechar{ṧ}{\mdpiextchar{ṧ}}  % U+1E67
\newunicodechar{Ṩ}{\mdpiextchar{Ṩ}}  % U+1E68
\newunicodechar{ṩ}{\mdpiextchar{ṩ}}  % U+1E69
%\newunicodechar{Ṫ}{\mdpiextchar{Ṫ}}  % U+1E6A
\newunicodechar{Ṫ}{\.{T}}  % U+1E6A
%\newunicodechar{ṫ}{\mdpiextchar{ṫ}}  % U+1E6B
\newunicodechar{ṫ}{\.{t}}  % U+1E6B
\newunicodechar{Ṱ}{\mdpiextchar{Ṱ}}  % U+1E70
\newunicodechar{ṱ}{\mdpiextchar{ṱ}}  % U+1E71
\newunicodechar{Ṳ}{\mdpiextchar{Ṳ}}  % U+1E72
\newunicodechar{ṳ}{\mdpiextchar{ṳ}}  % U+1E73
\newunicodechar{Ṵ}{\mdpiextchar{Ṵ}}  % U+1E74
\newunicodechar{ṵ}{\mdpiextchar{ṵ}}  % U+1E75
\newunicodechar{Ṷ}{\mdpiextchar{Ṷ}}  % U+1E76
\newunicodechar{ṷ}{\mdpiextchar{ṷ}}  % U+1E77
\newunicodechar{Ṹ}{\mdpiextchar{Ṹ}}  % U+1E78
\newunicodechar{ṹ}{\mdpiextchar{ṹ}}  % U+1E79
\newunicodechar{Ṻ}{\mdpiextchar{Ṻ}}  % U+1E7A
\newunicodechar{ṻ}{\mdpiextchar{ṻ}}  % U+1E7B
\newunicodechar{Ṽ}{\mdpiextchar{Ṽ}}  % U+1E7C
\newunicodechar{ṽ}{\mdpiextchar{ṽ}}  % U+1E7D
\newunicodechar{Ṿ}{\mdpiextchar{Ṿ}}  % U+1E7E
\newunicodechar{ṿ}{\mdpiextchar{ṿ}}  % U+1E7F
%\newunicodechar{Ẇ}{\mdpiextchar{Ẇ}}  % U+1E86
\newunicodechar{Ẇ}{\.{W}}  % U+1E86
%\newunicodechar{ẇ}{\mdpiextchar{ẇ}}  % U+1E87
\newunicodechar{ẇ}{\.{w}}  % U+1E87
\newunicodechar{Ẉ}{\mdpiextchar{Ẉ}}  % U+1E88
\newunicodechar{ẉ}{\mdpiextchar{ẉ}}  % U+1E89
%\newunicodechar{Ẋ}{\mdpiextchar{Ẋ}}  % U+1E8A
\newunicodechar{Ẋ}{\.{X}}  % U+1E8A
%\newunicodechar{ẋ}{\mdpiextchar{ẋ}}  % U+1E8B
\newunicodechar{ẋ}{\.{x}}  % U+1E8B
\newunicodechar{Ẍ}{\mdpiextchar{Ẍ}}  % U+1E8C
\newunicodechar{ẍ}{\mdpiextchar{ẍ}}  % U+1E8D
%\newunicodechar{Ẏ}{\mdpiextchar{Ẏ}}  % U+1E8E
\newunicodechar{Ẏ}{\.{Y}}  % U+1E8E
%\newunicodechar{ẏ}{\mdpiextchar{ẏ}}  % U+1E8F
\newunicodechar{ẏ}{\.{y}}  % U+1E8F
%\newunicodechar{Ẑ}{\mdpiextchar{Ẑ}}  % U+1E90
\newunicodechar{Ẑ}{\^{Z}}  % U+1E90
%\newunicodechar{ẑ}{\mdpiextchar{ẑ}}  % U+1E91
\newunicodechar{ẑ}{\^{z}}  % U+1E91
\newunicodechar{Ẕ}{\mdpiextchar{Ẕ}}  % U+1E94
\newunicodechar{ẕ}{\mdpiextchar{ẕ}}  % U+1E95
\newunicodechar{ẖ}{\mdpiextchar{ẖ}}  % U+1E96
\newunicodechar{ẘ}{\mdpiextchar{ẘ}}  % U+1E98
\newunicodechar{ẙ}{\mdpiextchar{ẙ}}  % U+1E99
\newunicodechar{ẚ}{\mdpiextchar{ẚ}}  % U+1E9A
\newunicodechar{ẛ}{\mdpiextchar{ẛ}}  % U+1E9B
\newunicodechar{ẜ}{\mdpiextchar{ẜ}}  % U+1E9C
\newunicodechar{ẝ}{\mdpiextchar{ẝ}}  % U+1E9D
\newunicodechar{ẞ}{\mdpiextchar{ẞ}}  % U+1E9E
\newunicodechar{ẟ}{\mdpiextchar{ẟ}}  % U+1E9F
\newunicodechar{Ỻ}{\mdpiextchar{Ỻ}}  % U+1EFA
\newunicodechar{ỻ}{\mdpiextchar{ỻ}}  % U+1EFB
\newunicodechar{Ỽ}{\mdpiextchar{Ỽ}}  % U+1EFC
\newunicodechar{ỽ}{\mdpiextchar{ỽ}}  % U+1EFD
\newunicodechar{Ỿ}{\mdpiextchar{Ỿ}}  % U+1EFE
\newunicodechar{ỿ}{\mdpiextchar{ỿ}}  % U+1EFF

%% --- Spaces / punctuation (Pagella lacks glyph) ---
\newunicodechar{ }{\quad}  % U+2003 EM SPACE
\newunicodechar{˂}{<}  % U+02C2

%% --- Circled / superscript digits (Pagella lacks glyph) ---
\newunicodechar{①}{\mdpicirclechar{①}}  % U+2460
\newunicodechar{②}{\mdpicirclechar{②}}  % U+2461
\newunicodechar{③}{\mdpicirclechar{③}}  % U+2462
\newunicodechar{④}{\mdpicirclechar{④}}  % U+2463
\newunicodechar{⑤}{\mdpicirclechar{⑤}}  % U+2464
\newunicodechar{⑥}{\mdpicirclechar{⑥}}  % U+2465
\newunicodechar{⑦}{\mdpicirclechar{⑦}}  % U+2466
\newunicodechar{⑧}{\mdpicirclechar{⑧}}  % U+2467
\newunicodechar{⑨}{\mdpicirclechar{⑨}}  % U+2468
%% Superscript 0–9 (Unicode uses U+2070 + U+00B9–U+00B3 + U+2074–U+2079)
\newunicodechar{⁰}{\textsuperscript{0}}  % U+2070
\newunicodechar{¹}{\textsuperscript{1}}  % U+00B9
\newunicodechar{²}{\textsuperscript{2}}  % U+00B2
\newunicodechar{³}{\textsuperscript{3}}  % U+00B3
\newunicodechar{⁴}{\textsuperscript{4}}  % U+2074
\newunicodechar{⁵}{\textsuperscript{5}}  % U+2075
\newunicodechar{⁶}{\textsuperscript{6}}  % U+2076
\newunicodechar{⁷}{\textsuperscript{7}}  % U+2077
\newunicodechar{⁸}{\textsuperscript{8}}  % U+2078
\newunicodechar{⁹}{\textsuperscript{9}}  % U+2079

%% --- Greek with tonos (Pagella lacks precomposed; extfont keeps Unicode) ---
%% Monotonic vowels: U+0386--U+038F, U+0390, U+03AA--U+03AB, U+03AC--U+03CE
\newunicodechar{Ά}{\mdpiextchar{Ά}}  % U+0386
\newunicodechar{Έ}{\mdpiextchar{Έ}}  % U+0388
\newunicodechar{Ή}{\mdpiextchar{Ή}}  % U+0389
\newunicodechar{Ί}{\mdpiextchar{Ί}}  % U+038A
\newunicodechar{Ό}{\mdpiextchar{Ό}}  % U+038C
\newunicodechar{Ύ}{\mdpiextchar{Ύ}}  % U+038E
\newunicodechar{Ώ}{\mdpiextchar{Ώ}}  % U+038F
\newunicodechar{ΐ}{\mdpiextchar{ΐ}}  % U+0390
\newunicodechar{Ϊ}{\mdpiextchar{Ϊ}}  % U+03AA
\newunicodechar{Ϋ}{\mdpiextchar{Ϋ}}  % U+03AB
\newunicodechar{ά}{\mdpiextchar{ά}}  % U+03AC
\newunicodechar{έ}{\mdpiextchar{έ}}  % U+03AD
\newunicodechar{ή}{\mdpiextchar{ή}}  % U+03AE
\newunicodechar{ί}{\mdpiextchar{ί}}  % U+03AF
\newunicodechar{ΰ}{\mdpiextchar{ΰ}}  % U+03B0
\newunicodechar{ϊ}{\mdpiextchar{ϊ}}  % U+03CA
\newunicodechar{ϋ}{\mdpiextchar{ϋ}}  % U+03CB
\newunicodechar{ό}{\mdpiextchar{ό}}  % U+03CC
\newunicodechar{ύ}{\mdpiextchar{ύ}}  % U+03CD
\newunicodechar{ώ}{\mdpiextchar{ώ}}  % U+03CE

%% --- Mathematical alphanumeric symbols → upright text in math/text ---
\newunicodechar{𝐴}{\relax\ifmmode A \else $A$\fi}  % U+1D434
\newunicodechar{𝐵}{\relax\ifmmode B \else $B$\fi}  % U+1D435
\newunicodechar{𝐶}{\relax\ifmmode C \else $C$\fi}  % U+1D436
\newunicodechar{𝐷}{\relax\ifmmode D \else $D$\fi}  % U+1D437
\newunicodechar{𝐸}{\relax\ifmmode E \else $E$\fi}  % U+1D438
\newunicodechar{𝐹}{\relax\ifmmode F \else $F$\fi}  % U+1D439
\newunicodechar{𝐺}{\relax\ifmmode G \else $G$\fi}  % U+1D43A
\newunicodechar{𝐻}{\relax\ifmmode H \else $H$\fi}  % U+1D43B
\newunicodechar{𝐼}{\relax\ifmmode I \else $I$\fi}  % U+1D43C
\newunicodechar{𝐽}{\relax\ifmmode J \else $J$\fi}  % U+1D43D
\newunicodechar{𝐾}{\relax\ifmmode K \else $K$\fi}  % U+1D43E
\newunicodechar{𝐿}{\relax\ifmmode L \else $L$\fi}  % U+1D43F
\newunicodechar{𝑀}{\relax\ifmmode M \else $M$\fi}  % U+1D440
\newunicodechar{𝑁}{\relax\ifmmode N \else $N$\fi}  % U+1D441
\newunicodechar{𝑂}{\relax\ifmmode O \else $O$\fi}  % U+1D442
\newunicodechar{𝑃}{\relax\ifmmode P \else $P$\fi}  % U+1D443
\newunicodechar{𝑄}{\relax\ifmmode Q \else $Q$\fi}  % U+1D444
\newunicodechar{𝑅}{\relax\ifmmode R \else $R$\fi}  % U+1D445
\newunicodechar{𝑆}{\relax\ifmmode S \else $S$\fi}  % U+1D446
\newunicodechar{𝑇}{\relax\ifmmode T \else $T$\fi}  % U+1D447
\newunicodechar{𝑈}{\relax\ifmmode U \else $U$\fi}  % U+1D448
\newunicodechar{𝑉}{\relax\ifmmode V \else $V$\fi}  % U+1D449
\newunicodechar{𝑊}{\relax\ifmmode W \else $W$\fi}  % U+1D44A
\newunicodechar{𝑋}{\relax\ifmmode X \else $X$\fi}  % U+1D44B
\newunicodechar{𝑌}{\relax\ifmmode Y \else $Y$\fi}  % U+1D44C
\newunicodechar{𝑍}{\relax\ifmmode Z \else $Z$\fi}  % U+1D44D
\newunicodechar{𝑎}{\relax\ifmmode a \else $a$\fi}  % U+1D44E
\newunicodechar{𝑏}{\relax\ifmmode b \else $b$\fi}  % U+1D44F
\newunicodechar{𝑐}{\relax\ifmmode c \else $c$\fi}  % U+1D450
\newunicodechar{𝑑}{\relax\ifmmode d \else $d$\fi}  % U+1D451
\newunicodechar{𝑒}{\relax\ifmmode e \else $e$\fi}  % U+1D452
\newunicodechar{𝑓}{\relax\ifmmode f \else $f$\fi}  % U+1D453
\newunicodechar{𝑔}{\relax\ifmmode g \else $g$\fi}  % U+1D454
\newunicodechar{𝑖}{\relax\ifmmode i \else $i$\fi}  % U+1D456
\newunicodechar{𝑗}{\relax\ifmmode j \else $j$\fi}  % U+1D457
\newunicodechar{𝑘}{\relax\ifmmode k \else $k$\fi}  % U+1D458
\newunicodechar{𝑙}{\relax\ifmmode l \else $l$\fi}  % U+1D459
\newunicodechar{𝑚}{\relax\ifmmode m \else $m$\fi}  % U+1D45A
\newunicodechar{𝑛}{\relax\ifmmode n \else $n$\fi}  % U+1D45B
\newunicodechar{𝑜}{\relax\ifmmode o \else $o$\fi}  % U+1D45C
\newunicodechar{𝑝}{\relax\ifmmode p \else $p$\fi}  % U+1D45D
\newunicodechar{𝑞}{\relax\ifmmode q \else $q$\fi}  % U+1D45E
\newunicodechar{𝑟}{\relax\ifmmode r \else $r$\fi}  % U+1D45F
\newunicodechar{𝑠}{\relax\ifmmode s \else $s$\fi}  % U+1D460
\newunicodechar{𝑡}{\relax\ifmmode t \else $t$\fi}  % U+1D461
\newunicodechar{𝑢}{\relax\ifmmode u \else $u$\fi}  % U+1D462
\newunicodechar{𝑣}{\relax\ifmmode v \else $v$\fi}  % U+1D463
\newunicodechar{𝑤}{\relax\ifmmode w \else $w$\fi}  % U+1D464
\newunicodechar{𝑥}{\relax\ifmmode x \else $x$\fi}  % U+1D465
\newunicodechar{𝑦}{\relax\ifmmode y \else $y$\fi}  % U+1D466
\newunicodechar{𝑧}{\relax\ifmmode z \else $z$\fi}  % U+1D467

%% --- Latin Extended-D U+A7B0–U+A7BF (Pagella lacks; extfont keeps Unicode) ---
\newunicodechar{Ʞ}{\mdpiextchar{Ʞ}}  % U+A7B0
\newunicodechar{Ʇ}{\mdpiextchar{Ʇ}}  % U+A7B1
\newunicodechar{Ʝ}{\mdpiextchar{Ʝ}}  % U+A7B2
\newunicodechar{Ꭓ}{\mdpiextchar{Ꭓ}}  % U+A7B3
\newunicodechar{Ꞵ}{\mdpiextchar{Ꞵ}}  % U+A7B4
\newunicodechar{ꞵ}{\mdpiextchar{ꞵ}}  % U+A7B5
\newunicodechar{Ꞷ}{\mdpiextchar{Ꞷ}}  % U+A7B6
\newunicodechar{ꞷ}{\mdpiextchar{ꞷ}}  % U+A7B7
\newunicodechar{Ꞹ}{\mdpiextchar{Ꞹ}}  % U+A7B8
\newunicodechar{ꞹ}{\mdpiextchar{ꞹ}}  % U+A7B9
\newunicodechar{Ꞻ}{\mdpiextchar{Ꞻ}}  % U+A7BA
\newunicodechar{ꞻ}{\mdpiextchar{ꞻ}}  % U+A7BB
\newunicodechar{Ꞽ}{\mdpiextchar{Ꞽ}}  % U+A7BC
\newunicodechar{ꞽ}{\mdpiextchar{ꞽ}}  % U+A7BD
\newunicodechar{Ꞿ}{\mdpiextchar{Ꞿ}}  % U+A7BE
\newunicodechar{ꞿ}{\mdpiextchar{ꞿ}}  % U+A7BF

%% --- Latin extended / phonetic (Pagella lacks; extfont keeps Unicode) ---
%% Pagella-missing Latin / IPA / phonetic (texgyrepagella cmap scan).
%% \mdpiextchar keeps the Unicode code point in tagged PDF.
%% Latin-Ext-A (4)
\newunicodechar{ĸ}{\mdpiextchar{ĸ}}  % U+0138
\newunicodechar{ŉ}{\mdpiextchar{ŉ}}  % U+0149
\newunicodechar{Ŧ}{\mdpiextchar{Ŧ}}  % U+0166
\newunicodechar{ŧ}{\mdpiextchar{ŧ}}  % U+0167
%% Latin-Ext-B (156)
\newunicodechar{ƀ}{\mdpiextchar{ƀ}}  % U+0180
\newunicodechar{Ɓ}{\mdpiextchar{Ɓ}}  % U+0181
\newunicodechar{Ƃ}{\mdpiextchar{Ƃ}}  % U+0182
\newunicodechar{ƃ}{\mdpiextchar{ƃ}}  % U+0183
\newunicodechar{Ƅ}{\mdpiextchar{Ƅ}}  % U+0184
\newunicodechar{ƅ}{\mdpiextchar{ƅ}}  % U+0185
\newunicodechar{Ɔ}{\mdpiextchar{Ɔ}}  % U+0186
\newunicodechar{Ƈ}{\mdpiextchar{Ƈ}}  % U+0187
\newunicodechar{ƈ}{\mdpiextchar{ƈ}}  % U+0188
\newunicodechar{Ɖ}{\mdpiextchar{Ɖ}}  % U+0189
\newunicodechar{Ɗ}{\mdpiextchar{Ɗ}}  % U+018A
\newunicodechar{Ƌ}{\mdpiextchar{Ƌ}}  % U+018B
\newunicodechar{ƌ}{\mdpiextchar{ƌ}}  % U+018C
\newunicodechar{ƍ}{\mdpiextchar{ƍ}}  % U+018D
\newunicodechar{Ə}{\mdpiextchar{Ə}}  % U+018F
\newunicodechar{Ɛ}{\mdpiextchar{Ɛ}}  % U+0190
\newunicodechar{Ƒ}{\mdpiextchar{Ƒ}}  % U+0191
\newunicodechar{Ɠ}{\mdpiextchar{Ɠ}}  % U+0193
\newunicodechar{Ɣ}{\mdpiextchar{Ɣ}}  % U+0194
\newunicodechar{ƕ}{\mdpiextchar{ƕ}}  % U+0195
\newunicodechar{Ɩ}{\mdpiextchar{Ɩ}}  % U+0196
\newunicodechar{Ɨ}{\mdpiextchar{Ɨ}}  % U+0197
\newunicodechar{Ƙ}{\mdpiextchar{Ƙ}}  % U+0198
\newunicodechar{ƙ}{\mdpiextchar{ƙ}}  % U+0199
\newunicodechar{ƚ}{\mdpiextchar{ƚ}}  % U+019A
\newunicodechar{ƛ}{\mdpiextchar{ƛ}}  % U+019B
\newunicodechar{Ɯ}{\mdpiextchar{Ɯ}}  % U+019C
\newunicodechar{Ɲ}{\mdpiextchar{Ɲ}}  % U+019D
\newunicodechar{ƞ}{\mdpiextchar{ƞ}}  % U+019E
\newunicodechar{Ɵ}{\mdpiextchar{Ɵ}}  % U+019F
\newunicodechar{Ƣ}{\mdpiextchar{Ƣ}}  % U+01A2
\newunicodechar{ƣ}{\mdpiextchar{ƣ}}  % U+01A3
\newunicodechar{Ƥ}{\mdpiextchar{Ƥ}}  % U+01A4
\newunicodechar{ƥ}{\mdpiextchar{ƥ}}  % U+01A5
\newunicodechar{Ʀ}{\mdpiextchar{Ʀ}}  % U+01A6
\newunicodechar{Ƨ}{\mdpiextchar{Ƨ}}  % U+01A7
\newunicodechar{ƨ}{\mdpiextchar{ƨ}}  % U+01A8
\newunicodechar{Ʃ}{\mdpiextchar{Ʃ}}  % U+01A9
\newunicodechar{ƪ}{\mdpiextchar{ƪ}}  % U+01AA
\newunicodechar{ƫ}{\mdpiextchar{ƫ}}  % U+01AB
\newunicodechar{Ƭ}{\mdpiextchar{Ƭ}}  % U+01AC
\newunicodechar{ƭ}{\mdpiextchar{ƭ}}  % U+01AD
\newunicodechar{Ʈ}{\mdpiextchar{Ʈ}}  % U+01AE
\newunicodechar{Ʊ}{\mdpiextchar{Ʊ}}  % U+01B1
\newunicodechar{Ʋ}{\mdpiextchar{Ʋ}}  % U+01B2
\newunicodechar{Ƴ}{\mdpiextchar{Ƴ}}  % U+01B3
\newunicodechar{ƴ}{\mdpiextchar{ƴ}}  % U+01B4
\newunicodechar{Ƶ}{\mdpiextchar{Ƶ}}  % U+01B5
\newunicodechar{ƶ}{\mdpiextchar{ƶ}}  % U+01B6
\newunicodechar{Ʒ}{\mdpiextchar{Ʒ}}  % U+01B7
\newunicodechar{Ƹ}{\mdpiextchar{Ƹ}}  % U+01B8
\newunicodechar{ƹ}{\mdpiextchar{ƹ}}  % U+01B9
\newunicodechar{ƺ}{\mdpiextchar{ƺ}}  % U+01BA
\newunicodechar{ƻ}{\mdpiextchar{ƻ}}  % U+01BB
\newunicodechar{Ƽ}{\mdpiextchar{Ƽ}}  % U+01BC
\newunicodechar{ƽ}{\mdpiextchar{ƽ}}  % U+01BD
\newunicodechar{ƾ}{\mdpiextchar{ƾ}}  % U+01BE
\newunicodechar{ƿ}{\mdpiextchar{ƿ}}  % U+01BF
%\newunicodechar{ǀ}{\mdpiextchar{ǀ}}  % U+01C0
\newunicodechar{ǀ}{|}  % U+01C0
%\newunicodechar{ǁ}{\mdpiextchar{ǁ}}  % U+01C1
\newunicodechar{ǁ}{\|}  % U+01C1
%\newunicodechar{ǂ}{\mdpiextchar{ǂ}}  % U+01C2
\newunicodechar{ǂ}{\neq}  % U+01C2
\newunicodechar{ǃ}{!}  % U+01C3
\newunicodechar{Ǆ}{D\v{Z}}  % U+01C4
\newunicodechar{ǅ}{D\v{z}}  % U+01C5
\newunicodechar{ǆ}{d\v{z}}  % U+01C6
%\newunicodechar{Ǉ}{\mdpiextchar{Ǉ}}  % U+01C7
\newunicodechar{Ǉ}{LJ}  % U+01C7
%\newunicodechar{ǈ}{\mdpiextchar{ǈ}}  % U+01C8
\newunicodechar{ǈ}{Lj}  % U+01C8
%\newunicodechar{ǉ}{\mdpiextchar{ǉ}}  % U+01C9
\newunicodechar{ǉ}{lj}  % U+01C9
%\newunicodechar{Ǌ}{\mdpiextchar{Ǌ}}  % U+01CA
\newunicodechar{Ǌ}{NJ}  % U+01CA
%\newunicodechar{ǋ}{\mdpiextchar{ǋ}}  % U+01CB
\newunicodechar{ǋ}{Nj}  % U+01CB
%\newunicodechar{ǌ}{\mdpiextchar{ǌ}}  % U+01CC
\newunicodechar{ǌ}{nj}  % U+01CC
\newunicodechar{Ǖ}{\mdpiextchar{Ǖ}}  % U+01D5
\newunicodechar{ǖ}{\mdpiextchar{ǖ}}  % U+01D6
\newunicodechar{Ǟ}{\mdpiextchar{Ǟ}}  % U+01DE
\newunicodechar{ǟ}{\mdpiextchar{ǟ}}  % U+01DF
\newunicodechar{Ǡ}{\mdpiextchar{Ǡ}}  % U+01E0
\newunicodechar{ǡ}{\mdpiextchar{ǡ}}  % U+01E1
\newunicodechar{Ǣ}{\mdpiextchar{Ǣ}}  % U+01E2
\newunicodechar{ǣ}{\mdpiextchar{ǣ}}  % U+01E3
\newunicodechar{Ǥ}{\mdpiextchar{Ǥ}}  % U+01E4
\newunicodechar{ǥ}{\mdpiextchar{ǥ}}  % U+01E5
\newunicodechar{Ǩ}{\mdpiextchar{Ǩ}}  % U+01E8
\newunicodechar{ǩ}{\mdpiextchar{ǩ}}  % U+01E9
\newunicodechar{Ǭ}{\mdpiextchar{Ǭ}}  % U+01EC
\newunicodechar{ǭ}{\mdpiextchar{ǭ}}  % U+01ED
\newunicodechar{Ǯ}{\mdpiextchar{Ǯ}}  % U+01EE
\newunicodechar{ǯ}{\mdpiextchar{ǯ}}  % U+01EF
\newunicodechar{Ǳ}{DZ}  % U+01F1
\newunicodechar{ǲ}{Dz}  % U+01F2
\newunicodechar{ǳ}{dz}  % U+01F3
\newunicodechar{Ƕ}{\mdpiextchar{Ƕ}}  % U+01F6
\newunicodechar{Ƿ}{\mdpiextchar{Ƿ}}  % U+01F7
\newunicodechar{Ǹ}{\mdpiextchar{Ǹ}}  % U+01F8
\newunicodechar{ǹ}{\mdpiextchar{ǹ}}  % U+01F9
\newunicodechar{Ȃ}{\mdpiextchar{Ȃ}}  % U+0202
\newunicodechar{ȃ}{\mdpiextchar{ȃ}}  % U+0203
\newunicodechar{Ȇ}{\mdpiextchar{Ȇ}}  % U+0206
\newunicodechar{ȇ}{\mdpiextchar{ȇ}}  % U+0207
\newunicodechar{Ȋ}{\mdpiextchar{Ȋ}}  % U+020A
\newunicodechar{ȋ}{\mdpiextchar{ȋ}}  % U+020B
\newunicodechar{Ȏ}{\mdpiextchar{Ȏ}}  % U+020E
\newunicodechar{ȏ}{\mdpiextchar{ȏ}}  % U+020F
\newunicodechar{Ȓ}{\mdpiextchar{Ȓ}}  % U+0212
\newunicodechar{ȓ}{\mdpiextchar{ȓ}}  % U+0213
\newunicodechar{Ȗ}{\mdpiextchar{Ȗ}}  % U+0216
\newunicodechar{ȗ}{\mdpiextchar{ȗ}}  % U+0217
\newunicodechar{Ȝ}{\mdpiextchar{Ȝ}}  % U+021C
\newunicodechar{ȝ}{\mdpiextchar{ȝ}}  % U+021D
\newunicodechar{Ȟ}{\mdpiextchar{Ȟ}}  % U+021E
\newunicodechar{ȟ}{\mdpiextchar{ȟ}}  % U+021F
\newunicodechar{Ƞ}{\mdpiextchar{Ƞ}}  % U+0220
\newunicodechar{ȡ}{\mdpiextchar{ȡ}}  % U+0221
\newunicodechar{Ȣ}{\mdpiextchar{Ȣ}}  % U+0222
\newunicodechar{ȣ}{\mdpiextchar{ȣ}}  % U+0223
\newunicodechar{Ȥ}{\mdpiextchar{Ȥ}}  % U+0224
\newunicodechar{ȥ}{\mdpiextchar{ȥ}}  % U+0225
%\newunicodechar{Ȧ}{\mdpiextchar{Ȧ}}  % U+0226
\newunicodechar{Ȧ}{\.{A}}  % U+0226
%\newunicodechar{ȧ}{\mdpiextchar{ȧ}}  % U+0227
\newunicodechar{ȧ}{\.{a}}  % U+0227
\newunicodechar{Ȩ}{\mdpiextchar{Ȩ}}  % U+0228
\newunicodechar{Ȫ}{\mdpiextchar{Ȫ}}  % U+022A
\newunicodechar{ȫ}{\mdpiextchar{ȫ}}  % U+022B
\newunicodechar{Ȭ}{\mdpiextchar{Ȭ}}  % U+022C
\newunicodechar{ȭ}{\mdpiextchar{ȭ}}  % U+022D
%\newunicodechar{Ȯ}{\mdpiextchar{Ȯ}}  % U+022E
\newunicodechar{Ȯ}{\.{O}}  % U+022E
%\newunicodechar{ȯ}{\mdpiextchar{ȯ}}  % U+022F
\newunicodechar{ȯ}{\.{o}}  % U+022F
\newunicodechar{Ȱ}{\mdpiextchar{Ȱ}}  % U+0230
\newunicodechar{ȱ}{\mdpiextchar{ȱ}}  % U+0231
%\newunicodechar{Ȳ}{\mdpiextchar{Ȳ}}  % U+0232
\newunicodechar{Ȳ}{\={Y}}  % U+0232
%\newunicodechar{ȳ}{\mdpiextchar{ȳ}}  % U+0233
\newunicodechar{ȳ}{\={y}}  % U+0233
\newunicodechar{ȴ}{\mdpiextchar{ȴ}}  % U+0234
\newunicodechar{ȵ}{\mdpiextchar{ȵ}}  % U+0235
\newunicodechar{ȶ}{\mdpiextchar{ȶ}}  % U+0236
\newunicodechar{ȸ}{\mdpiextchar{ȸ}}  % U+0238
\newunicodechar{ȹ}{\mdpiextchar{ȹ}}  % U+0239
\newunicodechar{Ⱥ}{\mdpiextchar{Ⱥ}}  % U+023A
\newunicodechar{Ȼ}{\mdpiextchar{Ȼ}}  % U+023B
\newunicodechar{ȼ}{\mdpiextchar{ȼ}}  % U+023C
\newunicodechar{Ƚ}{\mdpiextchar{Ƚ}}  % U+023D
\newunicodechar{Ⱦ}{\mdpiextchar{Ⱦ}}  % U+023E
\newunicodechar{ȿ}{\mdpiextchar{ȿ}}  % U+023F
\newunicodechar{ɀ}{\mdpiextchar{ɀ}}  % U+0240
\newunicodechar{Ɂ}{\mdpiextchar{Ɂ}}  % U+0241
\newunicodechar{ɂ}{\mdpiextchar{ɂ}}  % U+0242
\newunicodechar{Ƀ}{\mdpiextchar{Ƀ}}  % U+0243
\newunicodechar{Ʉ}{\mdpiextchar{Ʉ}}  % U+0244
\newunicodechar{Ʌ}{\mdpiextchar{Ʌ}}  % U+0245
\newunicodechar{Ɇ}{\mdpiextchar{Ɇ}}  % U+0246
\newunicodechar{ɇ}{\mdpiextchar{ɇ}}  % U+0247
\newunicodechar{Ɉ}{\mdpiextchar{Ɉ}}  % U+0248
\newunicodechar{ɉ}{\mdpiextchar{ɉ}}  % U+0249
\newunicodechar{Ɋ}{\mdpiextchar{Ɋ}}  % U+024A
\newunicodechar{ɋ}{\mdpiextchar{ɋ}}  % U+024B
\newunicodechar{Ɍ}{\mdpiextchar{Ɍ}}  % U+024C
\newunicodechar{ɍ}{\mdpiextchar{ɍ}}  % U+024D
\newunicodechar{Ɏ}{\mdpiextchar{Ɏ}}  % U+024E
\newunicodechar{ɏ}{\mdpiextchar{ɏ}}  % U+024F
%% IPA-Extensions (94)
\newunicodechar{ɐ}{\mdpiextchar{ɐ}}  % U+0250
\newunicodechar{ɑ}{\mdpiextchar{ɑ}}  % U+0251
\newunicodechar{ɒ}{\mdpiextchar{ɒ}}  % U+0252
\newunicodechar{ɓ}{\mdpiextchar{ɓ}}  % U+0253
\newunicodechar{ɔ}{\mdpiextchar{ɔ}}  % U+0254
\newunicodechar{ɕ}{\mdpiextchar{ɕ}}  % U+0255
\newunicodechar{ɖ}{\mdpiextchar{ɖ}}  % U+0256
\newunicodechar{ɗ}{\mdpiextchar{ɗ}}  % U+0257
\newunicodechar{ɚ}{\mdpiextchar{ɚ}}  % U+025A
\newunicodechar{ɛ}{\mdpiextchar{ɛ}}  % U+025B
\newunicodechar{ɜ}{\mdpiextchar{ɜ}}  % U+025C
\newunicodechar{ɝ}{\mdpiextchar{ɝ}}  % U+025D
\newunicodechar{ɞ}{\mdpiextchar{ɞ}}  % U+025E
\newunicodechar{ɟ}{\mdpiextchar{ɟ}}  % U+025F
\newunicodechar{ɠ}{\mdpiextchar{ɠ}}  % U+0260
\newunicodechar{ɡ}{\mdpiextchar{ɡ}}  % U+0261
\newunicodechar{ɢ}{\mdpiextchar{ɢ}}  % U+0262
\newunicodechar{ɣ}{\mdpiextchar{ɣ}}  % U+0263
\newunicodechar{ɤ}{\mdpiextchar{ɤ}}  % U+0264
\newunicodechar{ɥ}{\mdpiextchar{ɥ}}  % U+0265
\newunicodechar{ɦ}{\mdpiextchar{ɦ}}  % U+0266
\newunicodechar{ɧ}{\mdpiextchar{ɧ}}  % U+0267
\newunicodechar{ɨ}{\mdpiextchar{ɨ}}  % U+0268
\newunicodechar{ɩ}{\mdpiextchar{ɩ}}  % U+0269
\newunicodechar{ɪ}{\mdpiextchar{ɪ}}  % U+026A
\newunicodechar{ɫ}{\mdpiextchar{ɫ}}  % U+026B
\newunicodechar{ɬ}{\mdpiextchar{ɬ}}  % U+026C
\newunicodechar{ɭ}{\mdpiextchar{ɭ}}  % U+026D
\newunicodechar{ɮ}{\mdpiextchar{ɮ}}  % U+026E
\newunicodechar{ɯ}{\mdpiextchar{ɯ}}  % U+026F
\newunicodechar{ɰ}{\mdpiextchar{ɰ}}  % U+0270
\newunicodechar{ɱ}{\mdpiextchar{ɱ}}  % U+0271
\newunicodechar{ɲ}{\mdpiextchar{ɲ}}  % U+0272
\newunicodechar{ɳ}{\mdpiextchar{ɳ}}  % U+0273
\newunicodechar{ɴ}{\mdpiextchar{ɴ}}  % U+0274
\newunicodechar{ɵ}{\mdpiextchar{ɵ}}  % U+0275
\newunicodechar{ɶ}{\mdpiextchar{ɶ}}  % U+0276
\newunicodechar{ɷ}{\mdpiextchar{ɷ}}  % U+0277
\newunicodechar{ɸ}{\mdpiextchar{ɸ}}  % U+0278
\newunicodechar{ɹ}{\mdpiextchar{ɹ}}  % U+0279
\newunicodechar{ɺ}{\mdpiextchar{ɺ}}  % U+027A
\newunicodechar{ɻ}{\mdpiextchar{ɻ}}  % U+027B
\newunicodechar{ɼ}{\mdpiextchar{ɼ}}  % U+027C
\newunicodechar{ɽ}{\mdpiextchar{ɽ}}  % U+027D
\newunicodechar{ɾ}{\mdpiextchar{ɾ}}  % U+027E
\newunicodechar{ɿ}{\mdpiextchar{ɿ}}  % U+027F
\newunicodechar{ʀ}{\mdpiextchar{ʀ}}  % U+0280
\newunicodechar{ʁ}{\mdpiextchar{ʁ}}  % U+0281
\newunicodechar{ʂ}{\mdpiextchar{ʂ}}  % U+0282
\newunicodechar{ʃ}{\mdpiextchar{ʃ}}  % U+0283
\newunicodechar{ʄ}{\mdpiextchar{ʄ}}  % U+0284
\newunicodechar{ʅ}{\mdpiextchar{ʅ}}  % U+0285
\newunicodechar{ʆ}{\mdpiextchar{ʆ}}  % U+0286
\newunicodechar{ʇ}{\mdpiextchar{ʇ}}  % U+0287
\newunicodechar{ʈ}{\mdpiextchar{ʈ}}  % U+0288
\newunicodechar{ʉ}{\mdpiextchar{ʉ}}  % U+0289
\newunicodechar{ʊ}{\mdpiextchar{ʊ}}  % U+028A
\newunicodechar{ʋ}{\mdpiextchar{ʋ}}  % U+028B
\newunicodechar{ʌ}{\mdpiextchar{ʌ}}  % U+028C
\newunicodechar{ʍ}{\mdpiextchar{ʍ}}  % U+028D
\newunicodechar{ʎ}{\mdpiextchar{ʎ}}  % U+028E
\newunicodechar{ʏ}{\mdpiextchar{ʏ}}  % U+028F
\newunicodechar{ʐ}{\mdpiextchar{ʐ}}  % U+0290
\newunicodechar{ʑ}{\mdpiextchar{ʑ}}  % U+0291
\newunicodechar{ʒ}{\mdpiextchar{ʒ}}  % U+0292
\newunicodechar{ʓ}{\mdpiextchar{ʓ}}  % U+0293
\newunicodechar{ʔ}{\mdpiextchar{ʔ}}  % U+0294
\newunicodechar{ʕ}{\mdpiextchar{ʕ}}  % U+0295
\newunicodechar{ʖ}{\mdpiextchar{ʖ}}  % U+0296
\newunicodechar{ʗ}{\mdpiextchar{ʗ}}  % U+0297
\newunicodechar{ʘ}{\mdpiextchar{ʘ}}  % U+0298
\newunicodechar{ʙ}{\mdpiextchar{ʙ}}  % U+0299
\newunicodechar{ʚ}{\mdpiextchar{ʚ}}  % U+029A
\newunicodechar{ʛ}{\mdpiextchar{ʛ}}  % U+029B
\newunicodechar{ʜ}{\mdpiextchar{ʜ}}  % U+029C
\newunicodechar{ʝ}{\mdpiextchar{ʝ}}  % U+029D
\newunicodechar{ʞ}{\mdpiextchar{ʞ}}  % U+029E
\newunicodechar{ʟ}{\mdpiextchar{ʟ}}  % U+029F
\newunicodechar{ʠ}{\mdpiextchar{ʠ}}  % U+02A0
\newunicodechar{ʡ}{\mdpiextchar{ʡ}}  % U+02A1
\newunicodechar{ʢ}{\mdpiextchar{ʢ}}  % U+02A2
\newunicodechar{ʣ}{\mdpiextchar{ʣ}}  % U+02A3
\newunicodechar{ʤ}{\mdpiextchar{ʤ}}  % U+02A4
\newunicodechar{ʥ}{\mdpiextchar{ʥ}}  % U+02A5
\newunicodechar{ʦ}{\mdpiextchar{ʦ}}  % U+02A6
\newunicodechar{ʧ}{\mdpiextchar{ʧ}}  % U+02A7
\newunicodechar{ʨ}{\mdpiextchar{ʨ}}  % U+02A8
\newunicodechar{ʩ}{\mdpiextchar{ʩ}}  % U+02A9
\newunicodechar{ʪ}{\mdpiextchar{ʪ}}  % U+02AA
\newunicodechar{ʫ}{\mdpiextchar{ʫ}}  % U+02AB
\newunicodechar{ʬ}{\mdpiextchar{ʬ}}  % U+02AC
\newunicodechar{ʭ}{\mdpiextchar{ʭ}}  % U+02AD
\newunicodechar{ʮ}{\mdpiextchar{ʮ}}  % U+02AE
\newunicodechar{ʯ}{\mdpiextchar{ʯ}}  % U+02AF
%%% Spacing-Modifier-Letters (69)
%\newunicodechar{ʰ}{\mdpiextchar{ʰ}}  % U+02B0
%\newunicodechar{ʱ}{\mdpiextchar{ʱ}}  % U+02B1
%\newunicodechar{ʲ}{\mdpiextchar{ʲ}}  % U+02B2
%\newunicodechar{ʳ}{\mdpiextchar{ʳ}}  % U+02B3
%\newunicodechar{ʴ}{\mdpiextchar{ʴ}}  % U+02B4
%\newunicodechar{ʵ}{\mdpiextchar{ʵ}}  % U+02B5
%\newunicodechar{ʶ}{\mdpiextchar{ʶ}}  % U+02B6
%\newunicodechar{ʷ}{\mdpiextchar{ʷ}}  % U+02B7
%\newunicodechar{ʸ}{\mdpiextchar{ʸ}}  % U+02B8
\newunicodechar{ʹ}{'}  % U+02B9
\newunicodechar{ʺ}{"}  % U+02BA
\newunicodechar{ʻ}{\mdpiextchar{ʻ}}  % U+02BB
\newunicodechar{ʼ}{\mdpiextchar{ʼ}}  % U+02BC
\newunicodechar{ʽ}{\mdpiextchar{ʽ}}  % U+02BD
\newunicodechar{ˀ}{\mdpiextchar{ˀ}}  % U+02C0
\newunicodechar{ˁ}{\mdpiextchar{ˁ}}  % U+02C1
\newunicodechar{˃}{>}  % U+02C3
\newunicodechar{˄}{\mdpiextchar{˄}}  % U+02C4
\newunicodechar{˅}{\mdpiextchar{˅}}  % U+02C5
%\newunicodechar{ˈ}{\mdpiextchar{ˈ}}  % U+02C8
%\newunicodechar{ˉ}{\mdpiextchar{ˉ}}  % U+02C9
%\newunicodechar{ˊ}{\mdpiextchar{ˊ}}  % U+02CA
%\newunicodechar{ˋ}{\mdpiextchar{ˋ}}  % U+02CB
%\newunicodechar{ˌ}{\mdpiextchar{ˌ}}  % U+02CC
%\newunicodechar{ˍ}{\mdpiextchar{ˍ}}  % U+02CD
%\newunicodechar{ˎ}{\mdpiextchar{ˎ}}  % U+02CE
%\newunicodechar{ˏ}{\mdpiextchar{ˏ}}  % U+02CF
%\newunicodechar{ː}{\mdpiextchar{ː}}  % U+02D0
%\newunicodechar{ˑ}{\mdpiextchar{ˑ}}  % U+02D1
%\newunicodechar{˒}{\mdpiextchar{˒}}  % U+02D2
%\newunicodechar{˓}{\mdpiextchar{˓}}  % U+02D3
%\newunicodechar{˔}{\mdpiextchar{˔}}  % U+02D4
%\newunicodechar{˕}{\mdpiextchar{˕}}  % U+02D5
%\newunicodechar{˖}{\mdpiextchar{˖}}  % U+02D6
%\newunicodechar{˗}{\mdpiextchar{˗}}  % U+02D7
%\newunicodechar{˞}{\mdpiextchar{˞}}  % U+02DE
%\newunicodechar{˟}{\mdpiextchar{˟}}  % U+02DF
%\newunicodechar{ˠ}{\mdpiextchar{ˠ}}  % U+02E0
%\newunicodechar{ˡ}{\mdpiextchar{ˡ}}  % U+02E1
%\newunicodechar{ˢ}{\mdpiextchar{ˢ}}  % U+02E2
%\newunicodechar{ˣ}{\mdpiextchar{ˣ}}  % U+02E3
%\newunicodechar{ˤ}{\mdpiextchar{ˤ}}  % U+02E4
%\newunicodechar{˥}{\mdpiextchar{˥}}  % U+02E5
%\newunicodechar{˦}{\mdpiextchar{˦}}  % U+02E6
%\newunicodechar{˧}{\mdpiextchar{˧}}  % U+02E7
%\newunicodechar{˨}{\mdpiextchar{˨}}  % U+02E8
%\newunicodechar{˩}{\mdpiextchar{˩}}  % U+02E9
%\newunicodechar{˪}{\mdpiextchar{˪}}  % U+02EA
%\newunicodechar{˫}{\mdpiextchar{˫}}  % U+02EB
%\newunicodechar{ˬ}{\mdpiextchar{ˬ}}  % U+02EC
%\newunicodechar{˭}{\mdpiextchar{˭}}  % U+02ED
%\newunicodechar{ˮ}{\mdpiextchar{ˮ}}  % U+02EE
%\newunicodechar{˯}{\mdpiextchar{˯}}  % U+02EF
%\newunicodechar{˰}{\mdpiextchar{˰}}  % U+02F0
%\newunicodechar{˱}{\mdpiextchar{˱}}  % U+02F1
%\newunicodechar{˲}{\mdpiextchar{˲}}  % U+02F2
%\newunicodechar{˳}{\mdpiextchar{˳}}  % U+02F3
%\newunicodechar{˴}{\mdpiextchar{˴}}  % U+02F4
%\newunicodechar{˵}{\mdpiextchar{˵}}  % U+02F5
%\newunicodechar{˶}{\mdpiextchar{˶}}  % U+02F6
%\newunicodechar{˷}{\mdpiextchar{˷}}  % U+02F7
%\newunicodechar{˸}{\mdpiextchar{˸}}  % U+02F8
%\newunicodechar{˹}{\mdpiextchar{˹}}  % U+02F9
%\newunicodechar{˺}{\mdpiextchar{˺}}  % U+02FA
%\newunicodechar{˻}{\mdpiextchar{˻}}  % U+02FB
%\newunicodechar{˼}{\mdpiextchar{˼}}  % U+02FC
%\newunicodechar{˽}{\mdpiextchar{˽}}  % U+02FD
%\newunicodechar{˾}{\mdpiextchar{˾}}  % U+02FE
%\newunicodechar{˿}{\mdpiextchar{˿}}  % U+02FF
%% Latin-Ext-C (32)
\newunicodechar{Ⱡ}{\mdpiextchar{Ⱡ}}  % U+2C60
\newunicodechar{ⱡ}{\mdpiextchar{ⱡ}}  % U+2C61
%\newunicodechar{Ɫ}{\mdpiextchar{Ɫ}}  % U+2C62
%\newunicodechar{Ᵽ}{\mdpiextchar{Ᵽ}}  % U+2C63
%\newunicodechar{Ɽ}{\mdpiextchar{Ɽ}}  % U+2C64
%\newunicodechar{ⱥ}{\mdpiextchar{ⱥ}}  % U+2C65
%\newunicodechar{ⱦ}{\mdpiextchar{ⱦ}}  % U+2C66
\newunicodechar{Ⱨ}{\mdpiextchar{Ⱨ}}  % U+2C67
\newunicodechar{ⱨ}{\mdpiextchar{ⱨ}}  % U+2C68
\newunicodechar{Ⱪ}{\mdpiextchar{Ⱪ}}  % U+2C69
\newunicodechar{ⱪ}{\mdpiextchar{ⱪ}}  % U+2C6A
\newunicodechar{Ⱬ}{\mdpiextchar{Ⱬ}}  % U+2C6B
\newunicodechar{ⱬ}{\mdpiextchar{ⱬ}}  % U+2C6C
\newunicodechar{Ɑ}{\mdpiextchar{Ɑ}}  % U+2C6D
\newunicodechar{Ɱ}{\mdpiextchar{Ɱ}}  % U+2C6E
\newunicodechar{Ɐ}{\mdpiextchar{Ɐ}}  % U+2C6F
\newunicodechar{Ɒ}{\mdpiextchar{Ɒ}}  % U+2C70
\newunicodechar{ⱱ}{\mdpiextchar{ⱱ}}  % U+2C71
\newunicodechar{Ⱳ}{\mdpiextchar{Ⱳ}}  % U+2C72
\newunicodechar{ⱳ}{\mdpiextchar{ⱳ}}  % U+2C73
\newunicodechar{ⱴ}{\mdpiextchar{ⱴ}}  % U+2C74
\newunicodechar{Ⱶ}{\mdpiextchar{Ⱶ}}  % U+2C75
\newunicodechar{ⱶ}{\mdpiextchar{ⱶ}}  % U+2C76
\newunicodechar{ⱷ}{\mdpiextchar{ⱷ}}  % U+2C77
\newunicodechar{ⱸ}{\mdpiextchar{ⱸ}}  % U+2C78
\newunicodechar{ⱹ}{\mdpiextchar{ⱹ}}  % U+2C79
\newunicodechar{ⱺ}{\mdpiextchar{ⱺ}}  % U+2C7A
\newunicodechar{ⱻ}{\mdpiextchar{ⱻ}}  % U+2C7B
\newunicodechar{ⱼ}{\mdpiextchar{ⱼ}}  % U+2C7C
\newunicodechar{ⱽ}{\mdpiextchar{ⱽ}}  % U+2C7D
\newunicodechar{Ȿ}{\mdpiextchar{Ȿ}}  % U+2C7E
\newunicodechar{Ɀ}{\mdpiextchar{Ɀ}}  % U+2C7F
%%% Phonetic-Extensions (124)
%\newunicodechar{ᴀ}{\mdpiextchar{ᴀ}}  % U+1D00
%\newunicodechar{ᴁ}{\mdpiextchar{ᴁ}}  % U+1D01
%\newunicodechar{ᴂ}{\mdpiextchar{ᴂ}}  % U+1D02
%\newunicodechar{ᴃ}{\mdpiextchar{ᴃ}}  % U+1D03
%\newunicodechar{ᴄ}{\mdpiextchar{ᴄ}}  % U+1D04
%\newunicodechar{ᴅ}{\mdpiextchar{ᴅ}}  % U+1D05
%\newunicodechar{ᴆ}{\mdpiextchar{ᴆ}}  % U+1D06
%\newunicodechar{ᴇ}{\mdpiextchar{ᴇ}}  % U+1D07
%\newunicodechar{ᴈ}{\mdpiextchar{ᴈ}}  % U+1D08
%\newunicodechar{ᴉ}{\mdpiextchar{ᴉ}}  % U+1D09
%\newunicodechar{ᴊ}{\mdpiextchar{ᴊ}}  % U+1D0A
%\newunicodechar{ᴋ}{\mdpiextchar{ᴋ}}  % U+1D0B
%\newunicodechar{ᴌ}{\mdpiextchar{ᴌ}}  % U+1D0C
%\newunicodechar{ᴍ}{\mdpiextchar{ᴍ}}  % U+1D0D
%\newunicodechar{ᴎ}{\mdpiextchar{ᴎ}}  % U+1D0E
%\newunicodechar{ᴏ}{\mdpiextchar{ᴏ}}  % U+1D0F
%\newunicodechar{ᴐ}{\mdpiextchar{ᴐ}}  % U+1D10
%\newunicodechar{ᴑ}{\mdpiextchar{ᴑ}}  % U+1D11
%\newunicodechar{ᴒ}{\mdpiextchar{ᴒ}}  % U+1D12
%\newunicodechar{ᴓ}{\mdpiextchar{ᴓ}}  % U+1D13
%\newunicodechar{ᴔ}{\mdpiextchar{ᴔ}}  % U+1D14
%\newunicodechar{ᴕ}{\mdpiextchar{ᴕ}}  % U+1D15
%\newunicodechar{ᴖ}{\mdpiextchar{ᴖ}}  % U+1D16
%\newunicodechar{ᴗ}{\mdpiextchar{ᴗ}}  % U+1D17
%\newunicodechar{ᴘ}{\mdpiextchar{ᴘ}}  % U+1D18
%\newunicodechar{ᴙ}{\mdpiextchar{ᴙ}}  % U+1D19
%\newunicodechar{ᴚ}{\mdpiextchar{ᴚ}}  % U+1D1A
%\newunicodechar{ᴛ}{\mdpiextchar{ᴛ}}  % U+1D1B
%\newunicodechar{ᴜ}{\mdpiextchar{ᴜ}}  % U+1D1C
%\newunicodechar{ᴝ}{\mdpiextchar{ᴝ}}  % U+1D1D
%\newunicodechar{ᴞ}{\mdpiextchar{ᴞ}}  % U+1D1E
%\newunicodechar{ᴟ}{\mdpiextchar{ᴟ}}  % U+1D1F
%\newunicodechar{ᴠ}{\mdpiextchar{ᴠ}}  % U+1D20
%\newunicodechar{ᴡ}{\mdpiextchar{ᴡ}}  % U+1D21
%\newunicodechar{ᴢ}{\mdpiextchar{ᴢ}}  % U+1D22
%\newunicodechar{ᴣ}{\mdpiextchar{ᴣ}}  % U+1D23
%\newunicodechar{ᴤ}{\mdpiextchar{ᴤ}}  % U+1D24
%\newunicodechar{ᴥ}{\mdpiextchar{ᴥ}}  % U+1D25
%\newunicodechar{ᴦ}{\mdpiextchar{ᴦ}}  % U+1D26
%\newunicodechar{ᴧ}{\mdpiextchar{ᴧ}}  % U+1D27
%\newunicodechar{ᴨ}{\mdpiextchar{ᴨ}}  % U+1D28
%\newunicodechar{ᴩ}{\mdpiextchar{ᴩ}}  % U+1D29
%\newunicodechar{ᴪ}{\mdpiextchar{ᴪ}}  % U+1D2A
%\newunicodechar{ᴫ}{\mdpiextchar{ᴫ}}  % U+1D2B
%\newunicodechar{ᴬ}{\mdpiextchar{ᴬ}}  % U+1D2C
%\newunicodechar{ᴭ}{\mdpiextchar{ᴭ}}  % U+1D2D
%\newunicodechar{ᴮ}{\mdpiextchar{ᴮ}}  % U+1D2E
%\newunicodechar{ᴯ}{\mdpiextchar{ᴯ}}  % U+1D2F
%\newunicodechar{ᴰ}{\mdpiextchar{ᴰ}}  % U+1D30
%\newunicodechar{ᴱ}{\mdpiextchar{ᴱ}}  % U+1D31
%\newunicodechar{ᴲ}{\mdpiextchar{ᴲ}}  % U+1D32
%\newunicodechar{ᴳ}{\mdpiextchar{ᴳ}}  % U+1D33
%\newunicodechar{ᴴ}{\mdpiextchar{ᴴ}}  % U+1D34
%\newunicodechar{ᴵ}{\mdpiextchar{ᴵ}}  % U+1D35
%\newunicodechar{ᴶ}{\mdpiextchar{ᴶ}}  % U+1D36
%\newunicodechar{ᴷ}{\mdpiextchar{ᴷ}}  % U+1D37
%\newunicodechar{ᴸ}{\mdpiextchar{ᴸ}}  % U+1D38
%\newunicodechar{ᴹ}{\mdpiextchar{ᴹ}}  % U+1D39
%\newunicodechar{ᴺ}{\mdpiextchar{ᴺ}}  % U+1D3A
%\newunicodechar{ᴻ}{\mdpiextchar{ᴻ}}  % U+1D3B
%\newunicodechar{ᴼ}{\mdpiextchar{ᴼ}}  % U+1D3C
%\newunicodechar{ᴽ}{\mdpiextchar{ᴽ}}  % U+1D3D
%\newunicodechar{ᴾ}{\mdpiextchar{ᴾ}}  % U+1D3E
%\newunicodechar{ᴿ}{\mdpiextchar{ᴿ}}  % U+1D3F
%\newunicodechar{ᵀ}{\mdpiextchar{ᵀ}}  % U+1D40
%\newunicodechar{ᵁ}{\mdpiextchar{ᵁ}}  % U+1D41
%\newunicodechar{ᵂ}{\mdpiextchar{ᵂ}}  % U+1D42
%\newunicodechar{ᵇ}{\mdpiextchar{ᵇ}}  % U+1D47
%\newunicodechar{ᵈ}{\mdpiextchar{ᵈ}}  % U+1D48
%\newunicodechar{ᵉ}{\mdpiextchar{ᵉ}}  % U+1D49
%\newunicodechar{ᵊ}{\mdpiextchar{ᵊ}}  % U+1D4A
%\newunicodechar{ᵋ}{\mdpiextchar{ᵋ}}  % U+1D4B
%\newunicodechar{ᵌ}{\mdpiextchar{ᵌ}}  % U+1D4C
%\newunicodechar{ᵍ}{\mdpiextchar{ᵍ}}  % U+1D4D
%\newunicodechar{ᵎ}{\mdpiextchar{ᵎ}}  % U+1D4E
%\newunicodechar{ᵏ}{\mdpiextchar{ᵏ}}  % U+1D4F
%\newunicodechar{ᵐ}{\mdpiextchar{ᵐ}}  % U+1D50
%\newunicodechar{ᵑ}{\mdpiextchar{ᵑ}}  % U+1D51
%\newunicodechar{ᵒ}{\mdpiextchar{ᵒ}}  % U+1D52
%\newunicodechar{ᵓ}{\mdpiextchar{ᵓ}}  % U+1D53
%\newunicodechar{ᵔ}{\mdpiextchar{ᵔ}}  % U+1D54
%\newunicodechar{ᵕ}{\mdpiextchar{ᵕ}}  % U+1D55
%\newunicodechar{ᵖ}{\mdpiextchar{ᵖ}}  % U+1D56
%\newunicodechar{ᵗ}{\mdpiextchar{ᵗ}}  % U+1D57
%\newunicodechar{ᵘ}{\mdpiextchar{ᵘ}}  % U+1D58
%\newunicodechar{ᵙ}{\mdpiextchar{ᵙ}}  % U+1D59
%\newunicodechar{ᵚ}{\mdpiextchar{ᵚ}}  % U+1D5A
%\newunicodechar{ᵛ}{\mdpiextchar{ᵛ}}  % U+1D5B
%\newunicodechar{ᵜ}{\mdpiextchar{ᵜ}}  % U+1D5C
%\newunicodechar{ᵝ}{\mdpiextchar{ᵝ}}  % U+1D5D
%\newunicodechar{ᵞ}{\mdpiextchar{ᵞ}}  % U+1D5E
%\newunicodechar{ᵟ}{\mdpiextchar{ᵟ}}  % U+1D5F
%\newunicodechar{ᵠ}{\mdpiextchar{ᵠ}}  % U+1D60
%\newunicodechar{ᵡ}{\mdpiextchar{ᵡ}}  % U+1D61
%\newunicodechar{ᵢ}{\mdpiextchar{ᵢ}}  % U+1D62
%\newunicodechar{ᵣ}{\mdpiextchar{ᵣ}}  % U+1D63
%\newunicodechar{ᵤ}{\mdpiextchar{ᵤ}}  % U+1D64
%\newunicodechar{ᵥ}{\mdpiextchar{ᵥ}}  % U+1D65
%\newunicodechar{ᵦ}{\mdpiextchar{ᵦ}}  % U+1D66
%\newunicodechar{ᵧ}{\mdpiextchar{ᵧ}}  % U+1D67
%\newunicodechar{ᵨ}{\mdpiextchar{ᵨ}}  % U+1D68
%\newunicodechar{ᵩ}{\mdpiextchar{ᵩ}}  % U+1D69
%\newunicodechar{ᵪ}{\mdpiextchar{ᵪ}}  % U+1D6A
%\newunicodechar{ᵫ}{\mdpiextchar{ᵫ}}  % U+1D6B
%\newunicodechar{ᵬ}{\mdpiextchar{ᵬ}}  % U+1D6C
%\newunicodechar{ᵭ}{\mdpiextchar{ᵭ}}  % U+1D6D
%\newunicodechar{ᵮ}{\mdpiextchar{ᵮ}}  % U+1D6E
%\newunicodechar{ᵯ}{\mdpiextchar{ᵯ}}  % U+1D6F
%\newunicodechar{ᵰ}{\mdpiextchar{ᵰ}}  % U+1D70
%\newunicodechar{ᵱ}{\mdpiextchar{ᵱ}}  % U+1D71
%\newunicodechar{ᵲ}{\mdpiextchar{ᵲ}}  % U+1D72
%\newunicodechar{ᵳ}{\mdpiextchar{ᵳ}}  % U+1D73
%\newunicodechar{ᵴ}{\mdpiextchar{ᵴ}}  % U+1D74
%\newunicodechar{ᵵ}{\mdpiextchar{ᵵ}}  % U+1D75
%\newunicodechar{ᵶ}{\mdpiextchar{ᵶ}}  % U+1D76
%\newunicodechar{ᵷ}{\mdpiextchar{ᵷ}}  % U+1D77
%\newunicodechar{ᵸ}{\mdpiextchar{ᵸ}}  % U+1D78
%\newunicodechar{ᵹ}{\mdpiextchar{ᵹ}}  % U+1D79
%\newunicodechar{ᵺ}{\mdpiextchar{ᵺ}}  % U+1D7A
%\newunicodechar{ᵻ}{\mdpiextchar{ᵻ}}  % U+1D7B
%\newunicodechar{ᵼ}{\mdpiextchar{ᵼ}}  % U+1D7C
%\newunicodechar{ᵽ}{\mdpiextchar{ᵽ}}  % U+1D7D
%\newunicodechar{ᵾ}{\mdpiextchar{ᵾ}}  % U+1D7E
%\newunicodechar{ᵿ}{\mdpiextchar{ᵿ}}  % U+1D7F
%% Latin-Ext-D (208)
%\newunicodechar{꜠}{\mdpiextchar{꜠}}  % U+A720
%\newunicodechar{꜡}{\mdpiextchar{꜡}}  % U+A721
%\newunicodechar{Ꜣ}{\mdpiextchar{Ꜣ}}  % U+A722
%\newunicodechar{ꜣ}{\mdpiextchar{ꜣ}}  % U+A723
%\newunicodechar{Ꜥ}{\mdpiextchar{Ꜥ}}  % U+A724
%\newunicodechar{ꜥ}{\mdpiextchar{ꜥ}}  % U+A725
%\newunicodechar{Ꜧ}{\mdpiextchar{Ꜧ}}  % U+A726
%\newunicodechar{ꜧ}{\mdpiextchar{ꜧ}}  % U+A727
%\newunicodechar{Ꜩ}{\mdpiextchar{Ꜩ}}  % U+A728
%\newunicodechar{ꜩ}{\mdpiextchar{ꜩ}}  % U+A729
%\newunicodechar{Ꜫ}{\mdpiextchar{Ꜫ}}  % U+A72A
%\newunicodechar{ꜫ}{\mdpiextchar{ꜫ}}  % U+A72B
%\newunicodechar{Ꜭ}{\mdpiextchar{Ꜭ}}  % U+A72C
%\newunicodechar{ꜭ}{\mdpiextchar{ꜭ}}  % U+A72D
%\newunicodechar{Ꜯ}{\mdpiextchar{Ꜯ}}  % U+A72E
%\newunicodechar{ꜯ}{\mdpiextchar{ꜯ}}  % U+A72F
\newunicodechar{ꜰ}{F}  % U+A730
\newunicodechar{ꜱ}{S}  % U+A731
%\newunicodechar{Ꜳ}{\mdpiextchar{Ꜳ}}  % U+A732
\newunicodechar{Ꜳ}{AA}  % U+A732
\newunicodechar{ꜳ}{\mdpiextchar{ꜳ}}  % U+A733
%\newunicodechar{Ꜵ}{\mdpiextchar{Ꜵ}}  % U+A734
%\newunicodechar{ꜵ}{\mdpiextchar{ꜵ}}  % U+A735
%\newunicodechar{Ꜷ}{\mdpiextchar{Ꜷ}}  % U+A736
\newunicodechar{Ꜷ}{AJ}  % U+A736
%\newunicodechar{ꜷ}{\mdpiextchar{ꜷ}}  % U+A737
%\newunicodechar{Ꜹ}{\mdpiextchar{Ꜹ}}  % U+A738
%\newunicodechar{ꜹ}{\mdpiextchar{ꜹ}}  % U+A739
%\newunicodechar{Ꜻ}{\mdpiextchar{Ꜻ}}  % U+A73A
%\newunicodechar{ꜻ}{\mdpiextchar{ꜻ}}  % U+A73B
%\newunicodechar{Ꜽ}{\mdpiextchar{Ꜽ}}  % U+A73C
%\newunicodechar{ꜽ}{\mdpiextchar{ꜽ}}  % U+A73D
%\newunicodechar{Ꜿ}{\mdpiextchar{Ꜿ}}  % U+A73E
%\newunicodechar{ꜿ}{\mdpiextchar{ꜿ}}  % U+A73F
%\newunicodechar{Ꝁ}{\mdpiextchar{Ꝁ}}  % U+A740
%\newunicodechar{ꝁ}{\mdpiextchar{ꝁ}}  % U+A741
%\newunicodechar{Ꝃ}{\mdpiextchar{Ꝃ}}  % U+A742
%\newunicodechar{ꝃ}{\mdpiextchar{ꝃ}}  % U+A743
%\newunicodechar{Ꝅ}{\mdpiextchar{Ꝅ}}  % U+A744
%\newunicodechar{ꝅ}{\mdpiextchar{ꝅ}}  % U+A745
%\newunicodechar{Ꝇ}{\mdpiextchar{Ꝇ}}  % U+A746
%\newunicodechar{ꝇ}{\mdpiextchar{ꝇ}}  % U+A747
%\newunicodechar{Ꝉ}{\mdpiextchar{Ꝉ}}  % U+A748
%\newunicodechar{ꝉ}{\mdpiextchar{ꝉ}}  % U+A749
%\newunicodechar{Ꝋ}{\mdpiextchar{Ꝋ}}  % U+A74A
%\newunicodechar{ꝋ}{\mdpiextchar{ꝋ}}  % U+A74B
%\newunicodechar{Ꝍ}{\mdpiextchar{Ꝍ}}  % U+A74C
%\newunicodechar{ꝍ}{\mdpiextchar{ꝍ}}  % U+A74D
%\newunicodechar{Ꝏ}{\mdpiextchar{Ꝏ}}  % U+A74E
%\newunicodechar{ꝏ}{\mdpiextchar{ꝏ}}  % U+A74F
%\newunicodechar{Ꝑ}{\mdpiextchar{Ꝑ}}  % U+A750
%\newunicodechar{ꝑ}{\mdpiextchar{ꝑ}}  % U+A751
%\newunicodechar{Ꝓ}{\mdpiextchar{Ꝓ}}  % U+A752
%\newunicodechar{ꝓ}{\mdpiextchar{ꝓ}}  % U+A753
%\newunicodechar{Ꝕ}{\mdpiextchar{Ꝕ}}  % U+A754
%\newunicodechar{ꝕ}{\mdpiextchar{ꝕ}}  % U+A755
%\newunicodechar{Ꝗ}{\mdpiextchar{Ꝗ}}  % U+A756
%\newunicodechar{ꝗ}{\mdpiextchar{ꝗ}}  % U+A757
%\newunicodechar{Ꝙ}{\mdpiextchar{Ꝙ}}  % U+A758
%\newunicodechar{ꝙ}{\mdpiextchar{ꝙ}}  % U+A759
%\newunicodechar{Ꝛ}{\mdpiextchar{Ꝛ}}  % U+A75A
%\newunicodechar{ꝛ}{\mdpiextchar{ꝛ}}  % U+A75B
%\newunicodechar{Ꝝ}{\mdpiextchar{Ꝝ}}  % U+A75C
%\newunicodechar{ꝝ}{\mdpiextchar{ꝝ}}  % U+A75D
%\newunicodechar{Ꝟ}{\mdpiextchar{Ꝟ}}  % U+A75E
%\newunicodechar{ꝟ}{\mdpiextchar{ꝟ}}  % U+A75F
%\newunicodechar{Ꝡ}{\mdpiextchar{Ꝡ}}  % U+A760
%\newunicodechar{ꝡ}{\mdpiextchar{ꝡ}}  % U+A761
%\newunicodechar{Ꝣ}{\mdpiextchar{Ꝣ}}  % U+A762
%\newunicodechar{ꝣ}{\mdpiextchar{ꝣ}}  % U+A763
%\newunicodechar{Ꝥ}{\mdpiextchar{Ꝥ}}  % U+A764
%\newunicodechar{ꝥ}{\mdpiextchar{ꝥ}}  % U+A765
%\newunicodechar{Ꝧ}{\mdpiextchar{Ꝧ}}  % U+A766
%\newunicodechar{ꝧ}{\mdpiextchar{ꝧ}}  % U+A767
%\newunicodechar{Ꝩ}{\mdpiextchar{Ꝩ}}  % U+A768
%\newunicodechar{ꝩ}{\mdpiextchar{ꝩ}}  % U+A769
%\newunicodechar{Ꝫ}{\mdpiextchar{Ꝫ}}  % U+A76A
%\newunicodechar{ꝫ}{\mdpiextchar{ꝫ}}  % U+A76B
%\newunicodechar{Ꝭ}{\mdpiextchar{Ꝭ}}  % U+A76C
%\newunicodechar{ꝭ}{\mdpiextchar{ꝭ}}  % U+A76D
%\newunicodechar{Ꝯ}{\mdpiextchar{Ꝯ}}  % U+A76E
%\newunicodechar{ꝯ}{\mdpiextchar{ꝯ}}  % U+A76F
%\newunicodechar{ꝰ}{\mdpiextchar{ꝰ}}  % U+A770
%\newunicodechar{ꝱ}{\mdpiextchar{ꝱ}}  % U+A771
%\newunicodechar{ꝲ}{\mdpiextchar{ꝲ}}  % U+A772
%\newunicodechar{ꝳ}{\mdpiextchar{ꝳ}}  % U+A773
%\newunicodechar{ꝴ}{\mdpiextchar{ꝴ}}  % U+A774
%\newunicodechar{ꝵ}{\mdpiextchar{ꝵ}}  % U+A775
%\newunicodechar{ꝶ}{\mdpiextchar{ꝶ}}  % U+A776
%\newunicodechar{ꝷ}{\mdpiextchar{ꝷ}}  % U+A777
%\newunicodechar{ꝸ}{\mdpiextchar{ꝸ}}  % U+A778
%\newunicodechar{Ꝺ}{\mdpiextchar{Ꝺ}}  % U+A779
%\newunicodechar{ꝺ}{\mdpiextchar{ꝺ}}  % U+A77A
%\newunicodechar{Ꝼ}{\mdpiextchar{Ꝼ}}  % U+A77B
%\newunicodechar{ꝼ}{\mdpiextchar{ꝼ}}  % U+A77C
%\newunicodechar{Ᵹ}{\mdpiextchar{Ᵹ}}  % U+A77D
%\newunicodechar{Ꝿ}{\mdpiextchar{Ꝿ}}  % U+A77E
%\newunicodechar{ꝿ}{\mdpiextchar{ꝿ}}  % U+A77F
%\newunicodechar{Ꞁ}{\mdpiextchar{Ꞁ}}  % U+A780
%\newunicodechar{ꞁ}{\mdpiextchar{ꞁ}}  % U+A781
%\newunicodechar{Ꞃ}{\mdpiextchar{Ꞃ}}  % U+A782
%\newunicodechar{ꞃ}{\mdpiextchar{ꞃ}}  % U+A783
%\newunicodechar{Ꞅ}{\mdpiextchar{Ꞅ}}  % U+A784
%\newunicodechar{ꞅ}{\mdpiextchar{ꞅ}}  % U+A785
%\newunicodechar{Ꞇ}{\mdpiextchar{Ꞇ}}  % U+A786
%\newunicodechar{ꞇ}{\mdpiextchar{ꞇ}}  % U+A787
%\newunicodechar{ꞈ}{\mdpiextchar{ꞈ}}  % U+A788
\newunicodechar{꞉}{:}  % U+A789
\newunicodechar{꞊}{=}  % U+A78A
\newunicodechar{Ꞌ}{\mdpiextchar{Ꞌ}}  % U+A78B
\newunicodechar{ꞌ}{\mdpiextchar{ꞌ}}  % U+A78C
\newunicodechar{ʿ}{\mdpiextchar{ʿ}}  % U+02BF
\newunicodechar{ʾ}{\mdpiextchar{ʾ}}  % U+02BE
%\newunicodechar{Ɥ}{\mdpiextchar{Ɥ}}  % U+A78D
\newunicodechar{ꞎ}{\mdpiextchar{ꞎ}}  % U+A78E
\newunicodechar{ꞏ}{\mdpiextchar{ꞏ}}  % U+A78F
\newunicodechar{Ꞑ}{\mdpiextchar{Ꞑ}}  % U+A790
\newunicodechar{ꞑ}{\mdpiextchar{ꞑ}}  % U+A791
\newunicodechar{Ꞓ}{\mdpiextchar{Ꞓ}}  % U+A792
\newunicodechar{ꞓ}{\mdpiextchar{ꞓ}}  % U+A793
\newunicodechar{ꞔ}{\mdpiextchar{ꞔ}}  % U+A794
%\newunicodechar{ꞕ}{\mdpiextchar{ꞕ}}  % U+A795
%\newunicodechar{Ꞗ}{\mdpiextchar{Ꞗ}}  % U+A796
%\newunicodechar{ꞗ}{\mdpiextchar{ꞗ}}  % U+A797
%\newunicodechar{Ꞙ}{\mdpiextchar{Ꞙ}}  % U+A798
%\newunicodechar{ꞙ}{\mdpiextchar{ꞙ}}  % U+A799
%\newunicodechar{Ꞛ}{\mdpiextchar{Ꞛ}}  % U+A79A
%\newunicodechar{ꞛ}{\mdpiextchar{ꞛ}}  % U+A79B
%\newunicodechar{Ꞝ}{\mdpiextchar{Ꞝ}}  % U+A79C
%\newunicodechar{ꞝ}{\mdpiextchar{ꞝ}}  % U+A79D
%\newunicodechar{Ꞟ}{\mdpiextchar{Ꞟ}}  % U+A79E
%\newunicodechar{ꞟ}{\mdpiextchar{ꞟ}}  % U+A79F
%\newunicodechar{Ꞡ}{\mdpiextchar{Ꞡ}}  % U+A7A0
%\newunicodechar{ꞡ}{\mdpiextchar{ꞡ}}  % U+A7A1
%\newunicodechar{Ꞣ}{\mdpiextchar{Ꞣ}}  % U+A7A2
%\newunicodechar{ꞣ}{\mdpiextchar{ꞣ}}  % U+A7A3
%\newunicodechar{Ꞥ}{\mdpiextchar{Ꞥ}}  % U+A7A4
%\newunicodechar{ꞥ}{\mdpiextchar{ꞥ}}  % U+A7A5
%\newunicodechar{Ꞧ}{\mdpiextchar{Ꞧ}}  % U+A7A6
%\newunicodechar{ꞧ}{\mdpiextchar{ꞧ}}  % U+A7A7
%\newunicodechar{Ꞩ}{\mdpiextchar{Ꞩ}}  % U+A7A8
%\newunicodechar{ꞩ}{\mdpiextchar{ꞩ}}  % U+A7A9
%\newunicodechar{Ɦ}{\mdpiextchar{Ɦ}}  % U+A7AA
%\newunicodechar{Ɜ}{\mdpiextchar{Ɜ}}  % U+A7AB
%\newunicodechar{Ɡ}{\mdpiextchar{Ɡ}}  % U+A7AC
%\newunicodechar{Ɬ}{\mdpiextchar{Ɬ}}  % U+A7AD
%\newunicodechar{Ɪ}{\mdpiextchar{Ɪ}}  % U+A7AE
%\newunicodechar{ꞯ}{\mdpiextchar{ꞯ}}  % U+A7AF
%\newunicodechar{Ꟁ}{\mdpiextchar{Ꟁ}}  % U+A7C0
%\newunicodechar{ꟁ}{\mdpiextchar{ꟁ}}  % U+A7C1
%\newunicodechar{Ꟃ}{\mdpiextchar{Ꟃ}}  % U+A7C2
%\newunicodechar{ꟃ}{\mdpiextchar{ꟃ}}  % U+A7C3
\newunicodechar{Ꞔ}{\mdpiextchar{Ꞔ}}  % U+A7C4
\newunicodechar{Ʂ}{\mdpiextchar{Ʂ}}  % U+A7C5
\newunicodechar{Ᶎ}{\mdpiextchar{Ᶎ}}  % U+A7C6
\newunicodechar{Ꟈ}{\mdpiextchar{Ꟈ}}  % U+A7C7
\newunicodechar{ꟈ}{\mdpiextchar{ꟈ}}  % U+A7C8
\newunicodechar{Ꟊ}{\mdpiextchar{Ꟊ}}  % U+A7C9
\newunicodechar{ꟊ}{\mdpiextchar{ꟊ}}  % U+A7CA
%\newunicodechar{Ɤ}{\mdpiextchar{Ɤ}}  % U+A7CB
%\newunicodechar{Ꟍ}{\mdpiextchar{Ꟍ}}  % U+A7CC
%\newunicodechar{ꟍ}{\mdpiextchar{ꟍ}}  % U+A7CD
%\newunicodechar{꟎}{\mdpiextchar{꟎}}  % U+A7CE
%\newunicodechar{꟏}{\mdpiextchar{꟏}}  % U+A7CF
\newunicodechar{Ꟑ}{\mdpiextchar{Ꟑ}}  % U+A7D0
\newunicodechar{ꟑ}{\mdpiextchar{ꟑ}}  % U+A7D1
%\newunicodechar{꟒}{\mdpiextchar{꟒}}  % U+A7D2
\newunicodechar{ꟓ}{\mdpiextchar{ꟓ}}  % U+A7D3
%\newunicodechar{꟔}{\mdpiextchar{꟔}}  % U+A7D4
\newunicodechar{ꟕ}{\mdpiextchar{ꟕ}}  % U+A7D5
\newunicodechar{Ꟗ}{\mdpiextchar{Ꟗ}}  % U+A7D6
\newunicodechar{ꟗ}{\mdpiextchar{ꟗ}}  % U+A7D7
\newunicodechar{Ꟙ}{\mdpiextchar{Ꟙ}}  % U+A7D8
\newunicodechar{ꟙ}{\mdpiextchar{ꟙ}}  % U+A7D9
%\newunicodechar{Ꟛ}{\mdpiextchar{Ꟛ}}  % U+A7DA
%\newunicodechar{ꟛ}{\mdpiextchar{ꟛ}}  % U+A7DB
%\newunicodechar{Ƛ}{\mdpiextchar{Ƛ}}  % U+A7DC
%\newunicodechar{꟝}{\mdpiextchar{꟝}}  % U+A7DD
%\newunicodechar{꟞}{\mdpiextchar{꟞}}  % U+A7DE
%\newunicodechar{꟟}{\mdpiextchar{꟟}}  % U+A7DF
%\newunicodechar{꟠}{\mdpiextchar{꟠}}  % U+A7E0
%\newunicodechar{꟡}{\mdpiextchar{꟡}}  % U+A7E1
%\newunicodechar{꟢}{\mdpiextchar{꟢}}  % U+A7E2
%\newunicodechar{꟣}{\mdpiextchar{꟣}}  % U+A7E3
%\newunicodechar{꟤}{\mdpiextchar{꟤}}  % U+A7E4
%\newunicodechar{꟥}{\mdpiextchar{꟥}}  % U+A7E5
%\newunicodechar{꟦}{\mdpiextchar{꟦}}  % U+A7E6
%\newunicodechar{꟧}{\mdpiextchar{꟧}}  % U+A7E7
%\newunicodechar{꟨}{\mdpiextchar{꟨}}  % U+A7E8
%\newunicodechar{꟩}{\mdpiextchar{꟩}}  % U+A7E9
%\newunicodechar{꟪}{\mdpiextchar{꟪}}  % U+A7EA
%\newunicodechar{꟫}{\mdpiextchar{꟫}}  % U+A7EB
%\newunicodechar{꟬}{\mdpiextchar{꟬}}  % U+A7EC
%\newunicodechar{꟭}{\mdpiextchar{꟭}}  % U+A7ED
%\newunicodechar{꟮}{\mdpiextchar{꟮}}  % U+A7EE
%\newunicodechar{꟯}{\mdpiextchar{꟯}}  % U+A7EF
%\newunicodechar{꟰}{\mdpiextchar{꟰}}  % U+A7F0
%\newunicodechar{꟱}{\mdpiextchar{꟱}}  % U+A7F1
%\newunicodechar{ꟲ}{\mdpiextchar{ꟲ}}  % U+A7F2
%\newunicodechar{ꟳ}{\mdpiextchar{ꟳ}}  % U+A7F3
%\newunicodechar{ꟴ}{\mdpiextchar{ꟴ}}  % U+A7F4
%\newunicodechar{Ꟶ}{\mdpiextchar{Ꟶ}}  % U+A7F5
%\newunicodechar{ꟶ}{\mdpiextchar{ꟶ}}  % U+A7F6
%\newunicodechar{ꟷ}{\mdpiextchar{ꟷ}}  % U+A7F7
%\newunicodechar{ꟸ}{\mdpiextchar{ꟸ}}  % U+A7F8
%\newunicodechar{ꟹ}{\mdpiextchar{ꟹ}}  % U+A7F9
%\newunicodechar{ꟺ}{\mdpiextchar{ꟺ}}  % U+A7FA
%\newunicodechar{ꟻ}{\mdpiextchar{ꟻ}}  % U+A7FB
%\newunicodechar{ꟼ}{\mdpiextchar{ꟼ}}  % U+A7FC
%\newunicodechar{ꟽ}{\mdpiextchar{ꟽ}}  % U+A7FD
%\newunicodechar{ꟾ}{\mdpiextchar{ꟾ}}  % U+A7FE
%\newunicodechar{ꟿ}{\mdpiextchar{ꟿ}}  % U+A7FF


==> Definitions/unicode.tex <==
%% Updated on 2 September 2026
%% Pagella-missing / special Unicode mappings (pdfLaTeX) — loaded by mdpi.cls when class option unicode is set.
%%   \documentclass[...,unicode]{Definitions/mdpi}

\DeclareUnicodeCharacter{1E45}{\.{n}}
\DeclareUnicodeCharacter{1E41}{\.{m}}
\DeclareUnicodeCharacter{2003}{\quad}
%\DeclareUnicodeCharacter{0177}{\^{y}}
%\DeclareUnicodeCharacter{101}{\={a}}
\DeclareUnicodeCharacter{2009}{\thinspace}
\DeclareUnicodeCharacter{2002}{\enspace{}}
\DeclareUnicodeCharacter{2005}{\thinspace}
\DeclareUnicodeCharacter{0263}{\textipa{G}}
%\DeclareUnicodeCharacter{117}{\.{e}}
\DeclareUnicodeCharacter{A0}{~}
\DeclareUnicodeCharacter{2460}{\textcircled{\scriptsize{1}}}
\DeclareUnicodeCharacter{2461}{\textcircled{\scriptsize{2}}}
\DeclareUnicodeCharacter{2462}{\textcircled{\scriptsize{3}}}
\DeclareUnicodeCharacter{2463}{\textcircled{\scriptsize{4}}}
\DeclareUnicodeCharacter{2464}{\textcircled{\scriptsize{5}}}
\DeclareUnicodeCharacter{2465}{\textcircled{\scriptsize{6}}}
\DeclareUnicodeCharacter{2466}{\textcircled{\scriptsize{7}}}
\DeclareUnicodeCharacter{2467}{\textcircled{\scriptsize{8}}}
\DeclareUnicodeCharacter{2468}{\textcircled{\scriptsize{9}}}
\DeclareUnicodeCharacter{2070}{\textsuperscript{0}}
\DeclareUnicodeCharacter{2074}{\textsuperscript{4}}
\DeclareUnicodeCharacter{2075}{\textsuperscript{5}}
\DeclareUnicodeCharacter{2076}{\textsuperscript{6}}
\DeclareUnicodeCharacter{2077}{\textsuperscript{7}}
\DeclareUnicodeCharacter{2078}{\textsuperscript{8}}
\DeclareUnicodeCharacter{2079}{\textsuperscript{9}}
\DeclareUnicodeCharacter{02C2}{<}
\DeclareUnicodeCharacter{2033}{\relax\ifmmode '' \else $''$\fi}
\DeclareUnicodeCharacter{2034}{\relax\ifmmode ''' \else $'''$\fi}
\DeclareUnicodeCharacter{2026}{\relax\ifmmode … \else $\ldots$\fi}
\DeclareUnicodeCharacter{0229}{\c{e}}
\DeclareUnicodeCharacter{016F}{\r{u}}
%\DeclareUnicodeCharacter{0218}{\cb{S}}
%\DeclareUnicodeCharacter{0219}{\cb{s}}
%\DeclareUnicodeCharacter{021B}{\cb{t}}
\DeclareUnicodeCharacter{127}{\relax\ifmmode\rm\hbar\else $\rm\hbar$\fi}
\DeclareUnicodeCharacter{3AC}{\relax\ifmmode\acute{\alpha}\else $\acute{\alpha}$\fi}
\DeclareUnicodeCharacter{3AD}{\relax\ifmmode\acute{\varepsilon}\else $\acute{\varepsilon}$\fi}
\DeclareUnicodeCharacter{3AE}{\relax\ifmmode\acute{\eta}\else $\acute{\eta}$\fi}
\DeclareUnicodeCharacter{3AF}{\relax\ifmmode\acute{\iota}\else $\acute{\iota}$\fi}
\DeclareUnicodeCharacter{3CC}{\relax\ifmmode\acute{o}\else $\acute{o}$\fi}
\DeclareUnicodeCharacter{3CD}{\relax\ifmmode\acute{\upsilon}\else $\acute{\upsilon}$\fi}
\DeclareUnicodeCharacter{3CE}{\relax\ifmmode\acute{\omega}\else $\acute{\omega}$\fi}
\DeclareUnicodeCharacter{391}{A}
\DeclareUnicodeCharacter{392}{B}
\DeclareUnicodeCharacter{395}{E}
\DeclareUnicodeCharacter{396}{Z}
\DeclareUnicodeCharacter{397}{H}
\DeclareUnicodeCharacter{399}{I}
\DeclareUnicodeCharacter{39A}{K}
\DeclareUnicodeCharacter{39C}{M}
\DeclareUnicodeCharacter{39D}{N}
\DeclareUnicodeCharacter{39F}{O}
\DeclareUnicodeCharacter{3A1}{P}
\DeclareUnicodeCharacter{3A4}{T}
\DeclareUnicodeCharacter{3A7}{X}

\DeclareUnicodeCharacter{00B5}{\relax\ifmmode \mu{} \else $\mu$\fi}
\DeclareUnicodeCharacter{27E6}{\relax\ifmmode \llbracket \else $\llbracket$\fi}
\DeclareUnicodeCharacter{27E7}{\relax\ifmmode \rrbracket \else $\rrbracket$\fi}
\DeclareUnicodeCharacter{1D434}{\relax\ifmmode A \else $A$\fi}
\DeclareUnicodeCharacter{1D435}{\relax\ifmmode B \else $B$\fi}
\DeclareUnicodeCharacter{1D436}{\relax\ifmmode C \else $C$\fi}
\DeclareUnicodeCharacter{1D437}{\relax\ifmmode D \else $D$\fi}
\DeclareUnicodeCharacter{1D438}{\relax\ifmmode E \else $E$\fi}
\DeclareUnicodeCharacter{1D439}{\relax\ifmmode F \else $F$\fi}
\DeclareUnicodeCharacter{1D43A}{\relax\ifmmode G \else $G$\fi}
\DeclareUnicodeCharacter{1D43B}{\relax\ifmmode H \else $H$\fi}
\DeclareUnicodeCharacter{1D43C}{\relax\ifmmode I \else $I$\fi}
\DeclareUnicodeCharacter{1D43D}{\relax\ifmmode J \else $J$\fi}
\DeclareUnicodeCharacter{1D43E}{\relax\ifmmode K \else $K$\fi}
\DeclareUnicodeCharacter{1D43F}{\relax\ifmmode L \else $L$\fi}
\DeclareUnicodeCharacter{1D440}{\relax\ifmmode M \else $M$\fi}
\DeclareUnicodeCharacter{1D441}{\relax\ifmmode N \else $N$\fi}
\DeclareUnicodeCharacter{1D442}{\relax\ifmmode O \else $O$\fi}
\DeclareUnicodeCharacter{1D443}{\relax\ifmmode P \else $P$\fi}
\DeclareUnicodeCharacter{1D444}{\relax\ifmmode Q \else $Q$\fi}
\DeclareUnicodeCharacter{1D445}{\relax\ifmmode R \else $R$\fi}
\DeclareUnicodeCharacter{1D446}{\relax\ifmmode S \else $S$\fi}
\DeclareUnicodeCharacter{1D447}{\relax\ifmmode T \else $T$\fi}
\DeclareUnicodeCharacter{1D448}{\relax\ifmmode U \else $U$\fi}
\DeclareUnicodeCharacter{1D449}{\relax\ifmmode V \else $V$\fi}
\DeclareUnicodeCharacter{1D44A}{\relax\ifmmode W \else $W$\fi}
\DeclareUnicodeCharacter{1D44B}{\relax\ifmmode X \else $X$\fi}
\DeclareUnicodeCharacter{1D44C}{\relax\ifmmode Y \else $Y$\fi}
\DeclareUnicodeCharacter{1D44D}{\relax\ifmmode Z \else $Z$\fi}
\DeclareUnicodeCharacter{1D44E}{\relax\ifmmode a \else $a$\fi}
\DeclareUnicodeCharacter{1D44F}{\relax\ifmmode b \else $b$\fi}
\DeclareUnicodeCharacter{1D450}{\relax\ifmmode c \else $c$\fi}
\DeclareUnicodeCharacter{1D451}{\relax\ifmmode d \else $d$\fi}
\DeclareUnicodeCharacter{1D452}{\relax\ifmmode e \else $e$\fi}
\DeclareUnicodeCharacter{1D453}{\relax\ifmmode f \else $f$\fi}
\DeclareUnicodeCharacter{1D454}{\relax\ifmmode g \else $g$\fi}
\DeclareUnicodeCharacter{1D456}{\relax\ifmmode i \else $i$\fi}
\DeclareUnicodeCharacter{1D457}{\relax\ifmmode j \else $j$\fi}
\DeclareUnicodeCharacter{1D458}{\relax\ifmmode k \else $k$\fi}
\DeclareUnicodeCharacter{1D459}{\relax\ifmmode l \else $l$\fi}
\DeclareUnicodeCharacter{1D45A}{\relax\ifmmode m \else $m$\fi}
\DeclareUnicodeCharacter{1D45B}{\relax\ifmmode n \else $n$\fi}
\DeclareUnicodeCharacter{1D45C}{\relax\ifmmode o \else $o$\fi}
\DeclareUnicodeCharacter{1D45D}{\relax\ifmmode p \else $p$\fi}
\DeclareUnicodeCharacter{1D45E}{\relax\ifmmode q \else $q$\fi}
\DeclareUnicodeCharacter{1D45F}{\relax\ifmmode r \else $r$\fi}
\DeclareUnicodeCharacter{1D460}{\relax\ifmmode s \else $s$\fi}
\DeclareUnicodeCharacter{1D461}{\relax\ifmmode t \else $t$\fi}
\DeclareUnicodeCharacter{1D462}{\relax\ifmmode u \else $u$\fi}
\DeclareUnicodeCharacter{1D463}{\relax\ifmmode v \else $v$\fi}
\DeclareUnicodeCharacter{1D464}{\relax\ifmmode w \else $w$\fi}
\DeclareUnicodeCharacter{1D465}{\relax\ifmmode x \else $x$\fi}
\DeclareUnicodeCharacter{1D466}{\relax\ifmmode y \else $y$\fi}
\DeclareUnicodeCharacter{1D467}{\relax\ifmmode z \else $z$\fi}

\DeclareUnicodeCharacter{1E67}{\.{\v s}}
\DeclareUnicodeCharacter{1E11}{\relax\ifmmode \c{d} \else $\c{d}$\fi}
\DeclareUnicodeCharacter{1ECB}{\relax\ifmmode \d{i} \else $\d{i}$\fi}
\DeclareUnicodeCharacter{1D8D}{\relax\ifmmode \textlhookx \else $\textlhookx$\fi}
\DeclareUnicodeCharacter{104}{\relax\ifmmode \k{A} \else $\k{A}$\fi}
\DeclareUnicodeCharacter{211E}{\relax\ifmmode \textrecipe \else $\textrecipe$\fi}
\DeclareUnicodeCharacter{29D}{\relax\ifmmode \textctj \else $\textctj$\fi}

\DeclareUnicodeCharacter{1E2E}{\'{\"I}}
\DeclareUnicodeCharacter{23F}{\textrts}

\DeclareUnicodeCharacter{2C73}{\varw}

\DeclareUnicodeCharacter{2127}{\mho}

\DeclareUnicodeCharacter{28C}{\textturnv}
\DeclareUnicodeCharacter{252}{\textturnscripta}
\DeclareUnicodeCharacter{259}{\schwa}
\DeclareUnicodeCharacter{25B}{\m{e}}
\DeclareUnicodeCharacter{266}{\m{h}}
\DeclareUnicodeCharacter{127}{\B{h}}
\DeclareUnicodeCharacter{27E}{\textfishhookr}
\DeclareUnicodeCharacter{281}{\textinvscr}

